A robust approach for estimating change-points in the mean of an AR(p) process

We consider the problem of change-points estimation in the mean of an AR(p) process. Taking into account the dependence structure does not allow us to use the approach of the independent case. Especially, the dynamic programming algorithm giving the optimal solution in the independent case cannot be used anymore. We propose a two-step method, based on the preliminary robust (to the change-points) estimation of the autoregression parameters. Then, we propose to follow the classical approach, by plugging this estimator in the criterion used for change-point estimation, which is equivalent to decorrelate the series using the estimated autoregression parameters. We show that the asymptotic properties of these change-point location and mean estimators are the same as those of the classical estimators in the independent framework. The same plug-in approach is then used to approximate the modified BIC and choose the number of segments, and to derive a heuristic BIC criterion to select both the number of changes and the order of the autoregression. Finally, we show, in the simulation section, that for finite sample size taking into account the dependence structure improves the statistical performance of the change-point estimators and of the selection criterion.

==> chapitres/ar1.tex <==
\selectlanguage{french}
%
%\selectlanguage{francais}
%\includepdf[pages=1-41]{Bernoulli2/article.pdf}
Dans ce chapitre est présenté un article, co-écrit avec Stéphane Robin, \'Emilie Lebarbier et Céline Lévy-Leduc. Cet article a été soumis à la revue \emph{Bernoulli} et est actuellement cours de relecture. Des remarques additionnelles sur cet article, non proposées à publication, sont présentées dans la section~\ref{ch:commentaires:sec:ar1}.

\input{./chapitres/ar1/article.tex}

==> chapitres/ar1/article.tex <==
\begin{abstract}
\thispagestyle{plain}
Le problème qui nous intéresse est celui de l'estimation de ruptures multiples dans l'espérance d'un processus AR(1) gaussien. La prise en compte de la structure de dépendance nous interdit l'utilisation de l'algorithme de programmation dynamique, qui est le seul algorithme permettant de calculer la segmentation optimale dans le cas indépendant. Nous proposons un estimateur robuste du paramètre de la fonction d'autocorrelation, consistant et asymptotiquement gaussien. Nous proposons alors de suivre l'approche inférentielle classique en injectant cet estimateur dans le critère utilisé pour l'estimation de la localisation des ruptures. Nous démontrons que ces estimateurs partagent les propriétés asymptotiques des estimateurs classiques dans le cadre indépendant. La même approche \emph{plug-in}est alors utilisée pour approcher le critère BIC modifié et sélectionner le nombre de segments. Cette méthode est implémentée dans le package R \textsf{AR1seg} et est disponible sur le \emph{Comprehensive R Archive Network} (CRAN). Ce package est utilisé dans la section simulations dans laquelle nous montrons que pour des séries de taille finie la prise en compte de la structure de dépendance améliore les performances statistiques des estimateurs des instants de rupture et du nombre de ruptures sélectionné.
\end{abstract}


\selectlanguage{english}

\begin{abstract}
\thispagestyle{plain}
We consider the problem of multiple change-point estimation in the mean of a Gaussian AR(1) process.  Taking into account the dependence structure does not allow us to use the dynamic programming algorithm, which is the only algorithm giving the optimal solution in the independent case. We propose a robust estimator of the autocorrelation parameter, which is consistent and satisfies a central limit theorem. Then, we propose to follow the classical inference approach, by plugging this estimator in the criterion used for change-points estimation. We show that the asymptotic properties of these estimators are the same as those of the classical estimators in the independent framework. The same plug-in approach is then used to approximate the modified BIC and choose the number of segments. This method is implemented in the R package \textsf{AR1seg} and is available from the Comprehensive R Archive Network (CRAN). This package is used in the simulation section in which we show that for finite sample sizes taking into account the dependence structure improves the statistical performance of the change-point estimators and of the selection criterion.
\end{abstract}

\input{./chapitres/ar1/article/Intro.tex}
%
\input{./chapitres/ar1/article/Correlation.tex}
%%
\input{./chapitres/ar1/article/Segment.tex}
%%
\input{./chapitres/ar1/article/Selection.tex}
%%
\input{./chapitres/ar1/article/Simul.tex}
%%
\input{./chapitres/ar1/article/Conclusion.tex}
%
\input{./chapitres/ar1/article/supplement.tex}
%
%%% Local Variables:
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "article.tex"
%%% ispell-local-dictionary: "en_US"
%%% eval: (flyspell-mode 1)
%%% End:

==> chapitres/ar1/article/Conclusion.tex <==
\section{Conclusion}

In this paper, we propose a novel approach for estimating multiple change-points
in the mean of a Gaussian AR(1) process. Our approach is based on two main stages.
The first one consists in building a robust estimator of the autocorrelation parameter
which is used for whitening the original series. In the second stage, we apply
the inference approach commonly used to estimate change-points in the mean
of independent random variables. 
In the course of this study, we have shown that our approach, which is implemented in the R 
package \textsf{AR1seg}, is a very efficient
technique both on a theoretical and practical point of view.
More precisely, it has two main features which make it very
attractive. Firstly, the estimators that we propose have the same asymptotic properties as the classical estimators 
in the independent framework which means that the performances of our estimators are not affected by the dependence assumption.
Secondly, from a practical point of view, \textsf{AR1seg} is computationally
efficient and exhibits better performance on finite sample size data than 
existing approaches which do not take into account the dependence structure of the observations.

%%% Local Variables:
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "article.tex"
%%% ispell-local-dictionary: "en_US"
%%% eval: (flyspell-mode 1)
%%% End: 

==> chapitres/ar1/article/Correlation.tex <==
\section{Robust estimation of the parameter $\rho^{\star}$}\label{ar1:sec:correlation}

The aim of this section is to provide an estimator of $\rho^{\star}$ which can deal with the
presence of change-points in the data. In the absence of change-points ($m^{\star}=0$ in \eqref{ar1:eq:modele_new}), a consistent estimator
of $\rho^{\star}$ could be obtained by using the classical autocorrelation function estimator of $(y_i)_{0\leq i\leq n}$ computed at lag 1. 
Since change-points can be seen as outliers
in the AR(1) process, we shall propose a robust approach
for estimating $\rho^{\star}$. 
\textcite{MG} propose a robust estimator of the autocorrelation function of a stationary time series 
based on the robust scale estimator proposed by \textcite{CR}.
More precisely, the approach of \textcite{MG} would result in the following estimate of $\rho^{\star}$:
\begin{equation*}
\widehat{\rho}_{\textrm{MG}}=\dfrac{Q_{n}^2 \left(y^+\right) - Q_{n}^2 \left(y^-\right)}{Q_{n}^2 \left(y^+\right) + Q_{n}^2 \left(y^-\right)}\;,
\end{equation*}
where $y^+ = (y_{i+1}+y_i)_{0\leq i\leq n-1}$, $y^- = (y_{i+1}-y_i)_{0\leq i\leq n-1}$ 
and $Q_n$ is the scale estimator of \textcite{CR} which is such that $Q_n \left(x\right)$
is proportional to the first quartile of
\begin{equation*}
\left\lbrace \vert x_i - x_j \vert ; 0\leq i<j\leq n \right\rbrace \; .
\end{equation*}

The asymptotic properties of this estimator are studied by \textcite{levy2011robust} for Gaussian stationary processes with either short-range or long-range dependence.
However, as we shall see in the simulation section we can provide an estimator of $\rho^{\star}$ which is more
robust to the presence of change-points than $\widehat{\rho}_{\textrm{MG}}$. The asymptotic properties of 
this novel robust estimator are given in Proposition~\ref{ar1:prop:correlation}.


\begin{prop}\label{ar1:prop:correlation}
Let $y_0,\dots,y_n$ be $(n+1)$ observations satisfying (\ref{ar1:eq:modele_new}) 
%with $m=0$ 
and let
\begin{equation}\label{ar1:eq:est_rho}
\widetilde{\rho}_n = \frac{\left(\underset{0\leq i\leq n-2}{\med} \left|y_{i+2}-y_i\right|\right)^2}
{\left(\underset{0\leq i\leq n-1}{\med} \left|y_{i+1}-y_i\right|\right)^2}-1 \;,
\end{equation}
where $\med x_i$ denotes the median. Then, $\widetilde{\rho}_n$ satisfies
the following central limit theorem
\begin{equation}\label{ar1:eq:tcl_rho_tilde}
\sqrt{n}(\widetilde{\rho}_n - \rho^{\star})\stackrel{d}{\longrightarrow}\mathcal{N}(0,\tilde{\sigma}^2)\;, \textrm{ as } n\to\infty\;,
\end{equation}
where
\begin{equation}\label{ar1:eq:def_sigmatilde}
\tilde{\sigma}^2=\PE[\Psi(\eta_0,\eta_1,\eta_2)^2]
+2\sum_{k\geq 1}\PE\left[\Psi(\eta_0,\eta_1,\eta_2)\Psi(\eta_k,\eta_{k+1},\eta_{k+2})\right]\;,
\end{equation}
and the function $\Psi$ is defined by
\begin{multline}\label{ar1:eq:def_Psi}
\Psi : (x_0,x_1,x_2)\mapsto\\ -\frac{\left(1+\rho^{\star}\right)}{\Phi^{-1}(3/4)\varphi\left(\Phi^{-1}(3/4)\right)}
\left[\1_{\left\{|x_2-x_0|\leq \sqrt{2\sigma^{\star 2}}\Phi^{-1}(3/4)\right\}} - \1_{\left\{|x_1-x_0|\leq \sqrt{\frac{2\sigma^{\star 2}}{1+\rho^{\star}}}\Phi^{-1}(3/4)\right\}}\right]\;,
\end{multline}
where $\Phi$ and $\varphi$ denote the cumulative distribution function and the probability distribution function
of a standard Gaussian rv, respectively.
\end{prop}
The proof of Proposition \ref{ar1:prop:correlation} is given in Section \ref{ar1:proof:corr_tcl}.

\begin{remark}\label{ar1:corrr:remark:moments}
Let us now compare the properties of $\widetilde{\rho}_n$ with the properties of $\widehat{\rho}_n(1)$ where $\widehat{\rho}_n(\cdot)$ denotes the classical estimator of the autocorrelation function computed from $y_0,\dots,y_{n}$ defined in \eqref{ar1:eq:modele_new} with $m^{\star}=0$. By \textcite[Theorem~7.2.1 and Example~7.2.3]{brockwell}, we get that
$$
\sqrt{n}(\widehat{\rho}_n(1)-\rho^{\star})\stackrel{d}{\longrightarrow}\mathcal{N}\left(0,1-{\rho^{\star}}^2\right)\;,\textrm{ as }
n\to\infty\;.$$
From this result, we can see that $\widetilde{\rho}_n$ converges to $\rho^{\star}$ at the same rate as $\widehat{\rho}_n(1)$
except that our result still holds when $m\neq 0$.
\end{remark}

\begin{remark}\label{ar1:corrr:remark:test}
{Note that the asymptotic distribution given in \eqref{ar1:eq:tcl_rho_tilde} allows to define a test of $(H_0):$ `$\rho^{\star}=0$' as the asymptotic variance $\widetilde{\sigma}^2$ does not depend on any unknown parameter under $H_0$.}
\end{remark}

\begin{remark}
Since the estimator \eqref{ar1:eq:est_rho} involves differences of the process $(y_i)$ at different instants, 
it can only be used in the case of stable distributions as defined by \textcite{feller:1971}. 
Among them, we can quote the Cauchy, L\'evy and Gaussian distributions, where the Gaussian distribution is the only one
to have a finite second order moment. We give some hints in Section~\ref{ar1:subsec:hints} to explain why, in the case of the
Cauchy distribution, taking $\widetilde{\widetilde{\rho}}_n$ defined as follows leads to an accurate estimator of $\rho^\star$:
\begin{equation}\label{ar1:eq:rho_cauchy}
\widetilde{\widetilde{\rho}}_n=
\left\{
\begin{array}{cc}
-1+\sqrt{1+\widetilde{\rho}_n},&\textrm{if } \widetilde{\rho}_n\geq 0\;,\\
-\sqrt{1-\sqrt{1+\widetilde{\rho}_n}},&\textrm{if } \widetilde{\rho}_n<0\;,
\end{array}
\right.
\end{equation}
where $\widetilde{\rho}_n$ is defined by \eqref{ar1:eq:est_rho}.
Some simulations are also provided in Section~\ref{ar1:sec:add_simul} to illustrate the finite sample size 
properties of this estimator.
\end{remark}




%%% Local Variables:
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "article.tex"
%%% ispell-local-dictionary: "en_US"
%%% eval: (flyspell-mode 1)
%%% End: 

==> chapitres/ar1/article/Intro.tex <==
\section{Introduction}

Change-point detection problems arise in many fields, such as
genomics~\parencites{braun1998statistical}{braun2000multiple}{picard2005statistical}, medical imaging~\citep{lavielle2005using}, earth sciences~\parencites{Williams2003}{Gazeaux2013}, econometrics \parencites{lai2005autoregressive}{lavielle1999} or climate \parencites{mestre2000methodes}{climat}. In many of these problems, the observations can not be assumed to be independent. Indeed the autocovariance structure of
the time series display more complex patterns and might be taken
into account in change-point estimation.

An abundant literature exists about the statistical theory of
change-point detection. Only speaking about Gaussian processes,
various frameworks have been considered ranging from the independent
case with changes in the mean \citep{Bas93N}, to more complex
structural changes \citep{BP}, dependent processes
\citep{lavielle1999} or processes with changes in all parameters
\citep{BKW10}.

\textcites{lavielle1999}{LM} proved that, if the
number of changes is known, the least-squares estimators of the
change-point locations and of the parameters of each segment are
consistent under very mild conditions on the autocovariance
structure of the process with changes in the mean. A
quasi-likelihood approach is also proved to provide consistent
estimates for the model with changes in all
parameters by \textcite{BKW10}. 
 Many model selection criteria have also
been proposed to estimate the number of changes, mostly in the
independent case \parencites(see for example)(){yao}{lavielle2005using}{lebarbier2005detecting}{ZS}.

Change-point detection also raises algorithmic issues as the determination of the optimal set of change-point locations is a discrete optimization problem. The dynamic programming algorithm introduced by \textcite{AugerLawrence} is the only way to recover this optimal segmentation. The computational complexity of this algorithms is quadratic relatively to the length of the series. Only this algorithm and some of its improvements \parencites(such as these proposed by)(){pruned}[or][]{killick2012optimal} provide exactly the optimal change-point location estimators.

However, the dynamic programming algorithm only applies when ($i$) the loss function~(e.g. the negative log-likelihood) is additive with respect to the segments and when ($ii$) no parameter to be estimated is common to several segments. These requirements are met by the least-square criterion (which corresponds to the negative log-likelihood in the Gaussian homoscedastic independent model with changes in the mean) or by the model and criterion considered by \textcite{BKW10}. In other cases, iterative and stochastic procedures are needed \parencites(see)(){BPalgo}[or][]{LiL12}.

In this paper, we consider the segmentation of an AR(1) process with homogeneous auto-correlation coefficient $\rho^{\star}$:
\begin{equation}\label{ar1:eq:modele_new}
y_i=\mu_k^{\star}+\eta_i\;,\;
t_{n,k}^{\star}+1\leq i\leq t_{n,k+1}^{\star}\;,\; 0\leq k\leq m^{\star}\;,\; 1\leq
i\leq n\;,
\end{equation}
where $(\eta_i)_{i\in \mathbb{Z}}$ is a zero-mean stationary AR(1) Gaussian process defined as the solution of
\begin{equation}\label{ar1:eq:ar1}
\eta_i = \rho^{\star}\eta_{i-1} + \epsilon_i\;,
\end{equation}
where $|\rho^{\star}|<1$ and the $\epsilon_i$'s are  iid zero-mean Gaussian rv's with variance $\sigma^{\star2}$. We further also assume that $y_0$ is a Gaussian random variable with mean $\mu_0^{\star}$ and variance $\sigma^{\star2}/(1-{\rho^{\star}}^2)$.
Actually, most of the results we provide in this paper hold without the Gaussian assumption.

Note that this model is different from the ones considered by \textcite{davis2006structural} and \textcite{BKW10}. Indeed, \textcite{davis2006structural} considered the segmentation issue of a non-stationary time series which consists of blocks of different autoregressive processes where all the parameters of the autoregressive processes change from one segment to the other. \textcite{BKW10} proposed a methodology for estimating the change-points of a non-stationary time series built from a general class of models having piecewise constant parameters. In this framework, all the parameters may change jointly at each change-point. This differs from our Model~\eqref{ar1:eq:modele_new} where the parameters $\rho^{\star}$ and $\sigma^{\star}$ are not assumed to change from one segment to the other.
The direct maximum-likelihood inference for such a process violates both requirements ($i$) and ($ii$). Indeed the log-likelihood is not additive with respect to the segments because of the dependence that exists between data from neighbor segments and the unknown coefficient $\rho^{\star}$ needs to be estimated jointly over all segments.

Our aim is to propose a methodology for estimating both the change-point locations $\boldsymbol{t_n^{\star}} = (t_{n,k}^{\star})_{1\leq k\leq m^{\star}}$ and the means $\boldsymbol{\mu}^{\star}=(\mu_k^{\star})_{0\leq k\leq m^{\star}}$, accounting for the existence of the auto-correlation $\rho^{\star}$.

In the sequel, we shall use the following conventions: $t_{n,0}^{\star}=0,t_{n,m^{\star}+1}^{\star}=n$ and assume that there exists $\boldsymbol{\tau^{\star}}=(\tau_k^{\star})_{0\leq k\leq m+1}$ such that, for $0\leq k\leq m+1$ $t_{n,k}^{\star}=\lfloor n\tau_k^{\star}\rfloor$, $\lfloor x\rfloor$ denoting the integer part of $x$. Consequently, $\tau_0^{\star}=0$ and $\tau_{m^{\star}+1}^{\star}=1$.

If $\rho^{\star}$ was known, the series could be decorrelated and the dynamic programming algorithm then used for the segmentation of this decorrelated series. Here, $\rho^{\star}$ is unknown, but is estimated, and this estimator is then used to decorrelate the series.

To this aim, we borrow techniques from robust estimation \citep{MG}. Briefly speaking, we consider the data observed at the change-point locations as outliers and propose an estimate of $\rho^{\star}$ that is robust to the presence of such outliers. We shall prove that the estimate we propose is consistent and satisfies a central limit theorem.

We shall prove that the resulting change-point estimators satisfy the same asymptotic properties as those proposed by \textcites{LM}{BKW10}. 
Finally, we propose a model selection criterion inspired by the one proposed by \textcite{ZS} and prove some asymptotic properties of this criterion.

This method is implemented in the R package \textsf{AR1seg} and is available from the Comprehensive R Archive Network (CRAN).

This paper is organized as follows. In Section~\ref{ar1:sec:correlation}, we propose a robust estimator for $\rho^{\star}$ and establish its asymptotic properties. In Section~\ref{ar1:sec:change-points}, we prove that the change-point estimators defined in~\eqref{ar1:eq:tau_n} are consistent in both the Gaussian and the non-Gaussian case. In Section~\ref{ar1:sec:selection}, we provide a consistent model selection criterion in the non-Gaussian case and derive an approximation of a Gaussian criterion. In Section~\ref{ar1:sec:simul}, we illustrate by a simulation study the performance of this approach for time series having a finite sample size.

%%% Local Variables:
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "article.tex"
%%% ispell-local-dictionary: "en_US"
%%% eval: (flyspell-mode 1)
%%% End: 

==> chapitres/ar1/article/Segment.tex <==
\section{Change-points and expectations estimation}\label{ar1:sec:change-points}

In this section, the number of change-points $m^{\star}$ is assumed to be known. In the sequel, for notational simplicity, $m^{\star}$ will be denoted by $m$. 
Our goal is to estimate both the change-points and the means in Model~\eqref{ar1:eq:modele_new}. A first idea consists in using the following criterion which is based on a quasi-likelihood conditioned on $y_0$ and to minimize it with respect to $\rho$:
\begin{equation*}
\sum_{k=0}^{m} \sum_{i=t_{k}+2}^{t_{k+1}} \left(y_i- \rho y_{i-1}-\delta_k\right)^2 + \sum_{k=1}^m  \left\{\left(y_{t_k +1}-\frac{\delta_k}{1-\rho}\right)- \rho \left(y_{t_k}-\frac{\delta_{k-1}}{1-\rho}\right)\right\}^2 + \left(y_1- \rho y_{0}-\delta_0\right)^2 .
\end{equation*}
Due to the term that involves both $\delta_{k-1}$ and $\delta_k$, this criterion cannot be efficiently minimized. Therefore, we propose to use an alternative criterion defined as follows:
\begin{equation}\label{ar1:eq:SSm_def}
% S\left(y,\rho, \boldsymbol{\delta},\boldsymbol{t}\right) = \frac{1}{n}\sum_{k=0}^m \sum_{i=t_k +1}^{t_{k+1}}
% \left(y_i-\overline{\rho}_n y_{i-1}- \delta_k\right)^2 .
SS_m\left(y,\rho, \boldsymbol{\delta},\boldsymbol{t}\right) = \sum_{k=0}^m \sum_{i=t_k +1}^{t_{k+1}}
\left(y_i-\rho y_{i-1}- \delta_k\right)^2\;.
\end{equation}
Note that $SS_m\left(z,\rho, \left(1-\rho\right) \boldsymbol{\mu},\boldsymbol{t}\right)$ corresponds to $-n/2$ times the log-likelihood of the following model maximized with respect to $\sigma$:
\begin{eqnarray}\label{ar1:eq:bkw}
z_i - \mu_k^{\star} & = & \rho^{\star} \left(z_{i-1} - \mu_k^{\star}\right) +\epsilon_i\;,\; t_{n,k}^{\star}+1\leq i\leq t_{n,k+1}^{\star}\;,\; 0\leq k\leq m\;,\; 1\leq i\leq n\;,
\end{eqnarray}
and where $z_0$ is a Gaussian rv with mean $\mu_0^{\star}$ and variance $\sigma^{ \star2}/(1-{\rho^{\star}}^2)$.
In this model, {which is a subset of a model belonging to the class considered in \textcite{BKW10},} the expectation changes are not abrupt anymore as in Model~\eqref{ar1:eq:modele_new}.

The parameter $\rho$, involved in each term of \eqref{ar1:eq:SSm_def}, is still a problem in order to minimize $SS_m$ with respect to $\rho, \boldsymbol{\delta}$ and $\boldsymbol{t}$. This minimization problem is a complex discrete and global optimization problem. Dynamic Programming \citep{AugerLawrence} cannot be used in this case. Only iterative methods are suitable to this minimization problem, without any guarantee to converge to the global minimum.

However, if $\rho$ is replaced by an estimator $\overline{\rho}_n$, $SS_m (y,\overline{\rho}_n,\boldsymbol{\delta},\boldsymbol{t})$ can be minimized with respect to $\boldsymbol{\delta}$ and $\boldsymbol{t}$ by Dynamic Programming. Proposition \ref{ar1:Prop:Segment2} gives asymptotic results for the estimators resulting from this method.

\begin{prop}\label{ar1:Prop:Segment}
Let $ z = \left(z_0 ,\dots , z_n \right) $ be a finite sequence of real-valued rv's satisfying \eqref{ar1:eq:bkw} and $\left(\overline{\rho}_n\right)$ a sequence of real-valued rv's. Let $\boldsymbol{\widehat{\delta}}_n (z , \overline{\rho}_n)$ and $\boldsymbol{\widehat{t}}_n(z, \overline{\rho}_n)$ be defined by 
%We define:
\begin{eqnarray}
\left(\boldsymbol{\widehat{\delta}}_n(z, \overline{\rho}_n), \boldsymbol{\widehat{t}}_n(z, \overline{\rho}_n)\right) & = & \underset{\left(\boldsymbol{\delta},\boldsymbol{t}\right)\in \mathbb{R}^{m+1}\times \mathcal{A}_{n,m}}{\argmin} SS_m\left(z,\overline{\rho}_n , \boldsymbol{\delta},\boldsymbol{t}\right) \ \textit{,}\label{ar1:eq:delta_n,t_n}\\
\boldsymbol{\widehat{\tau}}_n(z, \overline{\rho}_n) & = & \frac{1}{n} \boldsymbol{\widehat{t}}_n(z, \overline{\rho}_n),\label{ar1:eq:tau_n}
\end{eqnarray}
\noindent where
\begin{equation}\label{ar1:eq:Anm}
\mathcal{A}_{n,m} = \\
\left\lbrace \left(t_0,\dots ,t_{m+1}\right);t_0=0<\dots <t_{m+1}=n, \forall k=1,\dots ,m+1, t_k-t_{k-1}\geq\Delta_n \right\rbrace
\end{equation}
and where $\left(\Delta_n\right)$ is a real sequence such that
{$n^{-1}\Delta_n \underset{n\to\infty}{\longrightarrow} 0$ and $n^{-\alpha}\Delta_n \underset{n\to\infty}{\longrightarrow} +\infty$ with $\alpha>0$.}
Assume that
\begin{equation}\label{ar1:eq:hypRhoRate}
\left(\overline{\rho}_n-\rho^{\star}\right) = O_P\left(n^{-1/2}\right),
\end{equation}
as $n$ tends to infinity. 
Then, 
\begin{equation*}
\| \boldsymbol{\widehat{\tau}}_n(z, \overline{\rho}_n) - \boldsymbol{\tau^{\star}} \| = O_P\left(n^{-1}\right), \qquad \| \boldsymbol{\widehat{\delta}}_n(z, \overline{\rho}_n) - \boldsymbol{\delta^{\star}} \|= O_P\left(n^{-1/2}\right),
\end{equation*}
where $\|\cdot\|$ is the Euclidian norm.\\
The results still hold if the $\epsilon_i$'s are only assumed to be centered and to have a finite second order moment.
\end{prop}

\begin{prop}\label{ar1:Prop:Segment2}
The results of Proposition \ref{ar1:Prop:Segment} still hold under the same assumptions 
when $z$ is replaced with $y$
satisfying \eqref{ar1:eq:modele_new}.

The results still hold if the $\epsilon_i$'s are only assumed to be centered and to have a finite second order moment.
\end{prop}

The proofs of Propositions \ref{ar1:Prop:Segment} and \ref{ar1:Prop:Segment2} are given in Sections \ref{ar1:subsec:prop:Segment} and 
\ref{ar1:subsec:prop:Segment2}, respectively. 
Note that the estimators defined in these propositions have the same asymptotic properties 
as those of the estimators proposed by \textcite{LM}. 
In the Gaussian framework, the estimator $\widetilde{\rho}_n$ defined in Section~\ref{ar1:sec:correlation} satisfies the same properties as $\overline{\rho}_n$ and can thus be used in the criterion $SS_m$ for providing consistent estimators of the change-points and of the means.




%%% Local Variables:
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "article.tex"
%%% ispell-local-dictionary: "en_US"
%%% eval: (flyspell-mode 1)
%%% End: 

==> chapitres/ar1/article/Selection.tex <==
\section{Selecting the number of change-points} \label{ar1:sec:selection}

%\newcommand{\Mcal}{\mathcal{M}}

We now consider the selection of the number of change-points. We first propose a penalized contrast criterion, which we prove to be consistent in the non-Gaussian case. The penalty has a general form, which needs to be specified for a practical use. Therefore, we also derive an adaptation of the modified BIC criterion proposed by \textcite{ZS} in the Gaussian context. This criterion does not rely on any tuning parameter and has been shown to be efficient in practical cases \parencite[see][]{picard2011joint}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Consistent model selection criterion}\label{ar1:subsec:beta}

We propose to select the number of change-points $m$ as follows 
\begin{equation} \label{ar1:Eq:ConsistentCrit}
\widehat{m} = \underset{ 0\leq m \leq m_{\max}}{\argmin} \frac1n SS_m(z, \overline{\rho}_n) + \beta_n m
\end{equation}
where $m_{\max}\geq m^{\star}$, $\left(\beta_n\right)_{n\geq 1}$ is a sequence of positive real numbers, $\overline{\rho}_n$ satisfies the assumptions of Proposition \ref{ar1:Prop:Segment} and
\begin{equation} \label{ar1:Eq:SSm}
SS_m(z, \rho) = \min_{\boldsymbol{\delta}, \boldsymbol{t} \in \mathcal{A}_{n,m}} SS_m(z, \rho, \boldsymbol{\delta}, \boldsymbol{t}) \; ,
\end{equation}
$\mathcal{A}_{n,m}$ being defined in~(\ref{ar1:eq:Anm}).

\begin{prop}\label{ar1:Prop:SelBeta}
Under the assumptions of Proposition \ref{ar1:Prop:Segment},  and if
\begin{eqnarray*}
\beta_n \underset{n\to\infty}{\longrightarrow} 0 , \quad n^{1/2}\beta_n\underset{n\to\infty}{\longrightarrow} +\infty , \quad \Delta_n\beta_n\underset{n\rightarrow\infty}{\longrightarrow} +\infty \; ,
\end{eqnarray*}
where $\Delta_n$ is defined in Proposition \ref{ar1:Prop:Segment}, $\widehat{m}$ defined by \eqref{ar1:Eq:ConsistentCrit} converges in probability to $m^{\star}$.\\
The result still holds if the $\epsilon_i$'s are only assumed to be independent, centered and to have a finite second order moment.
\end{prop}

\begin{prop}\label{ar1:Prop:SelBeta2}
The result of Proposition \ref{ar1:Prop:SelBeta} still holds under the same assumptions 
when $z$ is replaced by $y$ satisfying \eqref{ar1:eq:modele_new}.\\
The result still holds if the $\epsilon_i$'s are only assumed to be independent, centered and to have a finite second order moment.
\end{prop}

The proofs of Propositions \ref{ar1:Prop:SelBeta} and \ref{ar1:Prop:SelBeta2} are given in Sections \ref{ar1:subsec:bicbardet} and \ref{ar1:subsec:mbicbardet_bis}, respectively.

\begin{remark}\label{ar1:remark:forme_beta}
If $\beta_n = n^{-\beta}$, the assumptions of Propositions \ref{ar1:Prop:SelBeta} and \ref{ar1:Prop:SelBeta2} are fulfilled if and only if $0<\beta < \min \left(\alpha , 1/2 \right)$, where $\alpha$ is defined in Proposition \ref{ar1:Prop:Segment}. $\alpha$ stands for the usual bound for the control of the minimal segment length \parencite[see][]{LM}. The $1/2$ bound is the price to pay for the estimation of $\rho^{\star}$.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Modified BIC criterion}
\textcite{ZS} proposed a modified Bayesian information criterion (mBIC) to select the number $m$ of change-points in the particular case of segmentation of an independent Gaussian process $x$. This criterion is defined in a Bayesian context in which a non informative prior is set for the number of segments $m$. 
mBIC is derived from an $O_P(1)$ approximation of the Bayes factor between models with $m$ and $0$ change-points, respectively.
The mBIC selection procedure consists in choosing the number of change-points as:
\begin{equation}\label{ar1:eq:Criterion_formula}
\widehat{m} = \underset{m}{\argmax} C_m(x, 0)
\end{equation}
%
where the criterion $C_m(y, \rho)$ is defined for a process $y$ as
\begin{multline*}
  C_m(y, \rho) = \\
- \frac{n-m+1}{2} \log SS_m(y, \rho) + \log
\Gamma\left(\frac{n-m+1}{2}\right) -\frac{1}{2} \sum_{k=0}^m \log n_k(\boldsymbol{\widehat{t}}(y, \rho)) - m \log n ,
\end{multline*}
where $\Gamma$ is the usual Gamma function. In the latter equation
\begin{equation}\label{ar1:eq:nk}
n_k(\boldsymbol{\widehat{t}}(y, \rho))=\widehat{t}_{k+1}(y, \rho)-\widehat{t}_{k}(y, \rho),
\end{equation}
where $\boldsymbol{\widehat{t}}(y, \rho)=(\widehat{t}_1(y, \rho), \dots, \widehat{t}_m(y, \rho))$ is defined as $\boldsymbol{\widehat{t}}(y, \rho)= \underset{\boldsymbol{t}\in\mathcal{A}_{n,m}}{\argmin} \; \underset{\delta}{\min} \; SS_m(y, \rho, \delta, \boldsymbol{t})$.

Note that, in Model~\eqref{ar1:eq:bkw}, the criterion could be directly applied to the decorrelated series $v^{\star} = \left(v^{\star}_i\right)_{1\leq i\leq n} = \left(y_i - \rho^{\star} y_{i-1}\right)_{1\leq i\leq n}$ since
$$
C_m(y, \rho^{\star}) = C_m(v^{\star}, 0).
$$ 
We propose to use the same selection criterion, replacing $\rho^{\star}$ by some relevant estimator $\overline{\rho}_n$. 
The following two propositions show that this plug-in approach result in the same asymptotic properties under both Model \eqref{ar1:eq:bkw} and \eqref{ar1:eq:modele_new}. 

\begin{prop} \label{ar1:Prop:mBICBardet}
For any positive $m$, for a process $z$ satisfying \eqref{ar1:eq:bkw} and under the assumptions of Proposition \ref{ar1:Prop:Segment}, we have
\begin{eqnarray*}
C_m(z, \overline{\rho}_n) & = & C_m(z, \rho^{\star}) + O_P(1),\textrm{ as } n\to\infty\;.
\end{eqnarray*}
\end{prop}

\begin{prop} \label{ar1:Prop:mBIC}
For any positive $m$, for a process $y$ satisfying \eqref{ar1:eq:modele_new} and under the assumptions of Proposition \ref{ar1:Prop:Segment2} , we have
\begin{eqnarray*}
C_m(y, \overline{\rho}_n) & = & C_m(y, \rho^{\star}) + O_P(1),\textrm{ as } n\to\infty\;.
\end{eqnarray*}
\end{prop}

The proofs of Propositions \ref{ar1:Prop:mBICBardet} and \ref{ar1:Prop:mBIC} are given in Sections \ref{ar1:proof:Prop:mBICBardet} and \ref{ar1:proof:Prop:mBIC} respectively.

In practice, we propose to take $\overline{\rho}_n = \widetilde{\rho}_n$ 
which satisfies the condition of Proposition \ref{ar1:Prop:mBIC} 
to estimate the number of segments by
\begin{eqnarray} \label{ar1:Eq:BIC}
\widehat{m} & = & \argmax_m \left[- \left(\frac{n-m+1}{2} \right) \log SS_m(y, \widetilde{\rho}_n) + \log
\Gamma\left(\frac{n-m+1}{2}\right) \right. \nonumber \\
  & & \left. -\frac{1}{2} \sum_{k=0}^m \log n_k(\boldsymbol{\widehat{t}}(y, \widetilde{\rho}_n)) - m \log n \right],
\end{eqnarray}
where $SS_m(\cdot,\cdot)$ and $n_k(\cdot,\cdot)$ are defined in \eqref{ar1:Eq:SSm} and \eqref{ar1:eq:nk}, respectively.

\begin{remark}
Since the definition of the original mBIC criterion is intrinsically related to normality, we did not study precisely the quality of our approximation without the normality assumption.
\end{remark}

%%% Local Variables:
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "article.tex"
%%% ispell-local-dictionary: "en_US"
%%% eval: (flyspell-mode 1)
%%% End: 

==> chapitres/ar1/article/Simul.tex <==
\section{Numerical experiments}\label{ar1:sec:simul}

\subsection{Practical implementation}\label{ar1:sec:post-proc}

Our decorrelation procedure introduces spurious change-points in the
series, at distance $1$ of the true change-points (see Figure
\ref{ar1:fig:exp_vs_exp_diff}, top). Since these artefacts may affect
our procedure, we propose a post-processing to the estimated
change-points $\boldsymbol{\widehat{t}_n}$, which consists in
removing segments of length 1:
\begin{equation*}%\label{ar1:eq:PT}
PP\left( \boldsymbol{\widehat{t}}_n \right) = \left\lbrace \widehat{t}_{n,k}\in \boldsymbol{\widehat{t}}_n \right\rbrace \setminus \left\lbrace \widehat{t}_{n,i} \textit{ such that } \widehat{t}_{n,i} = \widehat{t}_{n,i-1} +1 \textit{ and } \widehat{t}_{n,i+1} \neq \widehat{t}_{n,i} +1 \right\rbrace \; .
\end{equation*}
This post-processing results in a smaller number of change-points. Figure \ref{ar1:fig:exp_vs_exp_diff} summarizes the whole processing.

\begin{figure}
\centering
\includegraphics[width=.75\textwidth]{pp.pdf}
\caption[Post-traitement des instants de rupture estimés, cas AR(1).]{\footnotesize{Top left: a series around two changes, with $\rho^{\star}=0.5$. Top right: the decorrelated series in the same region. Bottom left: before post-processing, two pairs of adjacent change-points are found. Bottom right: post-processing removes the last change-point of each pair of adjacent ones.}}
\label{ar1:fig:exp_vs_exp_diff}
\end{figure}

In practice, it may also be useful to have some guidance on how to check that the assumptions underpinning our approach are satisfied for a given data set. A possible approach is to subtract the estimated piecewise constant function from the original series. If the model is the expected one, this new series should be a realization of an AR(1) Gaussian process. Hence, the residuals built by decorrelation of this series should be Gaussian and independent. One way to check this is to perform a gaussianity test and a Portmanteau test on this series of residuals.

\subsection{Simulation design}\label{ar1:sec:design}

To assess the performance of the proposed method, we used a
simulation design inspired from the one conceived by \textcite{simul}.
We considered series of length $n \in \{100, 200, 400, 800, 1600\}$
with autocorrelation at lag 1, denoted by $\rho^{\star}$, ranging from
$-.9$ to $.9$~(by steps of $.1$) and residual standard deviation
$\sigma^{\star}$ between $.1$ and $.6$~(by steps of $.1$). All series were
affected by $m^{\star} = 6$ change-points located at
fractions $1/6 \pm 1/36, 3/6 \pm 2/36, 5/6 \pm 3/36$
of their length. Each combination was replicated $S=100$ times.
The mean within each segment alternates between 0 and 1, starting with $\mu_1 = 0$.

\paragraph{\textbf{Estimation of $\rho^{\star}$.}}

For each generated series, two different estimates $\overline{\rho}_n$ of $\rho^{\star}$ were computed: the original estimate $\overline{\rho}_n = \widehat{\rho}_{\textrm{MG}}$ proposed by \textcite{MG} and our revised version $\overline{\rho}_n = \widetilde{\rho}_n$.
We carried the same study on series with no change-point (centered series).

\paragraph{\textbf{Estimation of the segmentation parameters.}}

For each generated series, we estimated the change-point locations
$\widehat{\boldsymbol{\tau}}_n(y,
\overline{\rho}_n)$ using Proposition \ref{ar1:Prop:Segment} for each
$m$ from $1$ to $m_{\max} =75$ and with different choices of $\overline{\rho}_n$:
$\widetilde{\rho}_n$ (our estimator), $\rho^{\star}$ (the true value) and
zero (which does not take into account for the autocorrelation). For
each choice of $\overline{\rho}_n$, we then selected the number of
change-points $\hat{m}$ using \eqref{ar1:Eq:BIC}. Actually, the last
choice $\overline{\rho}_n=0$ corresponds to the classical
least-squares framework. In addition, we shall also use the
post-processing described in Section \ref{ar1:sec:post-proc} for the
cases where $\overline{\rho}_n=\widetilde{\rho}_n$ and $\rho^{\star}$.

To study the quality of the proposed model
selection criterion, we computed the distribution of $\widehat{m}$
for each estimate $\overline{\rho}_n \in \{\widetilde{\rho}_n,
\rho^{\star}, 0\}$ with post-processing or not for the first two estimates
of $\rho^{\star}$.

In order to assess the performance of the estimation of the
change-point locations,  we computed the Hausdorff distance defined
in the segmentation framework as follows, see \textcites{boysen:2009}{harchaoui2010}:

% \Sr{
% d\left(\boldsymbol{\tau^{\star}} ,\boldsymbol{\overline{\tau}_n}\right) = \max\left(d_1 \left(\boldsymbol{\tau^{\star}} ,\boldsymbol{\overline{\tau}_n}\right),\overline{\mathcal{T}}_n), d_2 \left(\boldsymbol{\tau^{\star}} ,\boldsymbol{\overline{\tau}_n}\right)\right)\;,
% }{

\begin{equation}\label{ar1:eq:hausdorff}
d\left(\boldsymbol{\tau}^{\star} , \widehat{\boldsymbol{\tau}}_n\left(y,
\overline{\rho}_n\right)\right) = \max\left( d_1
\left(\boldsymbol{\tau}^{\star}, \widehat{\boldsymbol{\tau}}_n\left(y,
\overline{\rho}_n\right)\right),d_2 \left(\boldsymbol{\tau}^{\star},
\widehat{\boldsymbol{\tau}}_n\left(y, \overline{\rho}_n\right)\right)\right)\;,
\end{equation}
where
\begin{eqnarray}
d_1 \left(\boldsymbol{a},\boldsymbol{b}\right) & = & \underset{b\in\boldsymbol{b}}{\sup}
\underset{a\in\boldsymbol{a}}{\inf} \left\vert a - b \right\vert
\label{ar1:eq:hausd_1},  \\
 \text{and \qquad} d_2
\left(\boldsymbol{a},\boldsymbol{b}\right) & = & d_1
\left(\boldsymbol{b},\boldsymbol{a}\right).\label{ar1:eq:hausd_2}
\end{eqnarray}
$d_1$ close to zero means that an estimated change-point is likely to be close to a true change-point. A small value of $d_2$ means that a true change-point is likely to be close to each estimated change-point. A perfect segmentation results in both null $d_1$ and $d_2$. Over-segmentation results in a small $d_1$ and a large $d_2$. Under-segmentation results in a large $d_1$ and a small $d_2$, provided that the estimated change-points are correctly located.

\subsection{Results}

\paragraph{\textbf{Estimation of $\rho^{\star}$.}}

In Figure \ref{ar1:fig:rho_no_break}, we compare the performance of our
robust estimator of $\rho^{\star}$: $\widetilde{\rho}_n$ with the ones of
the estimator $\widehat{\rho}_{\textrm{MG}}$ in the case where there
are no change-points in the observations. More precisely, in
this case, the observations $y$ are generated under the
Model~\eqref{ar1:eq:modele_new} with $\mu_k^{\star}=0$, for all $k$.  We
observe that the estimator proposed by \mbox{\textcite{MG}} performs better than our robust estimator.
However, it is not the case anymore in the presence of change-points
in the data as we can see in Figure \ref{ar1:fig:rho_with_break}. In the
latter case, our robust estimator $\widetilde{\rho}_n$ outperforms
the estimator $\widehat{\rho}_{\textrm{MG}}$ for almost all values
of $\rho^{\star}$.

\begin{figure}[!h]
\centering
%\begin{minipage}[t]{7.5cm}
%\centering
\includegraphics[width=0.7\textwidth]{Boxplot-rho-centered-sigma_02_06-n_400_1600.pdf}
\caption[Boîtes à moustaches de $\widetilde{\rho}_n-\rho^{\star}$ et de $\widehat{\rho}_{\textrm{MG}}-\rho^{\star}$, sans ruptures dans la série.]{\footnotesize{Boxplots of
$\widehat{\rho}_{\textrm{MG}}-\rho^{\star}$ in red and
$\widetilde{\rho}_n-\rho^{\star}$ in black for different values of
$\rho^{\star}$ in the case where there are no change-points in the data
with $n=400$ (plots on the left), $n=1600$ (plots on the right),
$\sigma^{\star}=0.2$ (top) and $\sigma^{\star}=0.6$ (bottom).}}
\label{ar1:fig:rho_no_break}
\end{figure}
%\end{minipage}
%\hspace{3mm}
%\begin{minipage}[t]{7.5cm}
\begin{figure}[!h]
\centering
\includegraphics[width=0.7\textwidth]{Boxplot-rho-biased-sigma_02_06-n_400_1600.pdf}
\caption[Boîtes à moustaches de $\widetilde{\rho}_n-\rho^{\star}$ et de $\widehat{\rho}_{\textrm{MG}}-\rho^{\star}$, avec ruptures dans la série.]{\footnotesize{Boxplots of
$\widehat{\rho}_{\textrm{MG}}-\rho^{\star}$ in red and
$\widetilde{\rho}_n-\rho^{\star}$ in black for different values of
$\rho^{\star}$ in the case where there are change-points in the data with
$n=400$ (plots on the left), $n=1600$ (plots on the right),
$\sigma^{\star}=0.2$ (top) and $\sigma^{\star}=0.6$ (bottom).}}
\label{ar1:fig:rho_with_break}
%\end{minipage}
\end{figure}


\paragraph{\textbf{Model selection.}}

In Figures \ref{ar1:fig:Kchap_sig01} and \ref{ar1:fig:Kchap_sig05}, we
compare the estimated number of change-points $\widehat{m}$ in
two different configurations of signal-to-noise ratio
($\sigma^{\star}=0.1$ and $\sigma^{\star}=0.5$) and with three different values
of $\rho^{\star}$ ($\rho^{\star}=0.3$, $0.6$ and $0.8$). In these figures, the
notation LS, Robust and Oracle correspond to the cases where
$\overline{\rho}_n=0$, $\overline{\rho}_n=\tilde{\rho}_n$ and
$\overline{\rho}_n=\rho^{\star}$, respectively. Moreover, we use the
notation -P when the post-processing described in Section~\ref{ar1:sec:post-proc} is used. In the situations where $\sigma^{\star}$ and
$\rho^{\star}$ are small, all the methods provide an accurate estimation
of the number of change-points. In the other cases,
LS tends to strongly overestimate the number of change-points.
Robust and Oracle tend to select twice the true number of change-points due to the artifactual
presence of change-points in the decorrelated series as explained in Section~\ref{ar1:sec:post-proc}. This is corrected by the post-processing and Robust-P provides the correct number of change-points in most of the considered configurations.
Moreover, we also observe that the performance of Robust and
Robust-P are similar to these of Oracle and Oracle-P: the robust
decorrelation procedure we propose performs as well as if $\rho^{\star}$
was known for $n=1600$. It has to be noted that the post-processing would not
improve the performance on LS {so we did not considered it}.

\begin{figure}[!h]
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_Kchap-n1600-sigma01-rho03.pdf}
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_Kchap-n1600-sigma01-rho06.pdf}
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_Kchap-n1600-sigma01-rho08.pdf}
\caption[Boîtes à moustaches du nombre estimé de ruptures, $\sigma^{\star}=0.1$.]{\footnotesize{Boxplots for the estimated number of change-points for $n=1600$ when $\overline{\rho}_n=0$ (LS), $\overline{\rho}_n=\tilde{\rho}_n$ (Robust and
Robust-P with post-processing) and $\overline{\rho}_n=\rho^{\star}$ (Oracle and Oracle-P with post-processing)
with $\sigma^{\star}=0.1$ and $\rho^{\star}=0.3$ (left),  $\rho^{\star}=0.6$ (middle) and $\rho^{\star}=0.8$ (right). The true number of change-points is equal to 6 (red horizontal line).}}
\label{ar1:fig:Kchap_sig01}
\end{figure}

\begin{figure}[!h]
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_Kchap-n1600-sigma05-rho03.pdf}
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_Kchap-n1600-sigma05-rho06.pdf}
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_Kchap-n1600-sigma05-rho08.pdf}
\caption[Boîtes à moustaches du nombre estimé de ruptures, $\sigma^{\star}=0.5$.]{\footnotesize{Boxplots for the estimated number of change-points for $n=1600$ when $\overline{\rho}_n=0$ (LS), $\overline{\rho}_n=\tilde{\rho}_n$ (Robust and
Robust-P with post-processing) and $\overline{\rho}_n=\rho^{\star}$ (Oracle and Oracle-P with post-processing)
with $\sigma^{\star}=0.5$ and $\rho^{\star}=0.3$ (left),  $\rho^{\star}=0.3$ (middle) and $\rho^{\star}=0.8$ (right). The true number of change-points is equal to 6 (red horizontal line).}}
\label{ar1:fig:Kchap_sig05}
\end{figure}

\paragraph{\textbf{Change-point locations.}}
%
In Figures \ref{ar1:fig:hausd_1_sig05} and \ref{ar1:fig:hausd_2_sig05} are
displayed the boxplots of the two parts $d_1$ and
$d_2$ of the Hausdorff distance
defined in (\ref{ar1:eq:hausd_1}) and (\ref{ar1:eq:hausd_2}), respectively for different values of $\rho^{\star}$ when
$\sigma^{\star}=0.5$. $d_2$ is displayed in Figure \ref{ar1:fig:hausd_2_sig01} for $\sigma^{\star}=0.1$; for this value of
$\sigma^{\star}$, $d_1$ was found null for all methods and all values of $\rho^{\star}$.


When the noise is small ($\sigma^{\star} = 0.1$), the robust procedure we propose performs well for the whole range of correlation. On the contrary, the performance of LS are deprecated when the correlation increases, whereas these of LS$^{\star}$ still provide accurate change-point locations. This shows that the least-square approach only fails because it turns to overestimate the number of change-points. %\\
This is all the more true for LS when the variance of the noise is
large~($\sigma^{\star} = 0.5$). When the problem
gets difficult~(both $\sigma^{\star}$ and $\rho^{\star}$ large), our robust
procedure tends to underestimate the number of
change-points~(which was expected) and the
estimated change-points are close to true ones.

\begin{figure}[!h]
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_hausdorff_One-n1600-sigma05-rho03.pdf}
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_hausdorff_One-n1600-sigma05-rho06.pdf}
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_hausdorff_One-n1600-sigma05-rho08.pdf}
\caption[Boîtes à moustaches de la première partie de la distance de Hausdorff, $\sigma^{\star}=0.5$.]{\footnotesize{Boxplots for the first part of the Hausdorff distance ($d_1$)  for $n=1600$ when $\overline{\rho}_n=0$ (LS and LS* when the true number of
change-points is known), $\overline{\rho}_n=\tilde{\rho}_n$ (Robust and
Robust-P with post-processing) and $\overline{\rho}_n=\rho^{\star}$ (Oracle and Oracle-P with post-processing)
with $\sigma^{\star}=0.5$ and $\rho^{\star}=0.3$ (left),  $\rho^{\star}=0.6$ (middle) and $\rho^{\star}=0.8$ (right).}}
\label{ar1:fig:hausd_1_sig05}
\end{figure}


\begin{figure}[!h]
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_hausdorff_Two-n1600-sigma01-rho03.pdf}
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_hausdorff_Two-n1600-sigma01-rho06.pdf}
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_hausdorff_Two-n1600-sigma01-rho08.pdf}
\caption[Boîtes à moustaches de la seconde partie de la distance de Hausdorff, $\sigma^{\star}=0.1$.]{\footnotesize{Boxplots for the second part of the Hausdorff distance ($d_2$) for $n=1600$ when $\overline{\rho}_n=0$ (LS and LS* when the true number of
change-points is known), $\overline{\rho}_n=\tilde{\rho}_n$ (Robust and
Robust-P with post-processing) and $\overline{\rho}_n=\rho^{\star}$ (Oracle and Oracle-P with post-processing)
with $\sigma^{\star}=0.1$ and $\rho^{\star}=0.3$ (left),  $\rho^{\star}=0.6$ (middle) and $\rho^{\star}=0.8$ (right).}}
\label{ar1:fig:hausd_2_sig01}
\end{figure}

\begin{figure}[!h]
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_hausdorff_Two-n1600-sigma05-rho03.pdf}
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_hausdorff_Two-n1600-sigma05-rho06.pdf}
\includegraphics[width=0.32\textwidth,height=5cm]{boxplot_hausdorff_Two-n1600-sigma05-rho08.pdf}
\caption[Boîtes à moustaches de la seconde partie de la distance de Hausdorff, $\sigma^{\star}=0.5$.]{\footnotesize{Boxplots for the second part of the Hausdorff distance ($d_2$) when $\overline{\rho}_n=0$ (LS and LS* when the true number of
change-points is known), $\overline{\rho}_n=\tilde{\rho}_n$ (Robust and
Robust-P with post-processing) and $\overline{\rho}_n=\rho^{\star}$ (Oracle and Oracle-P with post-processing)
with $\sigma^{\star}=0.5$ and $\rho^{\star}=0.3$ (left),  $\rho^{\star}=0.6$ (middle) and $\rho^{\star}=0.8$ (right).}}
\label{ar1:fig:hausd_2_sig05}
\end{figure}

An other way to illustrate the performance of the estimation of the change-point locations is the histograms of these estimates. We provide these plots only for LS, Robust-P and Oracle-P, because Post-processing does not change significantly LS estimates, and, furthermore, Robust (respectively Oracle) method's histograms with or without Post-Processing are very similar, see Figures \ref{ar1:fig:densplot1} and \ref{ar1:fig:densplot5}. These figures illustrate that in case of over-estimation of the number of changes by LS method, the additional change-points seem to be uniformly distributed.

\begin{figure}[!h]
\centering
\includegraphics[width=0.9\textwidth,height=6cm]{aggregation_n_1600_sigma_1.pdf}
\caption[Fréquence des instants de rupture estimés, $\sigma^{\star}=0.1$.]{\footnotesize{Frequencies of each possible change-point estimator, with $\sigma^{\star}=0.1$ and $n=1600$. Tick-marks on bottom-side axis represent the true change-point locations. $\overline{\rho}_n=0$ (LS, top line), $\overline{\rho}_n=\tilde{\rho}_n$ (Robust-P, middle line) and $\overline{\rho}_n=\rho^{\star}$ (Oracle-P, bottom line) with $\rho^{\star}=0.3$ (left),  $\rho^{\star}=0.6$ (middle) and $\rho^{\star}=0.8$ (right).}}
\label{ar1:fig:densplot1}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=0.9\textwidth,height=6cm]{aggregation_n_1600_sigma_5.pdf}
\caption[Fréquence des instants de rupture estimés, $\sigma^{\star}=0.5$.]{\footnotesize{Frequencies of each possible change-point estimator, with $\sigma^{\star}=0.5$ and $n=1600$. Tick-marks on bottom-side axis represent the true change-point locations.$\overline{\rho}_n=0$ (LS, top line), $\overline{\rho}_n=\tilde{\rho}_n$ (Robust-P, middle line) and $\overline{\rho}_n=\rho^{\star}$ (Oracle-P, bottom line) with $\rho^{\star}=0.3$ (left),  $\rho^{\star}=0.6$ (middle) and $\rho^{\star}=0.8$ (right).}}
\label{ar1:fig:densplot5}
\end{figure}

\subsection{Additional simulation studies}\label{ar1:sec:add_simul}
\subsubsection{Comparison with \textcite{BKW10}}
The quasi-maximum likelihood method proposed by \mbox{\textcite{BKW10}}, when applied to a Gaussian AR(1) process with changes in the mean $\left(y_0,\dots ,y_n\right)$ , consists in the minimization with respect to $\boldsymbol{\rho}=\left(\rho_0,\dots ,\rho_m\right), \boldsymbol{\sigma}=\left(\sigma_0,\dots ,\sigma_m\right), \boldsymbol{\delta}=\left(\delta_0,\dots ,\delta_m\right)$ and $\boldsymbol{t}=\left(t_0,\dots ,t_m\right)$ of the following function:
\begin{equation}\label{ar1:eq:bardetFunc}
\left(\boldsymbol{\rho}, \boldsymbol{\sigma} , \boldsymbol{\delta},\boldsymbol{t}\right) \mapsto \sum_{k=0}^m \left\lbrace \left(t_{k+1}-t_k\right)\log\left(\sigma_k^2\right)+\frac{1}{\sigma_k^2}\sum_{i=t_k +1}^{t_{k+1}}\left(y_i-\rho_k y_{i-1}- \delta_k\right)^2 \right\rbrace \; .
\end{equation}
Indeed, in the class of models considered in \textcite{BKW10}, changes in all the parameters are possible at each change-point. Using this method to estimate the change-point locations for data satisfying Model~\eqref{ar1:eq:modele_new} or~\eqref{ar1:eq:bkw} boils down to ignore the stationarity of $\left(\eta_i\right)_{i\geq 0}$ as defined in~\eqref{ar1:eq:ar1}. It can lead to a poor estimation of change-point locations, especially when there are many changes close to each other.
To illustrate this fact, we compared our estimator of change-point locations to the estimates given by the minimization of~\eqref{ar1:eq:bardetFunc}. We generated $100$ series of length $400$, under Model~\eqref{ar1:eq:modele_new}, with $\rho^{\star}=0.3$ and $\sigma^{\star}=0.4$. The number of change-points, their locations and the means within segments are the same as in Section~\ref{ar1:sec:design}. The number of changes is assumed to be known and we did not post-process the estimates. Simulations show that using the method of \textcite{BKW10} in this case can lead to a poor estimation of close change-points, while our method is less affected by the length of segments (see Figure~\ref{ar1:fig:BardetVsUs}). For example, the boundaries of the smallest segment are recovered in less than half of the simulations when minimizing~\eqref{ar1:eq:bardetFunc}.
\begin{figure}
\centering
\includegraphics[width=.45\textwidth]{PlotBardet.pdf}
\includegraphics[width=.45\textwidth]{PlotNous.pdf}
\caption[Fréquence des instants de rupture estimés, comparaison avec \textcite{BKW10}.]{\footnotesize{Frequencies of each possible change-point location estimate. Tick-marks on bottom-side axis represent the true change-point locations. Left: Estimation by the minimization of \eqref{ar1:eq:bardetFunc}. Right: Our method.}} \label{ar1:fig:BardetVsUs}
\end{figure}
\subsubsection{Robustness to model mis-specification}\label{ar1:sec:AR2} 
In this section, we study the
behaviour of our proposed robust procedure~(Robust-P) 
%faced to a situation 
when the signal is corrupted by an AR(2) Gaussian
process, e.g. in Model~\ref{ar1:eq:modele_new}, $\eta_i$ is a zero-mean
stationary process such that
$$
\eta_i = \phi_1^{\star} \eta_{i-1}+\phi_2^{\star} \eta_{i-2}+ \varepsilon_i ,
$$
where $\vert \phi_2 \vert < 1$, $\phi_1+\phi_2<1$ and
$\phi_2-\phi_1<1$. We considered series of fixed length $n=1600$, a
residual standard deviation $\sigma^{\star}=0.1$, $\phi_1^{\star}=0.3$ and
$\phi_2^{\star}$ in $\{-0.9,-0.8,-0.7,\dots,0.5,0.6\}$ 
%and $0.6$ (by steps of $0.1$) 
%to ensure the previous conditions. 
We used the same segmentation design as in
Subsection~\ref{ar1:sec:post-proc}. Each combination was
replicated $100$ times. All the results are
displayed in Figure \ref{ar1:fig:K-rho-h1-h2-AR2}.

The procedure performs well when $\phi_2^{\star}$ belongs to the interval
$[-0.5,0.2]$ as expected (similar to the case of AR(1)): the
estimated segmentation is close to the true one. When
$\phi_2^{\star}>0.2$, it tends to over-estimate the number of
change-points. The true change-points are detected ($d_1$ is close
to zero, e.g. the decorrelation procedure with the obtained negative
estimation of ${\rho}^{\star}$ leads to an increasing in the mean
differences) but false change-points are added (large $d_2$). When
$\phi_2^{\star}<-0.5$, under-segmentation is observed: the decorrelation
procedure with a large estimated value of ${\rho}^{\star}$ leads to a
difficult segmentation problem.

\begin{figure}
\centering
\includegraphics[width=.32\textwidth, height=0.2\textheight]{Nbrupt.pdf}
\includegraphics[width=.32\textwidth, height=0.2\textheight]{h1.pdf}
\includegraphics[width=.32\textwidth, height=0.2\textheight]{h2.pdf}
\caption[Résultats de la méthode pour l'AR(1) dans le cas d'un bruit AR(2).]{\footnotesize{Left: Boxplots for the estimated number
of change-points. 
%Top right: boxplots of $\tilde{\rho}_{n}$. 
Center and right: Boxplots for the first part of the Hausdorff distance ($d_1$) and for the second part of the Hausdorff distance ($d_2$) with $n=1600$, $\sigma^{\star}=0.1$ and $\phi_1^{\star}=0.3$ with respect to different values of $\phi_2^{\star}$.}} \label{ar1:fig:K-rho-h1-h2-AR2}
\end{figure}

\subsubsection{Estimator of $\rho^{\star}$ in the case of the Cauchy distribution}
In Section \ref{ar1:sec:correlation}, an analogous estimator of $\rho^{\star}$ in the case of Cauchy distributed observations is proposed. 
We follow the simulation design described in Subsection \ref{ar1:sec:design}, where the Gaussian rv's are replaced by
Cauchy rv's. More precisely, the expectation parameters are replaced by the location parameters of the Cauchy 
distribution and $\sigma^{\star}$ is replaced by the scale parameter of the Cauchy distribution. We can see from Figure \ref{ar1:fig:Cauchy} that $\widetilde{\widetilde{\rho}}_n$ is an accurate estimator of $\rho^{\star}$ except when $\rho^{\star}$ is close to zero.
%
\begin{figure}
\centering
\includegraphics[width=.4\textwidth]{Cauchy.pdf}
\caption[Boîtes à moustaches pour l'estimateur de l'autocorrélation à l'ordre 1, cas de la loi de Cauchy.]{\footnotesize{Boxplots of $\widetilde{\widetilde{\rho}}_n-\rho^{\star}$ for different values of $\rho^{\star}$  
when $n=1600$ and $\sigma^{\star}=0.1$.}} \label{ar1:fig:Cauchy}
\end{figure}
%
When this estimator of $\rho^{\star}$ is used in our change-point estimation method, it leads to poor estimations of the change-points
since the Cauchy distribution does not have finite second order moment (simulations not shown).
%%% Local Variables:
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "article.tex"
%%% ispell-local-dictionary: "en_US"
%%% eval: (flyspell-mode 1)
%%% End:


==> chapitres/arp/Abstractfr.tex <==
\vspace{-0.2cm}
Le problème qui nous intéresse est celui de l'estimation de ruptures multiples dans l'espérance d'un processus AR(p).  La prise en compte de la structure de dépendance nous interdit l'approche inférentielle du cas indépendant. En particulier, l'algorithme de programmation dynamique, qui est le seul algorithme permettant de calculer la segmentation optimale dans le cas indépendant, ne peut plus être utilisé. Nous proposons une méthode en deux étapes, basée sur l'estimation préliminaire des paramètres d'autorégression. Cette dernière est basée sur des techniques de statistique robuste car notre estimateur doit être robuste aux ruptures si nous souhaitons ne pas avoir à les estimer en premier lieu. Nous proposons alors de suivre l'approche inférentielle classique en injectant cet estimateur dans le critère utilisé pour l'estimation de la localisation des ruptures, ce qui est équivalent à décorréler la série à l'aide des paramètres d'autorégression estimés. Nous démontrons que ces estimateurs des instants de rupture et des espérances partagent les propriétés asymptotiques des estimateurs classiques dans le cadre indépendant. La même approche \emph{plug-in} est alors utilisée pour approcher le critère BIC modifié, sélectionner le nombre de segments et pour proposer un critère BIC heuristique pour sélectionner simultanément le nombre de ruptures et l'ordre de l'autorégression. Finalement, nous montrons, dans la section simulations, que pour des séries de taille finie la prise en compte de la structure de dépendance améliore les performances statistiques des estimateurs des lieux de rupture et du nombre de ruptures sélectionné.

==> chapitres/arp/AppSec4.tex <==
\subsection{Proof of Proposition \ref{Prop:mBICBardet}}

We first give some lemmas which are useful for the proof of Proposition \ref{Prop:mBICBardet}.

\begin{lemma} \label{Lem:SSm} Under the assumptions of 
Proposition \ref{Prop:mBICBardet} with $SS_m$ given by \eqref{Eq:SSm}, we have, for any positive $m$,
$$
SS_m(z, \overline{\rho}_n) = SS_m(z, \rho^*) + O_P(1),\textrm{ as } n\to\infty\;.
$$
\end{lemma}

\begin{lemma} \label{Lem:SSmstar} Under the assumptions of Proposition
\ref{Prop:mBICBardet} with $SS_m$ given by \eqref{Eq:SSm}, we have,
for any positive $m$,
$$
SS_m(z, \rho^*)^{-1} = O_P(n^{-1}),\textrm{ as } n\to\infty\;.
$$
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{proof}[Proof of Lemma \ref{Lem:SSm}]
 The proof of this Lemma follows exactly this of Lemma \ref{Lem:SSmY}. The difference is that, in \eqref{eq:bkw}, the term $\Delta^*$ appearing in the decomposition \eqref{eq:dec:second:terme} vanishes.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{proof}[Proof of Lemma \ref{Lem:SSmstar}]
We first define 
$$
SS_m \left(z, \rho, \boldsymbol{t}\right) = \underset{\delta}{\argmin } SS_m \left(z, \rho, \delta, \boldsymbol{t} \right).
$$ 
We have, for any positive $M$, 
\begin{eqnarray*}
 P\left(\frac{n}{SS_m(z, \rho^*)} > M \right) 
 & \leq & P\left( \left\{\frac{SS_m(z, \rho^*)}{SS_m(z, \rho^*, \boldsymbol{t^*})} > 1 \right\} \bigcap \left\{\frac{n}{SS_m(z, \rho^*)} > M\right\} \right) \\
  & & + P\left( \left\{\frac{SS_m(z, \rho^*)}{SS_m(z, \rho^*, \boldsymbol{t^*})} < 1 \right\} \bigcap \left\{\frac{n}{SS_m(z, \rho^*)} > M\right\} \right) \\
  & \leq & P\left(\frac{n}{SS_m(z, \rho^*, \boldsymbol{t^*})} > M \right) + P\left(\frac{SS_m(z, \rho^*)}{SS_m(z, \rho^*, \boldsymbol{t^*})} < 1 \right).
\end{eqnarray*}
Under the assumptions of Proposition \ref{Prop:Segment}, a by product of the proof of Theorem 3 in \textcite{LM} is that
$$
P\left(\frac{SS_m(z, \rho^*)}{SS_m(z, \rho^*, \boldsymbol{t^*})} < 1 \right) = P\left(SS_m(z, \rho^*) - SS_m(z, \rho^*, \boldsymbol{t^*}) < 0 \right) 
\leq \kappa n^{-\alpha},
$$
where $\kappa$ is a positive constant depending on $\boldsymbol{\delta^*}$ and $\boldsymbol{t^*}$, and $\alpha$ is a positive constant. 
Furthermore, as $\sigma^{*-2}SS_m(z, \rho^*, \boldsymbol{t^*})$ has a $\chi^2_{n-m-1}$ distribution, 
$n^{-1}SS_m(z, \rho^*, \boldsymbol{t^*})=\sigma^{*2}+o_P(1)$ and thus {$n^{-1} SS_m(z, \rho^*, \boldsymbol{t^*})=O_P(1)$}, which concludes the proof.
\end{proof}

\begin{proof}[Proof of Proposition \ref{Prop:mBICBardet}]
We have to prove that, for a given positive $m$, $C_m(z, \rho^*) - C_m(z, \overline{\rho}_n) = O_P(1)$. 
Observe that, since $\widehat{\tau}_k(z, \rho) = \widehat{t}_k(z, \rho) /n$, 
\begin{eqnarray} \label{Eq:DecompNkZ}
& & \sum_{k=0}^m \log n_k(\widehat{t}(z, \overline{\rho}_n)) - \sum_{k=0}^m \log
n_k(\widehat{t}(z, {\rho}^*)) \nonumber \\
& = & \sum_{k=0}^m \log (\widehat{\tau}_{k+1}(z, \overline{\rho}_n)-\widehat{\tau}_{k}(z, \overline{\rho}_n))- 
\sum_{k=0}^m \log (\widehat{\tau}_{k+1}(z, {\rho}^*)-\widehat{\tau}_{k}(z, {\rho}^*)).
\end{eqnarray}
By Proposition  \ref{Prop:Segment}, both quantities of the previous equation converge in probability
to $$\sum_{k=0}^m \log (\tau^*_{k+1}-\tau^*_{k}) \,$$
thus
\begin{equation} \label{Eq:CvgceNkZ}
\sum_{k=0}^m \log n_k(\widehat{t}(z, \overline{\rho}_n))- \sum_{k=0}^m \log
n_k(\widehat{t}(z, {\rho}^*))=O_P(1). 
\end{equation}
Further note that
$$
\log {SS}_m(z, \overline{\rho}_n) - \log {SS}_m(z, {\rho}^*)
=\log\left(\frac{{SS}_m(z, \overline{\rho}_n)}{{SS}_m(z, {\rho}^*)}\right) 
= R\left(\frac{{SS}_m(z, \overline{\rho}_n)-{SS}_m(z, {\rho}^*)}{{SS}_m(z, {\rho}^*)}\right),
$$
where $R(x)=\log(1+x)$.
Lemma \ref{Lem:SSm} states that ${SS}_m(z, \overline{\rho}_n)-{SS}_m(z, {\rho}^*) = O_P(1)$ and Lemma \ref{Lem:SSmstar} that $[{SS}_m(z, {\rho}^*)]^{-1} = O_P(n^{-1})$ so, by \cite[Lemma 2.12]{van}, we get that
$$
\log {SS}_m(z, \overline{\rho}_n) - \log {SS}_m(z, {\rho}^*)
= O_P(n^{-1}).
$$
Hence
$$
\frac{n-m+1}{2} \log {SS}_m(z, \overline{\rho}_n) - \frac{n-m+1}{2} \log {SS}_m(z, {\rho}^*) =
O_P(1),
$$
which with (\ref{Eq:CvgceNkZ}) concludes the proof of Proposition \ref{Prop:mBICBardet}.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Proposition \ref{Prop:mBIC}}
We first give some lemmas which are useful for the proof of Proposition \ref{Prop:mBIC}.

\begin{lemma} \label{Lem:SSmY} Under the assumptions of 
Proposition \ref{Prop:mBICBardet} with $SS_m$ given by \eqref{Eq:SSm}, we have, for any positive $m$,
$$
SS_m(y, \overline{\rho}_n) = SS_m(y, \rho^*) + O_P(1),\textrm{ as } n\to\infty\;.
$$
\end{lemma}

\begin{lemma} \label{Lem:SmYZ}
  If $(y_0, \dots y_n)$ is defined by \eqref{eq:modele_new} and $(z_0, \dots z_n)$ is defined as in Lemma \ref{Lem:YZ}, then 
  $$
  SS_m(y, {\rho}^*) = SS_m(z, {\rho}^*) + O_P(1),\textrm{ as } n\to\infty\;.
  $$
%   \begin{eqnarray*}
%   SS_m(y, {\rho}^*) & = & SS_m(z, {\rho}^*) + O_P(1),\textrm{ as } n\to\infty\;,\\
%   SS_m(y, \overline{\rho}_n) & = & SS_m(z, \overline{\rho}_n) + O_P(1),\textrm{ as } n\to\infty\;.
%   \end{eqnarray*}
\end{lemma}

\begin{lemma} \label{Lem:OP1}
  Let  $(X_n)$ and $(Y_n)$ be two sequences of rv's such that $X_n - Y_n = O_P(1)$. If $Y_n ^{-1} = O_P(n^{-1})$ then $X_n ^{-1} = O_P(n^{-1})$.
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{proof}[Proof of Lemma \ref{Lem:SSmY}]
Using the matrix notations from the proof of Lemma \ref{Lem:Delta_order}, we have
$$
SS_m(y, \rho^*) = \min_{T, \delta} \Vert y - \rho^* By - T \delta \Vert^2, 
\qquad
SS_m(y, \overline{\rho}_n) = \min_{T, \delta} \Vert y - \overline{\rho}_n  By - T \delta \Vert^2,
$$
where all minimizations are achieved over all segmentations with $m$ change points belonging to $\mathcal{A}_{n,m}$. 
Let us define $(\widehat{T}^*, \widehat{\delta}^*)$
and $(\overline{T}, \overline{\delta})$ by 
\begin{equation*}
(\widehat{T}^*, \widehat{\delta}^*) = \argmin_{T, \delta} \Vert y - \rho^*By - T\delta \Vert, 
\qquad
(\overline{T}, \overline{\delta}) = \argmin_{T, \delta} \Vert y - \overline{\rho}_n By - T\delta \Vert.
\end{equation*}
Note that $\widehat{T}^*$ and $\overline{T}$ refer to $\widehat{t}(y, \rho^*)$ and $\widehat{t}(y, \overline{\rho}_n)$, respectively. We have 
\begin{eqnarray} \label{Eq:UpperBoundSSdiff}
 \left| SS_m(y, \overline{\rho}_n) - SS_m(y, \rho^*) \right| 
 & = &  \left| \min_{T, \delta} \Vert y - \overline{\rho}_n By - T\delta \Vert^2 - \min_{T, \delta} \Vert y - \rho^* By - T\delta \Vert^2 \right| \nonumber \\
 & \leq & 
 \max \left( \left| \Vert y - \overline{\rho}_n By - \widehat{T}^*\widehat{\delta}^* \Vert^2 - \Vert y - \rho^*By - \widehat{T}^*\widehat{\delta}^* \Vert^2 \right|, \right. \nonumber\\
  & & \qquad \qquad \left. \left| \Vert y - \overline{\rho}_n By - \overline{T}\,\overline{\delta} \Vert^2 - \Vert y - \rho^*By - \overline{T}\,\overline{\delta} \Vert^2 \right| \right).
\end{eqnarray}
We now have to prove that this upper bound is $O_P(1)$. We first prove it for the second term of in the right-hand side of \eqref{Eq:UpperBoundSSdiff}. To do so, observe that
$\Vert y - \overline{\rho}_n By - \overline{T}\,\overline{\delta} \Vert^2
=\Vert y - \rho^*By - \overline{T}\,\overline{\delta}+(\rho^*-\overline{\rho}_n) By\Vert^2$. Thus,
$$
\Vert y - \overline{\rho}_n By - \overline{T}\overline{\delta} \Vert^2 - \Vert y - \rho^*By - \overline{T}\overline{\delta} \Vert^2 
=(\overline{\rho}_n  - \rho^*)^2 \Vert By\Vert^2 +2(\rho^*-\overline{\rho}_n)\langle By,y - \rho^*By - \overline{T}\,\overline{\delta} \rangle.
$$
Since, by (\ref{eq:modele_matriciel}) and Lemma \ref{Lem:YZ}, $y - \rho^*By - \overline{T}\,\overline{\delta}
=\epsilon - \Delta^* + (T^*\delta^*-\overline{T}\,\overline{\delta})=\epsilon- \Delta^*
+T^*(\delta^*-\overline{\delta})+(T^*-\overline{T})\overline{\delta}$, where $\Delta^*$ is the $n$-dimensional vector with entries $\Delta^*_i$, we get
\begin{multline}\label{eq:dec:second:terme}
\Vert y - \overline{\rho}_n By - \overline{T}\,\overline{\delta} \Vert^2 - \Vert y - \rho^*By - \overline{T}\,\overline{\delta} \Vert^2\\
=(\overline{\rho}_n  - \rho^*)^2 \Vert By\Vert^2 
+ 2 (\rho^*- \overline{\rho}_n ) \left(\langle By,\epsilon  \rangle + \langle By,T^* (\delta^* - \overline{\delta} )  \rangle 
+ \langle By,(T^*-\overline{T}) \overline{\delta}  \rangle - \langle By, \Delta^*\rangle \right).
\end{multline}
Let us now prove that each term in the right-hand side of (\ref{eq:dec:second:terme}) is $O_P(1)$.
\begin{enumerate}[($a$)]
\item Let us study the first term of (\ref{eq:dec:second:terme}).
Using Lemma \ref{lem:rateXY} and (\ref{eq:hypRhoRate}) we get that 
  \begin{equation}\label{Eq:rhoXnorm}
  (\overline{\rho}_n -\rho^*)^2 \Vert By\Vert^2 = O_P(1).
  \end{equation}
\item Let us now study the second term of (\ref{eq:dec:second:terme}). Observe that 
$
\left\langle By,\epsilon\right\rangle = \sum_{i=1}^n y_{i-1}\epsilon_i=\sum_{i=1}^n (y_{i-1}-\PE(y_{i-1}))\epsilon_i+\sum_{i=1}^n \PE(y_{i-1})\epsilon_i.
$
By using the Central limit theoreom for iid rv's and since there is a finite number of change-points, the second term
is $O_P(\sqrt{n})$. As for the first term, since $(y_{i-1}-\PE(y_{i-1}))$ is a causal AR(1) process, then by using the beginning of the proof of 
\cite[Proposition 8.10.1]{brockwell}, we get
that $\sum_{i=1}^n (y_{i-1}-\PE(y_{i-1}))\epsilon_i=O_P (\sqrt{n})$. Thus,
  \begin{equation} \label{Eq:CrossProd1}  
  \left\langle By,\epsilon\right\rangle %= \sum_{i=1}^n y_{i-1}\epsilon_i 
= O_P (\sqrt{n}).
 \end{equation}
  Furthermore, we have $\Vert T^* ( \delta^* - \overline{\delta} ) \Vert^2 = \sum_{k=0}^{m}\left(t_{k+1}^*-t_k^*\right) (\delta^*_k -\overline{\delta}_k)^2$ 
 where each term of the sum is $O_P(1)$, thanks to Proposition \ref{Prop:Segment2}, and so is the sum. 
Now using Lemma \ref{lem:rateXY} and the Cauchy-Schwarz inequality, we get 
\begin{equation} \label{Eq:CrossProd2}  
  \langle By, T^* ( \delta^* - \overline{\delta} )  \rangle = O_P(\sqrt{n}).
  \end{equation}
  The convergence rate of $\widehat{t}(y,\overline{\rho}_n)$ given in Proposition \ref{Prop:Segment2} ensures that, for any $\varepsilon>0$ there exists a positive $M$ 
such that each column of $(T^* - \overline{T})$ has at most $M$ non-zero coefficients with probability greater than $1-\varepsilon$. 
By using Proposition \ref{Prop:Segment2}, we obtain that with probability greater than $1-\varepsilon$
  \begin{equation}\label{eq:T*-Tbar}
  \Vert(T^* - \overline{T}) \overline{\delta} \Vert^2 \leq M \sum_k \overline{\delta}_k^2 =2 M \sum_k (\overline{\delta}_k-\delta^*_k)^2
+2M \sum_k {\delta^*_k}^2\leq MM',
\end{equation}
where $M'$ is a positive constant. 
By the Cauchy-Schwarz inequality, (\ref{eq:T*-Tbar}) and Lemma \ref{lem:rateXY}, we get 
  \begin{equation} \label{Eq:CrossProd3}  
  \langle By, (T^* - \overline{T}) \overline{\delta}  \rangle = O_P (\sqrt{n}).
  \end{equation}
  As $\Delta^*$ has only $m$ non-zero entries, $\langle By, \Delta^*\rangle$ is the sum of $m$ Gaussian rv's and is therefore $O_P(1)$.
  
  Thus, combining \eqref{Eq:CrossProd1}, \eqref{Eq:CrossProd2} and \eqref{Eq:CrossProd3} with (\ref{eq:hypRhoRate}), we get
  $$
  (\rho^*- \overline{\rho}_n ) \left(\langle By,\epsilon  \rangle + \langle By,T^* (\delta^* - \overline{\delta} )  \rangle + \langle By,(T^* - \overline{T}) \overline{\delta}  \rangle -  \langle By, \Delta^*\rangle \right) = O_P(1).
  $$
\end{enumerate}

To complete the proof, we need to consider the first term of \eqref{Eq:UpperBoundSSdiff}.
As $\rho^*$ satisfies the same assumptions as $\overline{\rho}_n$, using the same line of reasoning as for the second term holds so we get
$$
\Vert y - \overline{\rho}_n By - \widehat{T}^*\widehat{\delta}^* \Vert^2 - \Vert y - \rho^*By - \widehat{T}^*\widehat{\delta}^* \Vert^2 = O_P(1).
$$
% \textcolor{red}{
% By (\ref{eq:modele_matriciel}), the first term of \eqref{Eq:UpperBoundSSdiff} can be decomposed as
% \begin{eqnarray*}
%  & & \Vert Y - \overline{\rho}_n BY - \widehat{T}^*\widehat{\delta}^* \Vert^2 - \Vert Y - \rho^*BY - \widehat{T}^*\widehat{\delta}^* \Vert^2 
%   =  \| E + (\rho^* - \overline{\rho}_n ) BY \|^2 -\|E\|^2 \\
%  & = & (\rho^* - \overline{\rho}_n )^2 \|BY\|^2 + 2 (\rho^* - \overline{\rho}_n ) \langle BY, E\rangle, 
% \end{eqnarray*}
% each being $O_P(1)$ thanks to \eqref{Eq:rhoXnorm}, \eqref{Eq:CrossProd1} and (\ref{eq:hypRhoRate}),
% which concludes the proof.
% }
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{proof}[Proof of Lemma \ref{Lem:SmYZ}] 
The proof follows the same line of reasoning as the proof of Lemma \ref{Lem:SSmY}. 
Let us define $(\widehat{T}^y, \widehat{\delta}^y)$
and $(\widehat{T}^z, \widehat{\delta}^z)$ by 
\begin{equation*}
(\widehat{T}^y, \widehat{\delta}^y)
= \argmin_{T, \delta} 
\Vert y - \rho^* By - T \delta \Vert^2,
\qquad
(\widehat{T}^z, \widehat{\delta}^z)
= \argmin_{T, \delta} 
\Vert z - \rho^* Bz - T \delta \Vert^2.
\end{equation*}
% Note that $\widehat{T}^*$ and $\overline{T}$ refer to $\widehat{t}(y, \rho^*)$ and $\widehat{t}(z, \rho^*)$, respectively. 
We have 
\begin{multline*} 
\left|SS_m(y, \rho^*) - SS_m(z, \rho^*) \right\| 
 \leq 
 \max \left( \left| \Vert y - \rho^* By - \widehat{T}^y \widehat{\delta}^y \Vert^2 - \Vert z - \rho^*Bz - \widehat{T}^y \widehat{\delta}^y \Vert^2 \right|, \right. \\
 \left. \left| \Vert y - \rho^* By - \widehat{T}^z \widehat{\delta}^z \Vert^2 - \Vert z - \rho^*Bz - \widehat{T}^z \widehat{\delta}^z \Vert^2 \right| \right).
\end{multline*}
According to Lemma \ref{Lem:YZ}, we have $y - \rho^* By = z - \rho^* Bz - \Delta^*$ where $\Delta^*=(\Delta_i^*)$. As for the first term
\begin{multline*}
\Vert y - \rho^* By - \widehat{T}^y \widehat{\delta}^y \Vert^2 - \Vert z - \rho^*Bz - \widehat{T}^y \widehat{\delta}^y \Vert^2 \\
= \Vert \Delta^* \Vert^2 
- 2 \left(\langle \Delta^*,\epsilon \rangle + \langle \Delta^*, T^* (\delta^* - \widehat{\delta}^y )  \rangle 
+ \langle \Delta^*,(T^*-\widehat{T}^y) \widehat{\delta}^y \rangle \right),
\end{multline*}
the first term of which is a constant and all other terms being $O_P(1)$, which can be proved following the same line as the proof of Lemma \ref{Lem:SSmY}. The control of $\Vert y - \rho^* By - \widehat{T}^z \widehat{\delta}^z \Vert^2 - \Vert z - \rho^*Bz - \widehat{T}^z \widehat{\delta}^z \Vert^2$ follows the same lines.
  \end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{proof}[Proof of Lemma \ref{Lem:OP1}]
Observe that $X_n^{-1}=\left(Y_n+(X_n-Y_n)\right)^{-1}=Y_n^{-1}\left(1+Y_n^{-1}(X_n-Y_n)\right)^{-1}$. Since, by assumption, $Y_n^{-1}(X_n-Y_n)=O_P(n^{-1})$, the terms inside
the parentheses converges in probability to one. Thus, $\left(1+Y_n^{-1}(X_n-Y_n)\right)^{-1}$ is in particular $O_P(1)$ which concludes the proof.
\end{proof}

\begin{proof}[Proof of Proposition \ref{Prop:mBIC}]
   As for the proof of Proposition \ref{Prop:mBICBardet}, denoting $\widehat{\tau}_k(y, \rho) = \widehat{t}_k(y, \rho) /n$, the decomposition \eqref{Eq:DecompNkZ} still holds, replacing $z$ with $y$. Then, by Proposition~\ref{Prop:Segment2}, we have
   $$
   \sum_{k=0}^m \log n_k(\widehat{t}(y, \overline{\rho}_n))- \sum_{k=0}^m \log
   n_k(\widehat{t}(y, {\rho}^*))=O_P(1). 
   $$
   For a process $y$ under Model~\eqref{eq:modele_new}, we construct a process $z$ under Model~\eqref{eq:bkw} using Lemma~\ref{Lem:YZ}. The proof relies on the fact that $y$ inherits some properties of $z$. Again, we note that
   $$
   \log {SS}_m(y, \overline{\rho}_n) - \log {SS}_m(y, {\rho}^*)
    = R\left(\frac{{SS}_m(y, \overline{\rho}_n)-{SS}_m(y, {\rho}^*)}{{SS}_m(y, {\rho}^*)}\right).
   $$
  Lemma \ref{Lem:SSmY} states that ${SS}_m(y, \overline{\rho}_n)-{SS}_m(y, {\rho}^*) = O_P(1)$. 
  To conclude the proof we need to further show that $[{SS}_m(y, {\rho}^*)]^{-1} = O_P(n^{-1})$. We first show that $[{SS}_m(y, {\rho}^*) - {SS}_m(z, {\rho}^*)] = O_P(1)$ in Lemma~\ref{Lem:SmYZ} and, because $[{SS}_m(z, {\rho}^*)]^{-1} = O_P(n^{-1})$, we conclude using Lemma~\ref{Lem:OP1}.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Cha13.tex"
%%% End:



==> chapitres/commentaires.tex <==
Cette section contient des commentaires sur les articles présentés dans les chapitres~\ref{ch:ar1} et~\ref{ch:arp}.

\subsection{Commentaires sur le chapitre \ref{ch:ar1}}\label{ch:commentaires:sec:ar1}
\input{./chapitres/commentaires/ar1}

\subsection{Commentaires sur le chapitre \ref{ch:arp}}\label{ch:commentaires:sec:arp}
\input{./chapitres/commentaires/arp}


==> chapitres/commentaires/ar1.tex <==
L'article présenté au chapitre~\ref{ch:ar1} a pour objet principal la segmentation, c'est sur ce point que porte sa contribution principale, à savoir la justification théorique de la procédure consistant à décorréler les séries temporelles étudiées avant de les segmenter. C'est sur ce point, notamment la possibilité offerte de sélectionner le nombre de ruptures par le critère mBIC de \textcite{ZS} sans sur-segmentation~(cf. figure~\ref{comm:fig:zs:surseg}), que la méthodologie proposée est évaluée. Toutefois, les commentaires porteront principalement sur l'estimation du paramètre d'autorégression $\rho^\star$. On notera que l'estimation de ce paramètre n'est qu'un outil de la méthode de segmentation proposée, et absolument pas un but en soi. Seront évoqués la construction de l'estimateur utilisé, un autre estimateur, leurs propriétés asymptotiques respectives et leur utilisation dans une statistique de test.

\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{example.pdf}
\caption[Exemple de série où la décorrélation permet d'éviter la sur-segmentation.]{Exemple d'une des séries simulées dans l'étude réalisée dans la section \ref{ar1:sec:simul}, affectée de six ruptures. Ici, $n=1600$, $\rho^\star = 0.9$, $\sigma^\star = 0.3$. Les droites verticales marquent la localisation des ruptures estimées. On constate la sur-segmentation de la série si on utilise le critère mBIC sans décorrélation (gauche), contrairement au résultat donné par le critère mBIC après décorrélation (droite).}\label{comm:fig:zs:surseg}
\end{figure}



\subsubsection{Construction de l'estimateur $\widetilde{\rho}_n$}

\input{./chapitres/commentaires/ar1/construction.tex}

\subsubsection{Un autre estimateur}

\input{./chapitres/commentaires/ar1/autre.tex}

\subsubsection{Efficacité asymptotique relative}\label{ch:commentaires:sec:ar1:subs:efficacite}

\input{./chapitres/commentaires/ar1/efficacite.tex}

\subsubsection{Tester l'hypothèse \enquote{$\rho^\star = 0$}}\label{ch:commentaires:sec:ar1:subs:test}

\input{./chapitres/commentaires/ar1/test.tex}


==> chapitres/commentaires/ar1/autre.tex <==
L'estimateur $\widetilde{\rho}_n$, défini en \eqref{ar1:eq:est_rho}, permet de justifier, par ses propriétés et sa rapidité de calcul, la démarche suivie dans le reste de l'article~\parencite[complexité en temps en $O(n)$ grâce à un algorithme de sélection, voir par exemple ][]{blum1973time}. Mais on pourrait trouver bien d'autres estimateurs.

L'estimateur que l'on va construire ici a, au prix d'une complexité en temps de son calcul plus grande \parencite[en $O(n\log n)$, comme l'estimateur $Q_n$ de ][]{CR}, une variance asymptotique qui semble, d'après les simulations~(cf. section~\ref{ch:commentaires:sec:ar1:subs:efficacite}), plus petite que $\widetilde{\rho}_n$. Supposons que l'on observe $\left(y_i\right)_{1\leq i\leq n}$ défini en l'équation~\eqref{ar1:eq:modele_new}. Soit $\boldsymbol{x}=\left(x_i\right)_{1\leq i\leq n-1} = \left(y_{i+1}-y_i\right)_{1\leq i\leq n-1}$. Soit $\widehat{\rho}_{MG,n}\left(h,\cdot\right)$ l'estimateur de \textcite{MG} de l'autocorrélation à l'ordre $h\in\mathbb{Z}$, défini en~\eqref{eq:MGcorr}. On considère l'estimateur suivant de $\rho^\star$:
\begin{equation}\label{ch:commentaires:sec:ar1:subs:autre:eq:def}
\widetilde{\rho}_n^\prime = 1 + 2\widehat{\rho}_{MG,n}\left(1,\boldsymbol{x}\right) \; .
\end{equation}

\begin{prop}\label{prop:nouveauRho}
Soit $\left(y_i\right)_{1\leq i\leq n}$ défini en l'équation \eqref{ar1:eq:modele_new} et  $\left(\eta_i\right)_{i\in\mathbb{Z}}$ défini en \eqref{ar1:eq:ar1}. On note $\boldsymbol{x}=\left(x_i\right)_{1\leq i\leq n-1} = \left(y_{i+1}-y_i\right)_{1\leq i\leq n-1}$, et $\left(\nu_i\right)_{i\in\mathbb{Z}}=\left(\eta_{i+1}-\eta_i\right)_{i\in\mathbb{Z}}$. Soit $\widetilde{\rho}_n^\prime$ défini en \eqref{ch:commentaires:sec:ar1:subs:autre:eq:def}. Alors
\begin{eqnarray*}\label{ch:outils:sec:robuste:convergenceRhoPrime} 
\sqrt{n}\left(\widetilde{\rho}_n^\prime-\rho^{\star 2}\right) & \underset{n\rightarrow\infty}{\overset{d}{\longrightarrow}} & \mathcal{N}\left(0, \tilde{\sigma}^{\prime 2} \right) \; ,
\end{eqnarray*}
où
\begin{eqnarray}
\tilde{\sigma}^{\prime 2} & = & 4\mathbb{E}\left[\psi^2\left(\nu_0,\nu_{1}\right)\right] + 8 \sum_{k=1}^\infty \mathbb{E}\left[ \psi\left(\nu_0,\nu_{1}\right) \psi\left(\nu_{k},\nu_{k+1}\right) \right] \; , \label{eq:sigma_prime_carre}\\
\psi : (x,y) & \mapsto & \left\{\frac{1+\rho^\star}{2} \IF\left(\frac{x+y}{\sqrt{\sigma^{\star 2}(1-\rho^\star)}}\right)  - \frac{3-\rho^\star}{2} \IF\left(\frac{(x-y)\sqrt{1+\rho^\star}}{\sqrt{\sigma^{\star 2}(3-\rho^\star)(1-\rho^\star)}}\right)\right\}\; , \\
\IF : x & \mapsto & c_{Q,\Phi}\left(\frac{1/4-\Phi(x+1/c_{Q,\Phi}) +\Phi(x-1/c_{Q,\Phi})}{\int_{\rset} \phi(y)\phi(y+1/c_{Q,\Phi})\rmd y}\right) \; ,
\end{eqnarray}
$\Phi$ est la fonction de répartition de la loi normale centrée réduite, $\phi=\Phi^\prime$ et $c_{Q,\Phi}$ est défini par \eqref{eq:constante_cQPhi}.
\end{prop}
\begin{proof}
Le résultat découle directement de :
\begin{itemize}
\item le corollaire \ref{ch:outils:sec:robuste:cor:asymptotiqueCLL} appliqué à $\left(\nu_i\right)_{i\in\mathbb{Z}}$.
\item $\forall h\in\mathbb{Z}, \gamma_\nu(h) = 2\gamma_\eta(h)-\gamma_\eta(h-1)-\gamma_\eta(h+1)$.
\item $\gamma_\eta (0) = \frac{\sigma^{\star 2}}{1-\rho^{\star 2}}$, en particulier $\rho^\star = 1 + 2\rho_\nu (1)$.
\end{itemize}
\end{proof}
\begin{remarque}
$\tilde{\sigma}^{\prime 2}$ ne dépend que de $\rho^\star$ et non de $\sigma^\star$. À l'instar de la variance asymptotique $\tilde{\sigma}^{\prime 2}$ de l'estimateur $\widetilde{\rho}_n$ donnée par l'équation \eqref{ar1:eq:def_sigmatilde}, l'expression \eqref{eq:sigma_prime_carre} n'est pas aisément calculable en fonction de $\rho^\star$. On propose ci-dessous un calcul par la méthode de Monte-Carlo.
\end{remarque}

==> chapitres/commentaires/ar1/construction.tex <==
Les estimateurs $S_n$ et $Q_n$ de \textcite{CR} d'un paramètre d'échelle d'un échantillon $\boldsymbol{x}=\left(x_1,\dots,x_n\right)$, définis resp. en \eqref{eq:CRS} et en \eqref{eq:CRQ}, font intervenir les quantiles des différences $\left|x_i - x_j\right|, \; (1\leq i<j \leq n)$. Plaçons-nous dans le modèle des valeurs aberrantes additives~(\emph{additive outliers}, AO), où un nombre $k$ d'observations de cet échantillon est affecté par une perturbation déterministe: $\tilde{\boldsymbol{x}} = \boldsymbol{x} + \boldsymbol{v}$ où $\boldsymbol{v}\in\mathbb{R}^n$ n'a que $k$ composantes non-nulles. La définition du modèle AO est ici simplifiée pour la clarté de l'exposé \parencite[cf.][section 8.1.2]{maronna}.

Parmi les $n(n-1)/2$ différences $v_i - v_j, \; (1\leq i<j \leq n)$, au plus $k(n-1)$ différences sont non nulles. Donc parmi les $n(n-1)/2$ différences $\tilde{x}_i - \tilde{x}_j = (x_i - x_j) + (v_i - v_j), \; (1\leq i<j \leq n)$, au plus $k(n-1)$ différences sont différentes de $x_i - x_j$, on dira qu'elles sont contaminées. C'est ce qui permet d'obtenir un point d'effondrement (cf. définition \ref{def:BP}) tendant vers $1/2$ pour $Q_n$.

Supposons maintenant que l'on observe $\left(y_i\right)_{1\leq i\leq n}$ défini en l'équation \eqref{ar1:eq:modele_new}. Les seules différences $y_i - y_j, \; (1\leq i<j \leq n)$ dont on est sûr qu'elles soient égales à $\eta_i - \eta_j$, et donc centrées, sont les différences intra-segment: 
$$y_i - y_j, \; (t_{k-1}^\star + 1 \leq i<j \leq t_k^\star, 1\leq k \leq m^\star +1 ) \; .$$
Il n'y en a que $\sum_{k=1}^{m^\star +1} \left(t_k^\star - t_{k-1}^\star \right)\left(t_k^\star - t_{k-1}^\star - 1 \right)/2$. S'il n'y a qu'une seule rupture, la borne supérieure de cette quantité, quand la rupture varie, est $n(n-2)/4$; soit une proportion $(n-2)/(2n-2)<1/2$ des différences $y_i - y_j, \; (1\leq i<j \leq n)$. De plus, cette borne supérieure décroît avec le nombre de ruptures. Par conséquent, même avec une seule rupture, on a possiblement un taux de contamination strictement supérieur à $1/2$ des différences $y_i - y_j, \; (1\leq i<j \leq n)$~(cf. figure~\ref{ch:commentaires:sec:ar1:subs:construction:fig:contamination}).

Pour construire un estimateur de $\rho^\star$ dans ce cadre, nous ne considérons donc pas toutes les différences  $y_i - y_j, \; (1\leq i<j \leq n)$, mais seulement une partie d'entre elles. En effet, parmi les $n-1$ différences $y_{i+1}-y_i, \; (1\leq i\leq n-1)$, seules $m^\star$ différences sont contaminées. De même, parmi les $n-2$ différences $y_{i+2}-y_i, \; (1\leq i\leq n-2)$, au plus $2m^\star$ différences sont contaminées. D'où l'estimateur proposé, défini en \eqref{ar1:eq:est_rho}, faisant intervenir les médianes de ces deux familles de différences entre observations.

\begin{figure}
\centering
\setlength{\unitlength}{0.05cm}
\begin{picture}(120,110)
%\begin{picture}(360,330)
\put(0,110){
   \circle{8}
}
\textcolor{red}{
\put(0,100){
   \circle*{8}
}}
\put(0,100){
   \circle{8}
}
\put(10,106){\shortstack[c]{$\mathbb{E}\left(y_i - y_j\right)=0$}}
\put(10,96){\shortstack[c]{$\mathbb{E}\left(y_i - y_j\right)\neq 0$}}

\put(45,0){\shortstack[c]{$j$}}
\put(120,55){\shortstack[c]{$i$}}

\put(0,10){\footnotesize{\shortstack[c]{$2$}}}
\put(15,10){\shortstack[c]{$\cdots$}}
\put(21,10){\footnotesize{\shortstack[c]{$t_k-1$}}}
\put(42,10){\footnotesize{\shortstack[c]{$t_k$}}}
\put(50,10){\footnotesize{\shortstack[c]{$t_k +1$}}}
\put(70,10){\shortstack[c]{$\cdots$}}
\put(90,10){\footnotesize{\shortstack[c]{$n$}}}

\put(100,17.5){\footnotesize{\shortstack[c]{$1$}}}
\put(100,35){\shortstack[c]{$\vdots$}}
\put(100,47.5){\footnotesize{\shortstack[c]{$t_k-2$}}}
\put(100,57.5){\footnotesize{\shortstack[c]{$t_k-1$}}}
\put(100,67.5){\footnotesize{\shortstack[c]{$t_k$}}}
\put(100,90){\shortstack[c]{$\vdots$}}
\put(100,107.5){\footnotesize{\shortstack[c]{$n-1$}}}

\put(0,20){
   \circle{8}
}
\put(15,20){\shortstack[c]{$\cdots$}}
\put(30,20){
   \circle{8}
}
\textcolor{red}{
\put(40,20){
   \circle*{8}
}}
\put(40,20){
   \circle{8}
}
\textcolor{red}{
\put(50,20){
   \circle*{8}
}}
\put(50,20){
   \circle{8}
}
\put(70,20){\shortstack[c]{$\cdots$}}
\textcolor{red}{
\put(90,20){
   \circle*{8}
}}
\put(90,20){
   \circle{8}
}

\put(15,35){\shortstack[c]{$\udots$}}
\put(30,35){\shortstack[c]{$\vdots$}}
\put(40,35){\shortstack[c]{$\vdots$}}
\put(50,35){\shortstack[c]{$\vdots$}}
\put(90,35){\shortstack[c]{$\vdots$}}

\put(30,50){
	\circle{8}
}
\textcolor{red}{
\put(40,50){
   \circle*{8}
}}
\put(40,50){
	\circle{8}
}
\textcolor{red}{
\put(50,50){
   \circle*{8}
}}
\put(50,50){
	\circle{8}
}
\put(70,50){\shortstack[c]{$\cdots$}}
\textcolor{red}{
\put(90,50){
   \circle*{8}
}}
\put(90,50){
	\circle{8}
}

\textcolor{red}{
\put(40,60){
   \circle*{8}
}}
\put(40,60){
	\circle{8}
}
\textcolor{red}{
\put(50,60){
   \circle*{8}
}}
\put(50,60){
	\circle{8}
}
\put(70,60){\shortstack[c]{$\cdots$}}
\textcolor{red}{
\put(90,60){
   \circle*{8}
}}
\put(90,60){
	\circle{8}
}

\put(50,70){
	\circle{8}
}
\put(70,70){\shortstack[c]{$\cdots$}}
\put(90,70){
	\circle{8}
}

\put(70,90){\shortstack[c]{$\udots$}}
\put(90,90){\shortstack[c]{$\vdots$}}

\put(90,110){
	\circle{8}
}
%\put(10,10){\shortstack[c]{$\Huge\dots$}}
%\put(15,10){
%   \circle*{5}
%}

\thicklines
\textcolor{darkgreen}{
\put(43.275,63.075){
\rotatebox{45}{
\oval(136,8)
}
}
}
\end{picture}
\caption[Surcontamination des différences entre observations dans un modèle de segmentation.]{Illustration de la surcontamination des différences entre observations $y_i - y_j,\; (1\leq i<j\leq n)$ dans un modèle de segmentation par rapport au modèle AO. Le problème disparaît si on impose $j=i+1$.}\label{ch:commentaires:sec:ar1:subs:construction:fig:contamination}
\end{figure}

==> chapitres/commentaires/ar1/efficacite.tex <==
Pour chaque paramètre d'autorégression $\rho^\star \in \left\{ -0.9, -0.8, \dots , 0.9\right\}$, nous avons simulé 5000~séries AR(1) centrées, gaussiennes, de variance~1, de longueur~10000. Le but n'étant pas de mesurer la robustesse de ces estimateurs à la présence de ruptures, ces séries ne sont pas affectées par des ruptures. Les variances asymptotiques des deux estimateurs $\widetilde{\rho}_n$ et $\widetilde{\rho}_n^\prime$, respectivement $\tilde{\sigma}^2$ et $\tilde{\sigma}^{2\prime}$, ont été estimées. Cela a permis d'estimer l'efficacité asymptotique relative respective des deux estimateurs $\widetilde{\rho}_n$ et $\widetilde{\rho}_n^\prime$ relativement à l'estimateur des moments $\widehat{\rho}_n(1)$~(cf. remarque~\ref{ar1:corrr:remark:moments}), c'est-à-dire
\begin{eqnarray*}
\frac{1-\rho^{\star 2}}{\tilde{\sigma}^2} \; , & & \frac{1-\rho^{\star 2}}{\tilde{\sigma}^{\prime 2}} \; .
\end{eqnarray*}

La figure~\ref{ch:commentaire:sec:ar1:fig:efficacite} représente les résultats. $\widetilde{\rho}_n^\prime$ est meilleur que $\widetilde{\rho}_n$ et les performances de ces deux estimateurs décroissent fortement quand $\rho^\star$ tend vers 1. L'influence de l'erreur d'estimation de $\rho^\star$ dans les performances de la segmentation était visible dans l'étude de simulation de la section \ref{ar1:sec:simul}, voir par exemple la figure \ref{ar1:fig:hausd_1_sig05}. La figure \ref{ar1:fig:Kchap_sig05} semble elle suggérer que pour sélectionner le nombre de ruptures à l'aide du critère mBIC, il vaut mieux décorréler avec un estimateur peu performant que ne pas décorréler du tout quand $\rho^\star$ est proche de 1.

Pour résumer, l'estimateur $\widetilde{\rho}_n^\prime$ semble avoir de meilleures performances que $\widetilde{\rho}_n$. Ces dernières se dégradent fortement quand $\rho^\star$ est positivement grand. Toutefois, malgré cette perte d'efficacité des estimateurs du paramètre d'autorégression, il reste préférable de décorréler la série avant de sélectionner le nombre de ruptures par mBIC.

\begin{figure}
\centering
\includegraphics[width=0.6\textwidth]{efficacite.pdf}
\caption[Efficacité asymptotique relative des estimateurs du paramètre d'autorégression.]{Efficacité asymptotique relative estimée de $\widetilde{\rho}_n$ et $\widehat{\rho}_n(1)$ (ligne pleine) et de $\widetilde{\rho}_n^\prime$ et $\widehat{\rho}_n(1)$ (en pointillés), en fonction de $\rho^\star$.}\label{ch:commentaire:sec:ar1:fig:efficacite}
\end{figure}

==> chapitres/commentaires/ar1/test.tex <==
Comme annoncé dans la remarque \ref{ar1:corrr:remark:test}, la normalité asymptotique de $\widehat{\rho}_n$ permet de tester $H_0: \; \rho^\star = 0$ contre $H_1 : \; \rho^\star \neq 0$ ou $H_1^\prime : \; \rho^\star > 0$. La méthode de segmentation après décorrélation introduite au chapitre~\ref{ch:ar1} n'apporte pas d'amélioration substantielle à la segmentation dans le cas $\rho^\star < 0$. Le test le plus judicieux pour savoir s'il faut décorréler avant de segmenter semble être $H_0$ contre $H_1^\prime$.

\begin{prop}
Sous les mêmes hypothèses et avec les mêmes notations que la proposition~\ref{ar1:prop:correlation}, si $\rho^\star=0$ alors $\tilde{\sigma}^2 = \tilde{\sigma}^2_0$, où
\begin{equation*}
\tilde{\sigma}^2_0 = \frac{3 - 8 P\left(\max\left(\left|Y-X\right|,\left|Z-X\right|\right)\leq \sqrt{2}\Phi^{-1}(3/4)\right)}{2\left[\Phi^{-1}(3/4)\phi\left(\Phi^{-1}(3/4)\right)\right]^2} \; ,
\end{equation*}
où $X,Y,Z$ sont trois v.a.r. indépendantes de loi normale centrée réduite, $\Phi$ est la fonction de répartition de la loi normale centrée réduite et $\phi=\Phi^\prime$.
\end{prop}

\begin{proof}
$\rho^\star=0$ donc les v.a.r. gaussiennes $\eta_i$ sont indépendantes. On supposera, sans perdre de généralité, que $\sigma^\star = 1$.
On remarque que $\forall k \in\mathbb{N}, \PE\left[\Psi\left(\eta_k,\eta_{k+1},\eta_{k+2}\right)\right] = 0$, où $\Psi$ est défini en \eqref{ar1:eq:def_Psi}. Or les v.a.r. $\eta_i$ sont indépendantes, donc $$\forall k \geq 3, \PE\left[\Psi\left(\eta_0,\eta_{1},\eta_{2}\right)\Psi\left(\eta_k,\eta_{k+1},\eta_{k+2}\right)\right] = 0 \; . $$ Par conséquent, d'après \eqref{ar1:eq:def_sigmatilde}, 
\begin{equation*}
\tilde{\sigma}^2 = \PE\left[\Psi\left(\eta_0,\eta_{1},\eta_{2}\right)^2\right] + 2 \PE\left[\Psi\left(\eta_0,\eta_{1},\eta_{2}\right)\Psi\left(\eta_1,\eta_{2},\eta_{3}\right)\right] + \PE\left[\Psi\left(\eta_0,\eta_{1},\eta_{2}\right)\Psi\left(\eta_2,\eta_{3},\eta_{4}\right)\right] \; .
\end{equation*}
Notons:
\begin{eqnarray*}
\lambda & = & \left[\Phi^{-1}(3/4)\phi\left(\Phi^{-1}(3/4)\right)\right]^{-2} \; , \\
c &= & \sqrt{2}\Phi^{-1}(3/4) \; , \\
p & = & P\left(\max\left(\left|Y-X\right|,\left|Z-X\right|\right)\leq \sqrt{2}\Phi^{-1}(3/4)\right) \; .
\end{eqnarray*}

On remarque que, pour tous $i,j,k,l\in\zset$ tels que $i\neq j$ et $k\neq l$:
\begin{itemize}
\item si $\left\{i,j\right\}\cap \left\{k,l\right\} = \emptyset$, alors $P\left(\left|\eta_i - \eta_j\right|\leq c, \left|\eta_k - \eta_l\right|\leq c\right)=P\left(\left|\eta_i - \eta_j\right|\leq c)P(\left|\eta_k - \eta_l\right|\leq c\right)=1/4$,
\item si $\sharp\left( \left\{i,j\right\}\cap \left\{k,l\right\} \right) = 1$, alors $P\left(\left|\eta_i - \eta_j\right|\leq c, \left|\eta_k - \eta_l\right|\leq c\right) = p$,
\item si $\left\{i,j\right\}= \left\{k,l\right\}$, alors $P\left(\left|\eta_i - \eta_j\right|\leq c, \left|\eta_k - \eta_l\right|\leq c\right)=P\left(\left|\eta_i - \eta_j\right|\leq c\right)=1/2$.
\end{itemize}
Cela permet de calculer:
\begin{eqnarray*}
\PE\left[\Psi\left(\eta_0,\eta_{1},\eta_{2}\right)^2\right] & = & \lambda (1- 2p) \; , \\
2 \PE\left[\Psi\left(\eta_0,\eta_{1},\eta_{2}\right)\Psi\left(\eta_1,\eta_{2},\eta_{3}\right)\right] & = & \lambda\left(\frac{1}{2} - 2p\right) \; , \\
\PE\left[\Psi\left(\eta_0,\eta_{1},\eta_{2}\right)\Psi\left(\eta_2,\eta_{3},\eta_{4}\right)\right] & = & 0 \; .
\end{eqnarray*}
D'où $\tilde{\sigma}_0^2 = \lambda\left(\frac{3}{2} - 4p\right)$ et le résultat.
\end{proof}

\begin{remarque}
Le calcul numérique de $\tilde{\sigma}^2_0$ donne 8.567488.
\end{remarque}

La p-valeur asymptotique du test de $H_0$ contre $H_1$ est donc $2-2\Phi\left(\sqrt{\frac{n}{\tilde{\sigma}_0^2}} \left| \widetilde{\rho}_n \right|\right)$. La p-valeur asymptotique du test de $H_0$ contre $H_1^\prime$ est $1-\Phi\left(\sqrt{\frac{n}{\tilde{\sigma}_0^2}} \widetilde{\rho}_n \right)$.

On peut faire la même chose avec $\widetilde{\rho}_n^\prime$. On a estimé la valeur de $\tilde{\sigma}^{\prime 2}$ quand $\rho^\star=0$ par Monte-Carlo (cf. section \ref{ch:commentaires:sec:ar1:subs:efficacite}). La valeur trouvée était 2.53566. Ces estimations, par la méthode de Monte-Carlo, semblent indiquer que, pour tout $\rho^\star$, la variance asymptotique de $\widetilde{\rho}_n^\prime$ est plus petite que celle de $\widetilde{\rho}_n^\prime$. Par conséquent, le test de $H_0$ contre $H_1$, resp. $H_1^\prime$, de p-valeur asymptotique $2-2\Phi\left(\sqrt{\frac{n}{\tilde{\sigma}_0^{\prime 2}}} \left| \widetilde{\rho}_n^\prime \right|\right)$, resp. $1-\Phi\left(\sqrt{\frac{n}{\tilde{\sigma}_0^{\prime 2}}} \widetilde{\rho}_n^\prime \right)$, semble plus puissant que le test qui utilise $\widetilde{\rho}_n$ au lieu de $\widetilde{\rho}_n^\prime$.

Pour résumer, pour déterminer s'il faut ou non décorréler avant de segmenter une série AR(1), nous recommanderions de tester l'hypothèse $H_0: \; \rho^\star = 0$ contre $H_1^\prime : \; \rho^\star > 0$, en utilisant le test de p-valeur asymptotique $1-\Phi\left(\sqrt{\frac{n}{\tilde{\sigma}_0^{\prime 2}}} \widetilde{\rho}_n^\prime \right)$.

==> chapitres/commentaires/arp.tex <==
Les commentaires qui suivent sur l'article présenté dans le chaptire~\ref{ch:arp} portent sur l'estimation des paramètres de l'autorégression, notamment sur quelques idées opur réduire la variance des estimateurs, ainsi que sur le post-traitement à l'ordre $p>1$ des instants de rupture estimés, qui pose des problèmes sensiblement différents de l'ordre 1.

\subsubsection{À propos de l'estimation des paramètres de l'autorégression}
\input{./chapitres/commentaires/arp/estimation}

\subsubsection{À propos du post-traitement}
\input{./chapitres/commentaires/arp/post}


==> chapitres/commentaires/arp/estimation.tex <==
Les performances de l'estimateur $\widetilde{\Phi}_n^{(p)}$ varient beaucoup sur l'ensemble des paramètres. Cela peut être vu comme un problème de conditionnement de la matrice $R_p$, définie en \eqref{eq:matrixR}, à inverser. Voilà pourquoi l'emploi d'une version régularisée de l'estimateur est suggérée dans la remarque \ref{arp:remark:regularization}. Toutefois, la sélection conjointe du nombre de ruptures et de l'ordre de l'autorégression parvient à éviter en partie ces configurations qui induisent de mauvaises estimations des paramètres de l'autorégression et des instants de rupture (voir le tableau~\ref{table:phi1_02_phi2_06_sigma04} et les figures~\ref{fig:box:phi1_02_phi2_06_sigma04} et~\ref{fig:dens:phi1_02_phi2_06_sigma04}).

==> chapitres/commentaires/arp/post.tex <==
Le post-traitement des ruptures estimées (cf. section \ref{sec:post-proc}), est de même nature dans le cas des séries AR($p$) ou AR(1). La décorrélation induit possiblement $p$ ruptures artéfactuelles adjacentes à droite de la \enquote{vraie} rupture estimée. On les élimine donc. Des problèmes peuvent apparaître dans le cas où l'on a deux vraies ruptures à distance inférieure ou égale à $p$. Dans ce cas, la \enquote{vraie} seconde rupture ne peut pas être distinguée des ruptures artéfactuelles engendrées par la première rupture. Cette seconde rupture sera éliminée par le post-traitement, mais le premier des artéfacts qu'elle a engendré se trouvant à une distance supérieure à $p$ de la première rupture, s'il est détecté, sera conservé (voir figure \ref{figure:pp5}). Pour éviter ce problème, on peut interdire à des ruptures estimées d'être à distance inférieure ou égale à $p$, ce qui est cohérent avec le fait que dans les propositions~\ref{Prop:Segment} et~\ref{Prop:Segment2}, l'optimisation du critère se fait sous contrainte d'une distance entre ruptures qui tend vers l'infini avec la taille de la série (équation~\eqref{eq:Anm}).

\begin{figure}[!h]
\centering
\includegraphics[width=0.7\textwidth]{pp52.pdf}
\caption[Post-traitement, cas AR$(p)$.]{En haut à gauche: une série AR(5) affectée de deux ruptures dans l'espérance, à distance 3 l'une de l'autre. En haut à droite: la série décorrélée. En bas à gauche: avant le post-traitement, on détecte des ruptures, qu'il s'agisse de vraies ruptures~(vert, trait plein) ou d'artéfacts dûs à la décorrélation~(rouge, trait pointillé). En bas à droite: dans cette configuration, le post-traitement élimine les artéfacts de la première rupture, mais aussi la vraie seconde rupture, alors qu'un des artéfacts qui lui est associé est conservé.}\label{figure:pp5}
\end{figure}

==> chapitres/intro.tex <==
L'objet de ce chapitre est, d'une part, de présenter la segmentation de processus et son rapport à la dépendance entre les observations et, d'autre part, de délimiter l'objet de cette thèse.

La segmentation de processus a de nombreux champs d'application, comme:
\begin{itemize}
\item la climatologie~\parencites(par exemple)(){peterson1998homogeneity}{aguilar2003guidance}{beaulieu2007synthese}{beaulieu2012change},
\item l'économétrie~\parencites{stock1996evidence}{BPalgo}{pesaran2006forecasting}{geweke2011inference},
\item la génomique~\parencites{braun1998statistical}{braun2000multiple}{picard2005statistical}{hocking2013learning},
\item la géodésie~\parencites{Williams2003}{kenyeres2004EPN}{perfetti2006discontinuities}{Gazeaux2013},
\item l'hydrométrie~\parencites{cobb1978problem}{jaruskova1997}{perreault2000bayesian}{ehsanzadeh2011},
\item l'imagerie médicale~\parencites{kaplan2000brain}{lavielle2005using},
\item la stylométrie~\parencites{chen2015graph}.
\end{itemize} 
Formulé de façon générale, le problème est le suivant: étant donné des observations $y_1,\dots ,y_n$, il s'agit d'identifier les segments sur lesquels la série $y_i,\dots ,y_j\; (i<j)$ est homogène, en un sens à préciser. Les bornes de ces segments sont les \emph{ruptures}. Elle marquent l'instant de la perte de cette propriété d'homogénéité. Les questions qui se posent sont alors:
\begin{itemize}
\item combien y a-t-il de ruptures?
\item quelle sont leurs positions?
\item quelles sont les propriétés de la série à l'intérieur de chaque segment? ses propriétés globales en dehors de la segmentation? On peut penser à des problèmes de sélection de modèle, d'estimation, de test,~etc.
\end{itemize}

\section{Cas où les observations sont indépendantes}\label{ch:intro:sec:indep}
\input{./chapitres/intro/indep}
\section{Cas où les observations sont dépendantes}
\input{./chapitres/intro/dep}

\section{Approche adoptée}\label{ch:intro:sec:dep:subs:approche}
\input{./chapitres/intro/approche}


==> chapitres/intro/approche.tex <==
Dans cette thèse, on s'intéresse à la segmentation dans la moyenne de processus dépendants. On considère le modèle~\eqref{eq:modele_LM}, en supposant de plus que $y_1,\dots ,y_n$ sont $n$ observations successives d'un processus $\left(y_i\right)_{i\in\mathbb{Z}}$. Le travail est guidé par deux idées:
\begin{itemize}
\item la prise en compte de la dépendance dans l'inférence,
\item l'efficacité algorithmique.
\end{itemize}

Les algorithmes exacts efficaces (de type programmation dynamique) le sont à condition que le contraste à minimiser soit additif en les segments (voir la section~\ref{ch:outils:sec:algo}). Or, la prise en compte de la dépendance viole en général cette contrainte. L'objectif de cette thèse est de faire entrer l'inférence pour un processus dépendant dans un cadre admissible pour la programmation dynamique, tout en conservant les garanties statistiques.
 
 Il n'y a aucune rupture dans la structure de dépendance de $\left(\eta_i\right)_{i\in\mathbb{Z}}$. Donc, à priori, aucune raison de traiter ce cas comme dans la section \ref{ch:intro:sec:dep:subs:autres}. Néanmoins, les approches présentées dans la section \ref{ch:intro:sec:dep:subs:autres} peuvent nous aider à prendre en compte la structure de dépendance de $\left(\eta_i\right)_{i\in\mathbb{Z}}$.

On considère que le processus $\left(\eta_i\right)_{i\in\mathbb{Z}}$ est centré et faiblement stationnaire et que sa fonction d'autocovariance appartient à une famille paramétrée $\left(\sigma^2\gamma_\theta\right)_{\sigma^2>0,\theta\in\Theta}$. Si $\left(\eta_i\right)_{i\in\mathbb{Z}}$ est un processus causal, on peut exprimer la quasi-vraisemblance de $\left(y_1,\dots,y_n\right)$ conditionnellement à $\left(y_i\right)_{i\leq 0}$. Il s'agit de la vraisemblance conditionnelle de $\left(y_1,\dots,y_n\right)$ sachant $\left(y_i\right)_{i\leq 0}$ si le processus est supposé gaussien.

Dans cette quasi-vraisemblance, les termes correspondant aux ruptures $t_k$, aux espérances $\mu_k$, à $\sigma^2$ et à $\theta$ sont liés. À priori, ce critère ne peut pas être maximisé en utilisant l'algorithme de programmation dynamique, qui s'impose dans le cas où les observations sont indépendantes~(section~\ref{ch:intro:sec:indep:subs:algo}).

Le premier problème qui se pose est la présence d'un paramètre $\theta$ global. Nous n'avons pas pour objectif ultime d'estimer ce paramètre. Il s'agit d'un paramètre de nuisance, dont l'estimation permettra possiblement d'améliorer l'estimation des autres paramètres.

Le but est alors de construire un tel estimateur de $\theta$, tout en évitant d'avoir à segmenter la série, c'est-à-dire d'estimer les ruptures $t_k^\star$ sans connaître $\theta$, ce que l'on cherche précisément à éviter. Nous nous sommes orientés vers des méthodes robustes.

Nous avons mis en œuvre cette méthodologie dans le cas où $\left(\eta_i\right)_{i\in\mathbb{Z}}$ est un processus $AR(1)$ dans le chapitre~\ref{ch:ar1} et dans le cas où il s'agit d'un processus autorégressif d'ordre fini arbitraire dans le chapitre~\ref{ch:arp}. Dans ces cas-là, du point de vue de l'inférence des ruptures, l'estimation préalable du paramètre $\theta$, qui est ici le paramètre de l'autorégression, revient à décorréler la série, puis à adopter l'inférence classique du cas indépendant sur les séries ainsi décorrélées.

 Dans le chapitre~\ref{ch:commentaires_discussion}, on discute de la méthodologie adoptée, de méthodes alternatives et de résultats additionnels. Les limites de l'approche adoptée sont ensuite discutées avant de tracer quelques perspectives de travaux futurs concernant des résultats mathématiques employés à étendre, l'extension de la méthode employée à une classe de processus plus large ou des problèmes connexes en segmentation permettant de mettre en œuvre une approche similaire.

==> chapitres/intro/dep.tex <==
Jusqu'à présent, nous avons considéré que les observations des séries temporelles considérées étaient indépendantes. Toutefois, dans un certain nombre d'applications, par exemple en géosciences ou en météorologie\footnote{Références en préambule du chaptire~\ref{chap:intro}.}, cette condition est clairement violée.

\subsection{Plusieurs types de ruptures}
\input{./chapitres/intro/dep/types}

\subsection{Ruptures dans la loi marginale}\label{ch:intro:sec:dep:subs:marginale}
\input{./chapitres/intro/dep/marginale}

\subsection{Autres types de ruptures}\label{ch:intro:sec:dep:subs:autres}
\input{./chapitres/intro/dep/autres}

\subsection{Sélection de modèle}\label{ch:intro:sec:dep:subs:selection}
\input{./chapitres/intro/dep/selection}

==> chapitres/intro/dep/autres.tex <==
On peut aussi considérer des ruptures qui affectent d'autres propriétés des séries que la loi marginale, c'est-à-dire qu'elles affectent la structure de dépendance des séries temporelles.

Supposons d'abord que $y_1,\dots ,y_n$ sont $n$ observations consécutives d'un \emph{processus stationnaire par morceaux}, c'est-à-dire qu'il existe des ruptures $0=t_0^\star < t_1^\star < \dots < t_m^\star < t_{m+1}^\star = n$ telles que, pour tout entier $k\in\left\lbrace0,\dots, m\right\rbrace$, $y_{t_k^\star +1},\dots ,y_{t_{k+1}^\star},$ sont des observations consécutives d'un processus faiblement stationnaire. Les ruptures vérifient \eqref{eq:cadre_asymptotique} et les moments d'ordre un et deux du processus sur chaque segment ne varient pas avec $n$, de sorte qu'au $k^e$ segment on peut associer l'espérance $\mu_k^\star$ et la fonction d'autocovariance $\gamma_k^\star$. Notons que si on impose l'égalité de toutes les fonctions d'autocovariance $\gamma_k^\star$, on a un modèle de segmentation de l'espérance tel que décrit dans la section \ref{ch:intro:sec:dep:subs:marginale}.

Ce modèle ne décrit pas les moments d'ordre deux de la série. En particulier, rien n'est dit de la covariance de deux observations séparées par une ou plusieurs ruptures. C'est par exemple le type de modèle considéré par \textcite{davis2006structural}.

La classe de modèles considérée par \textcite{BKW10} est différente. Premièrement, car, même en absence de rupture, les séries peuvent être non-stationnaires et deuxièmement, car le comportement de la série aux ruptures est lui aussi différent. \textcite{BKW10} considèrent des séries $y_1,\dots ,y_n$ qui sont des observations successives d'un processus $\left(y_i\right)_{i\in\mathbb{Z}}$, tel que, pour tout $t_{k-1}^\star<i\leq t_{k}^\star$,
\begin{equation}\label{eq:modele_bardet}
y_i = f_{\theta_k^\star}\left(\left(y_j\right)_{j<i}\right) + m_{\theta_k^\star}\left(\left(y_j\right)_{j<i}\right) \epsilon_i
\end{equation}
où $\left(\epsilon_i\right)_{i\in\mathbb{Z}}$ est une suite de v.a.r. i.i.d. centrées de variance 1 et $\left(f_{\theta}\right)_{\theta\in\Theta}$ et $\left(m_{\theta}\right)_{\theta\in\Theta}$ sont des familles de fonctions. Un tel processus est causal, au sens où chaque observation est fonction du passé et d'un aléa indépendant du passé. \textcite{davis2010consistency} ne proposent qu'un sous-modèle de \eqref{eq:modele_bardet}, où l'équation \eqref{eq:modele_bardet} devient l'équation d'un processus autorégressif dont les coefficients et l'ordre varient entre les segments.

\textcite{BKW10} estiment les ruptures par quasi-maximum de vraisemblance: la fonction de vraisemblance de $\left(y_1,\dots ,y_n\right)$ conditionnelle à $\left(y_j\right)_{j\leq 0}$ que l'on aurait si $\left(\epsilon_i\right)_{i\in\mathbb{Z}}$ était gaussien est maximisée en les paramètres $\theta_k$ et en les instants de rupture. Sous certaines hypothèses de régularité et d'identifiabilité du modèle, \textcite{BKW10} obtiennent les résultats classiques, évoqués dans le cas indépendant dans la section~\ref{ch:intro:sec:indep:subs:frequentiste}, de consistance des estimateurs des ruptures et des autres paramètres, ainsi que le taux de convergence en $1/n$ pour les estimateurs des ruptures $\tau_k^\star$, sous l'hypothèse~\eqref{eq:cadre_asymptotique}.

==> chapitres/intro/dep/marginale.tex <==
On se place dans le modèle \eqref{eq:modele_semiparam}, en supposant les variances constantes, mais sans supposer les observations indépendantes. \textcite{LM} démontrent que, sous certaines conditions, la dépendance entre les observations n'affecte pas la vitesse de convergence des estimateurs des moindres carrés des ruptures et des paramètres $\mu_k^\star$, tels que définis en \eqref{ch:intro:sec:indep:subs:frequentiste:eq:moindres_carres}.

Plus précisément, dans le modèle considéré par \textcite{LM},

\begin{equation}\label{eq:modele_LM}
\forall i\in\left\lbrace 1,\dots ,n\right\rbrace, y_i = \mu_k^\star + \eta_i \textit{ si } t_{k-1}^\star < i \leq t_{k}^\star \; ,
\end{equation}
où les ruptures vérifient la condition \eqref{eq:cadre_asymptotique}. Si la condition
\begin{equation}\label{eq:cond_LM}
\exists \phi < 2, \exists C>0 , \forall j > i >0, \mathbb{E}\left[\left(\sum_{t=i}^j \eta_i\right)^2\right] \leq C \left| j - i +1 \right|^\phi
\end{equation}
est vérifiée, les estimateurs des moindres carrés des ruptures et des paramètres $\mu_k^\star$, \textit{modulo} certaines restrictions de l'ensemble des paramètres considérés dans la minimisation du critère des moindres carrés, sont consistants, les estimateurs des ruptures $\tau_k^\star$ convergeant à la vitesse $1/n$. La condition \eqref{eq:cond_LM} est vérifiée pour une large classe de processus $\left(\eta_i\right)$. Si on se restreint aux processus centrés faiblement stationnaires (cf. définition \ref{def:stationnarite_faible}), elle est vérifiée pour les processus à \emph{courte mémoire}, c'est-à-dire tels que la fonction d'autocovariance associée au processus est absolument sommable, mais aussi pour certains processus à \emph{longue mémoire}. \mbox{\textcite{BP}} avaient déjà démontré le résultat sur les estimateurs des ruptures et des $\mu_k^\star$, notamment dans le cas où $\left(\eta_i\right)_{i\in\mathbb{Z}}$ est un processus centré faiblement stationnaire à courte mémoire. \mbox{\textcite{lavielle1999}} a étendu ces résultats à un cadre plus général que les ruptures de moyennes ainsi qu'à d'autres critères que les moindres carrés.

Concernant la sélection du nombre de ruptures, \textcite{LM} donnent des conditions sur la pénalisation pour obtenir des critères pénalisés consistants. Là aussi, si $\left(\eta_i\right)_{i\in\mathbb{Z}}$ reste un processus centré faiblement stationnaire à courte mémoire, ces conditions ne sont pas affectées par la structure de dépendance.

Les résultats de \textcite{LM}, ainsi que ceux de \textcite{lavielle1999}, pourraient donc plaider pour une non-prise en compte de la dépendance entre observations dans l'estimation des ruptures et la sélection de leur nombre dans un modèle de segmentation, pour peu que la perturbation $\left(\eta_i\right)_{i\in\mathbb{Z}}$ vérifie certaines conditions.

Toutefois, \textcite{LM} montrent que la variance asymptotique des estimateurs des ruptures peut être affectée par la structure de dépendance, y compris si $\left(\eta_i\right)_{i\in\mathbb{Z}}$ reste un processus centré faiblement stationnaire à courte mémoire. De même, \textcite{antoch1997effect} et \textcite{robbins2011mean} ont montré que la dépendance entre observations, y compris sous la forme d'une perturbation qui serait un processus centré faiblement stationnaire à courte mémoire, n'est pas sans effet sur la variance asymptotique de différentes statistiques de test d'une rupture dans l'espérance. La prise en compte de la relation de dépendance stochastique entre observations dans l'estimation des ruptures peut donc s'avérer importante.

==> chapitres/intro/dep/selection.tex <==
Le problème du choix du nombre de ruptures se pose également dans le cas dépendant. La sélection de modèle par contraste pénalisé a été étudiée pour des modèles de ruptures dans la loi marginale ou dans la structure de dépendance par \textcite{LM} et \textcite{BKW10} respectivement. Ces auteurs donnent des conditions suffisantes sur la forme de la pénalité pour garantir la consistance du nombre de ruptures sélectionné. Ces conditions sont cependant très larges et n'aboutissent pas à un critère explicite.

Un critère MDL, fondé sur la théorie de l'information, a également été proposé par \textcite{davis2006structural} dans le cas des modèles avec une autorégression spécifique à chaque segment. \textcite{davis2013} généralisent ce critère à d'autres modèles et en démontrent la consistance sous certaines conditions.

Le critère de \textcite{ZS} est explicitement restreint au cas où les observations sont indépendantes. Dans les chapitres~\ref{ch:ar1} et~\ref{ch:arp}, on propose une adaptation de ce critère pour certaines structures de dépendance sérielle qui conserve les garanties statistiques et l'efficacité algorithmique.

==> chapitres/intro/dep/types.tex <==
Différents types de ruptures peuvent affecter ces séries dépendantes:
\begin{itemize}
\item On pourra toujours considérer des ruptures dans la loi marginale des observations, comme dans la section \ref{ch:intro:sec:indep}, à la différence près que les observations ne sont plus considérées comme indépendantes. Voir~\textcite{lavielle1999}, \textcite{LM} et, dans un cadre plus général que celui présenté ici, \textcite{BP}.
\item On pourra considérer des ruptures dans la structure de dépendance de la série. Certains des modèles considérés sont détaillés dans la section~\ref{ch:intro:sec:dep:subs:autres}.
\item On pourra considérer des ruptures qui affectent à la fois la loi marginale des observations et la structure de dépendance de la série.
\end{itemize}

==> chapitres/intro/indep.tex <==
Dans le cas où les observations sont indépendantes, la segmentation se réduit à la détection de ruptures dans la loi marginale des observations. Formellement,
on dispose de variables aléatoires indépendantes $y_1,\dots ,y_n,$ sur un même espace mesurable. Les ruptures sont alors les entiers $0=t_0<t_1<\dots <t_m < t_{m+1}=n$ tels que pour tout entier $1\leq k \leq m+1$,
\begin{equation*}
\left\lbrace \begin{tabular}{cl}
$y_{t_{k-1} +1},\dots, y_{t_{k}}$ & sont de même loi. \\
$y_i$ et $y_j$ & sont de lois différentes si $k\leq m$ et $t_{k-1} <i \leq t_{k} < j \leq t_{k+1}$.
\end{tabular} \right.
\end{equation*}

\subsection{Typologie des problèmes de segmentation}\label{intro:indep:subs:typologie}
\input{./chapitres/intro/indep/typologie}

\subsection{Modèles}
\input{./chapitres/intro/indep/modeles}

\subsection{Méthodes bayésiennes}
\input{./chapitres/intro/indep/bayesien}

\subsection{Cadre fréquentiste}\label{ch:intro:sec:indep:subs:frequentiste}
\input{./chapitres/intro/indep/frequentiste}

\subsection{Sélection du nombre de ruptures}
\input{./chapitres/intro/indep/selection}

\subsection{Problème algorithmique}\label{ch:intro:sec:indep:subs:algo}
\input{./chapitres/intro/indep/algo}


==> chapitres/intro/indep/algo.tex <==
L'estimation de ruptures multiples par maximum de vraisemblance ou moindres carrés fait apparaître un problème algorithmique. Cette question est centrale en segmentation. Par exemple, \textcites{SSB}{jandhyala2013inference}, dans leur exposé, introduisent l'estimation de ruptures multiples à travers le problème algorithmique que cela pose. En effet, l'exploration de l'ensemble des segmentations prendrait un temps $O\left(n^m\right)$, une complexité algorithmique souvent prohibitive. Pour la recherche de la segmentation optimale, trois approches peuvent alors être considérées:

\begin{itemize}
\item \'Etablir un algorithme efficace donnant la solution optimale. Seul l'algorithme de programmation dynamique \parencites{AugerLawrence}{BPalgo}, ainsi que ses versions élaguées \parencites{pruned}{maidstone2014optimal} permettent de recouvrer la segmentation optimale en un temps polynomial. L'algorithme de partition optimale de \textcite{jackson2005algorithm}, ainsi que ses versions élaguées \parencites{killick2012optimal}{maidstone2014optimal}, fournissent eux aussi la segmentation optimale en réalisant simultanément la sélection du nombre de ruptures, avec certaines contraintes sur le critère de sélection de modèle. Tous ces algorithmes peuvent être utilisés pour peu que le critère à optimiser soit additif sur les segments~(voir section~\ref{ch:outils:sec:algo}).
\item Définir une heuristique fournissant une solution sous-optimale acceptable. La segmentation binaire \parencites(voir par exemple)(){scott1974cluster}{venkatraman1992consistency}{bai1997estimating}  peut être vue comme une suite de tests sur la présence d'une rupture \emph{supplémentaire} à celles qui ont déjà été estimées. Cette contrainte, le fait que les $m$ ruptures estimées dans le modèle à $m$ changements sont incluses dans les $m+1$ ruptures du modèle avec un changement supplémentaire, est très forte et entraîne une sous-exploration de l'ensemble des segmentations possibles, d'où la solution sous-optimale. Le problème est connu et a mené à des raffinements de la méthode \parencites{olshen2004circular}{fryzlewicz2014wild} pour en réduire l'impact.

\textcite{davis2006structural} proposent un algorithme génétique fournissant une solution approchée à la segmentation par minimisation d'un critère MDL~(\emph{Minimum description length}). Toutefois, \textcite{barber2011bayesian} font remarquer que ce critère peut tout aussi bien être minimisé par l'algorithme de programmation dynamique.
\item Modifier le problème d'optimisation pour le rendre résoluble. En segmentation, le Lasso, tel que formulé par \textcite{harchaoui2010}, revient à remplacer la contrainte \enquote{$m$ ruptures} par une contrainte convexe. Là aussi, la modification du problème d'optimisation fait que la segmentation proposée n'est pas optimale au sens du critère initial.
\end{itemize}

Les choix méthodologiques ont été orientés de façon à préserver l'applicabilité de l'algorithme de programmation dynamique, le plus souvent élaguée. Les algorithmes de partition optimale n'ont pas été utilisés car le critère de sélection de modèle que nous avons utilisé ne le permettait pas.

==> chapitres/intro/indep/bayesien.tex <==
Les méthodes bayésiennes en segmentation ont été introduites d'abord dans le cas où il y a au plus une rupture \citep{chernoff1964}, puis dans le cas des modèles à ruptures multiples~\citep{barry1992}. Dans le cadre bayésien, tous les paramètres du modèle, notamment le nombre et la position des ruptures, sont des variables aléatoires, qui suivent une loi à priori.

 L'objectif de l'inférence est alors de fournir les lois à posteriori
\begin{eqnarray*}
P\left(t_1,\dots ,t_m | y_1,\dots ,y_n\right), & & P\left(m | y_1,\dots ,y_n\right) \; .
\end{eqnarray*}

Le calcul de cette loi à posteriori n'est pas nécessairement trivial. Il y a trois façons de procéder:
\begin{itemize}
\item Les lois à priori sont choisies de façon à obtenir des expressions analytiques calculables pour les loi à posteriori \parencite{rigaill2012exact}. Cette approche est classique en statistique bayésienne et fait usage des lois conjuguées.
\item On renonce à obtenir une expression analytique pour la loi à posteriori. Nous n'avons accès à cette loi de probabilité qu'à travers des échantillons simulés de cette loi. La simulation de tels échantillons peut se faire à l'aide de méthodes de Monte-Carlo par chaînes de Markov  \citep{lavielle2001application}, où la loi des échantillons simulés tend vers la loi à posteriori quand le temps d'exécution de l'algorithme tend vers l'infini. Il faut alors être attentif à ce que le temps d'exécution de l'algorithme soit suffisamment long \citep{fearnhead2006exact}. Un autre algorithme, de type \textit{forward-backward}, permet une simulation exacte de la loi à posteriori \citep{fearnhead2006exact}.
\item L'approche asymptotique, pour la loi du nombre de ruptures seulement, qui consiste à fournir une approximation des probabilités à posteriori quand le nombre d'observations $n$ tend vers l'infini. Cette approche a été développée pour l'estimation du nombre de ruptures par \textcite[voir section \ref{ch:outils:sec:selection:subs:seg:subsubs:bic}]{ZS}. Il s'agit de l'adaptation à la segmentation du critère de sélection de modèle proposé par \textcite{schwarz}.
\end{itemize}
Parmi ces trois approches seule la dernière sera abordée.


==> chapitres/intro/indep/frequentiste.tex <==
Avant d'aborder les résultats asymptotiques établis en segmentation, il faut donner un sens à la théorie asymptotique dans ce cadre.

Pour pouvoir établir des résultats de consistance sur les estimateurs des ruptures, nous devons définir la suite des vrais instants de rupture quand la longueur de la série varie.

Un cadre fréquemment adopté et ayant permis d'établir de nombreux résultats asymptotiques \parencites{BP}{Bai}{LM}{BKW10} est le suivant. On considère $\left(y_{i,n}\right)_{1\leq i\leq n, n\geq n_0}$. Pour chaque $n\geq n_0$, $\left(y_{i,n}\right)_{1\leq i\leq n}$ est une série affectée par des ruptures. On suppose qu'il existe $0 = \tau_0^\star < \tau_1^\star < \dots < \tau_m^\star < \tau_{m+1}^\star = 1$, tels que, pour tout $n\geq n_0$, les ruptures de la série $\left(y_{i,n}\right)_{1\leq i\leq n}$  sont localisées en
\begin{equation}\label{eq:cadre_asymptotique}
t_{k,n}^\star = \left\lfloor n\tau_k^\star \right\rfloor \; (1\leq k \leq m) \; .
\end{equation}
Ainsi, les instants de rupture sont des fractions de la longueur totale de la série. Les paramètres à estimer correspondant aux instants de rupture sont donc $\tau_1^ \star, \dots ,\tau_m^\star$, des réels compris entre $0$ et $1$. On considère que le nombre de ruptures ne varie pas avec la taille des séries.

C'est le cadre sous-jacent de la plupart des travaux concernant l'estimation des instants de rupture en statistique fréquentiste depuis le début des années 1990, même si $\left(y_{i,n}\right)_{1\leq i\leq n, n\geq n_0}$ n'est pas explicitement défini de façon systématique. En général, on définit une série $y_1,\dots ,y_n$, puis on fait tendre $n$ vers l'infini pour obtenir des résultats asymptotiques. En réalité, cela n'a de sens qu'à travers $\left(y_{i,n}\right)_{1\leq i\leq n, n\geq n_0}$.

Illustrons cette construction dans le cas gaussien. On considère le modèle défini à $n$ fixé par l'équation \eqref{eq:modele_gaussien}, avec la contrainte supplémentaire d'avoir toutes les variances égales~(à~$\sigma^{\star 2}$). Soit $0 = \tau_0^\star < \tau_1^\star < \dots < \tau_m^\star < \tau_{m+1}^\star = 1$ et $\left(\epsilon_t\right)_{0<t\leq 1, t\in\mathbb{Q}}$ une famille de v.a.r. i.i.d. gaussiennes centrées de variance $\sigma^{\star 2}$. Soit $\mu:\left(0,1\right]\rightarrow \mathbb{R}$ définie par
$$ \forall t\in \left(0,1\right], \mu (t) = \sum_{k=0}^m \mu_k^\star \mathbf{1}_{\left(\tau_k^\star, \tau_{k+1}^\star\right]} (t) \; . $$

Pour tout $n$, la loi de $\left(y_{i,n}\right)_{1\leq i\leq n}$ est donnée par:
$$ \left(y_{i,n}\right)_{1\leq i\leq n} \overset{d}{=} \left(\mu\left(\frac{i}{n}\right) + \epsilon_{i/n}\right)_{1\leq i\leq n} \; . $$

\subsubsection{Estimation par maximum de vraisemblance}

On se place dans le modèle défini par \eqref{eq:modele_parametrique} et le cadre asymptotique défini par \eqref{eq:cadre_asymptotique}. Supposons que les lois de probabilité $P_\theta$ admettent une densité $f_\theta$ par rapport à une certaine mesure de référence. L'estimateur du maximum de vraisemblance des ruptures et des paramètres au sein de chaque segment est alors
\begin{equation}
\left(\widehat{t}_1,\dots ,\widehat{t}_m, \widehat{\theta}_0,\dots ,\widehat{\theta}_m\right) = \underset{\underset{\theta_0,\dots ,\theta_m\in\Theta}{0=t_0<t_1<\dots <t_m<t_{m+1}=n}}{\argmax} \quad \prod_{k=0}^m\prod_{i=t_k+1}^{t_{k+1}} f_{\theta_k}\left(y_k\right) \; .
\end{equation}
La normalisation $\widehat{\tau}_k = \widehat{t}_k/n$ donne des estimateurs des ruptures $\tau_k^\star$. \textcite{he2010asymptotic} ont démontré, sous certaines conditions de régularité, que les estimateurs $\widehat{\tau}_k$ sont consistants et convergent à l'ordre $1/n$. De plus, les estimateurs des paramètres $\widehat{\theta}_k$ sont eux aussi consistants et conjointement asymptotiquement normaux, y compris conjointement à un éventuel paramètre global.

\subsubsection{Estimation par moindres carrés}
On se place dans le modèle \eqref{eq:modele_semiparam}, avec une variance constante, et le cadre asymptotique défini par \eqref{eq:cadre_asymptotique}. L'estimateur des moindres carrés des ruptures et des espérances est alors:
\begin{equation}\label{ch:intro:sec:indep:subs:frequentiste:eq:moindres_carres}
\left(\widehat{t}_1,\dots ,\widehat{t}_m, \widehat{\mu}_0,\dots ,\widehat{\mu}_m\right) = \underset{\underset{\mu_0,\dots ,\mu_m}{0=t_0<t_1<\dots <t_m<t_{m+1}=n}}{\argmin} \quad \sum_{k=0}^m\sum_{i=t_k+1}^{t_{k+1}} \left(y_i - \mu_k\right)^2 \; .
\end{equation}
À ma connaissance, les premiers résultats asymptotiques dans ce cadre sont ceux de \textcite{yao1989least}. \textcite{LM} fournissent des résultats similaires à ceux de \textcite{he2010asymptotic} pour l'estimateur du maximum de vraisemblance dans ce cas.

\subsubsection{Estimation par maximum de vraisemblance gaussienne}
On se place dans le modèle \eqref{eq:modele_semiparam} et le cadre asymptotique défini par \eqref{eq:cadre_asymptotique}. Les ruptures et les autres paramètres peuvent être estimés par maximisation de la vraisemblance gaussienne, qui est la fonction de vraisemblance associée au modèle \eqref{eq:modele_gaussien}. Même si les observations ne sont pas gaussiennes, \textcite{lavielle1999} garantit sous certaines conditions la consistance des estimateurs et des vitesses de convergences de même ordre que celles de \textcite{he2010asymptotic}.

==> chapitres/intro/indep/modeles.tex <==
Dans la section~\ref{intro:indep:subs:typologie}, nous n'avons fixé aucune condition sur les lois marginales possibles des observations. Or il existe bien souvent une modélisation préalable de la série.

On peut se donner un modèle paramétrique $\left(P_\theta\right)_{\theta\in\Theta}$ et fixer comme condition
\begin{equation}\label{eq:modele_parametrique}
\forall k \in \left\lbrace 1,\dots,m+1\right\rbrace,\left( \forall i \in\left\lbrace t_{k-1}^\star +1,\dots,t_{k}^\star\right\rbrace, y_i\sim P_{\theta_k^\star} \textit{ et } k\leq m \Rightarrow \theta_k^\star \neq \theta_{k+1}^\star \right) \; .
\end{equation}

On peut ajouter à ce modèle un paramètre global, qui reste constant sur tous les segments. Par exemple, le modèle gaussien est ici:

\begin{equation}\label{eq:modele_gaussien}
\forall k \in \left\lbrace 1,\dots,m+1\right\rbrace, \forall i \in\left\lbrace t_{k-1}^\star +1,\dots,t_{k}^\star\right\rbrace, y_i \sim \mathcal{N}\left(\mu_k^\star,\sigma_k^{\star 2}\right) \; .
\end{equation}
Le modèle peut être restreint au cas où toutes les variances $\sigma_k^{\star 2}$ sont égales, ce qui fait de cette variance commune un paramètre global du modèle. De même, on peut se restreindre au cas où toutes les espérances sont égales. Dans le premier cas, on segmente dans l'espérance, dans le second cas, dans la variance (voir figure~\ref{fig:exemple_types_ruptures}).

\begin{figure}[!b]
\centering
\includegraphics[width=0.75\textwidth]{casruptures.pdf}
\caption[Séries dans différents modèles de segmentation gaussiens.]{Réalisation de 4 séries de 60 v.a.r. indépendantes de loi normale. Les droites verticales indiquent les ruptures éventuelles, localisées en 30 et 40. Haut, gauche: cas i.i.d. centré réduit. Haut, droite: variance constante égale à 1, ruptures dans l'espérance~(0, 4 puis~2). Bas, gauche: espérance constante égale à 0, ruptures dans la variance~(1, 16 puis~1/16). Bas, droite: ruptures simultanées dans l'espérance et la variance, avec les mêmes valeurs que précédemment.}\label{fig:exemple_types_ruptures}
\end{figure}

Il peut être préférable dans certains cas d'étendre le modèle. On peut simplement demander à ce que certaines quantités associées aux lois marginales soient constantes sur les segments. Par exemple, par analogie avec le modèle gaussien, on peut considérer le modèle suivant:
\begin{equation}\label{eq:modele_semiparam}
\forall k \in \left\lbrace 1,\dots,m+1\right\rbrace, \forall i \in\left\lbrace t_{k-1}^\star +1,\dots ,t_{k}^\star\right\rbrace, y_i \textit{ est de carré intégrable, } \mathbb{E}y_i = \mu_k^\star, \mathrm{Var}\left(y_i\right) = \sigma_k^{\star 2} \; .
\end{equation}
Tous les sous-modèles définis dans le cas gaussien peuvent être définis de façon analogue. Dans le cas où l'on segmente dans l'espérance, il s'agit d'un modèle de régression non-linéaire, où la fonction de régression est constante par morceaux. Si les instants de rupture étaient connus, il s'agirait d'un modèle linéaire.

==> chapitres/intro/indep/selection.tex <==
On a supposé jusqu'ici le nombre de ruptures $m$ connu. Mais, dans la plupart des applications, il doit être estimé, ce qui nous amène à un problème de sélection de modèle. Des critères de différents types ont été proposés:
\begin{itemize}
\item des procédures séquentielles de tests \citep{BP},
\item des approches par contraste pénalisé dans un cadre fréquentiste \parencites{yao}{lee1995}{lebarbier2005detecting},
\item des approches bayésiennes \parencites{ZS}{rigaill2012exact}.
\end{itemize}

Une présentation plus détaillée de ces différentes approches est donnée dans la section~\ref{ch:outils:sec:selection}. Si l'estimation des instants de rupture et des paramètres des lois marginales est un problème bien compris à $m$ connu, l'estimation de ce dernier reste un problème difficile. La définition même du \enquote{bon} ou du \enquote{vrai} $m$ à sélectionner n'est pas consensuelle. De plus, les résultats asymptotiques ne suffisent pas toujours à déterminer une procédure pratique, notamment quand des constantes de pénalisation restent à calibrer.

Dans ce travail, on porte une attention particulière au critère de \mbox{\textcite{ZS},} qui est défini indépendamment de toute constante, et qui fournit de bons résultats pratiques~\parencites{picard2011joint}{frick2014multiscale}.

==> chapitres/intro/indep/typologie.tex <==
Historiquement, les problèmes de segmentation sont apparus comme le problème de la détection d'une rupture \parencites{page1954continuous}{page1955test}. Il s'agit alors de tester
\begin{eqnarray*}
H_0 : & & y_1,\dots ,y_n \textit{ identiquement distribués } \\
 \textit{ contre } & & \\
 H_1: & \exists t\in\left\lbrace 1,\dots ,n-1\right\rbrace , & \left\lbrace \begin{tabular}{cc}
 $y_1,\dots ,y_t$ & \textit{ identiquement distribués }, \\
 $y_{t+1},\dots ,y_n$ & \textit{ identiquement distribués }, \\
 $y_1$ \textit{ et } $y_n$ & \textit{ sont de lois différentes.}
\end{tabular}\right.
\end{eqnarray*}
Des conditions supplémentaires sur la loi des observations (appartenance à un certain modèle,~etc.) peuvent être fixées. Si l'hypothèse nulle $H_0$ est rejetée, il est aussi question d'estimer l'instant de rupture $t$.
La détection de rupture peut être \emph{séquentielle}~(\emph{on-line}) ou \emph{rétrospective}~(\emph{off-line}). Dans le premier cas, la taille $n$ de la série croît et pour chaque $n$ on teste la présence d'une rupture ou non \parencite[voir par exemple][]{Bas93N}. Typiquement, il s'agit de réaliser un compromis entre la détection à temps d'une rupture et la nécessité d'éviter les fausses alarmes. Dans le cas de la détection de rupture rétrospective, la totalité de la série $y_1,\dots ,y_n$ est observée et, à posteriori, on teste la présence d'une rupture. La détection de rupture séquentielle et les problèmes spécifiques qu'elle pose ne seront pas abordés dans cette thèse.

Si le cas où au moins deux ruptures peuvent être présentes est possible, on parle alors de \emph{détection de ruptures multiples} ou de \emph{segmentation à ruptures multiples}. La méthodologie du cas où il y a au plus une rupture dans la série peut être adaptée. En particulier, comme \textcite{BP}, on peut tester l'absence de rupture contre la présence de $m$ ruptures, ou bien la présence de $m$ ruptures contre la présence de $m+1$ ruptures. Toutefois, en cas de ruptures multiples, l'estimation du nombre de ruptures par l'intermédiaire de ces tests mène à un problème complexe de tests multiples. Une méthode fréquemment adoptée consiste à
\begin{itemize}
\item dans le modèle à $m$ ruptures, estimer les instants de ruptures ainsi que les autres paramètres du modèle,
\item sélectionner un modèle à $m$ de ruptures, à l'aide d'une procédure de sélection de modèle.
\end{itemize}
Toutefois, certaines méthodes bayésiennes \parencite{lavielle2001application} ou fréquentistes \parencite[comme le Lasso, pour \emph{Least absolute shrinkage and selection operator}, voir][]{harchaoui2010} réalisent ces deux étapes simultanément.

Dans cette thèse, nous nous intéressons à la segmentation rétrospective à ruptures multiples.

==> chapitres/notations.tex <==
\paragraph{Abréviations latines usuelles en français ou en anglais:} \textit{cf., e.g., et al., i.e.}

\section*{Abréviations en français}

\begin{tabular}{lr}
càdlàg & continu à droite et limité à gauche\\
i.i.d. & indépendants et identiquement distribués\\
resp. & respectivement\\
v.a. & variable aléatoire\\
v.a.r. & variable aléatoire réelle
\end{tabular}

\section*{Abréviations en anglais}

\begin{tabular}{lr}
AIC & Akaike information criterion\\
AICc & Akaike information criterion corrected\\
AO & Additive outliers\\
ARMA & Autoregressive-moving-average\\
BIC & Bayesian information criterion\\
cdf & cumulative distribution function\\
DP & Dynamic programming\\
iid & independent and identically distributed\\
IQR & Interquartile range\\
Lasso & Least absolute shrinkage and selection operator\\
MAD & Median absolute deviation\\
mBIC & Modified Bayesian information criterion\\
MDL & Minimum description length\\
NGS & Next-generation sequencing\\
rv & random variable\\
SNIP & Segment neighborhood with inequality pruning
\end{tabular}

\newpage
\section*{Symboles}
Dans tout le document, les variables aléatoires ont pour espace de départ un même espace probabilisé $\left(\Omega,\mathcal{A},P\right)$.


\vspace{1cm}
\begin{tabular}{ll}
$\nset, \zset, \mathbb{Q}, \rset, \cset$ & ensembles usuels\\
$\delta_{x,y}$ & Symbole égal à 1 si et seulement si $x=y$,\\
& égal à 0 sinon.\\
$\sharp$ & cardinal\\
$C_n^k$ & coefficient binomial $k$ parmi $n$\\
$\left[a,b\right)$ & intervalle $\left\lbrace x\in\rset ; a\leq x < b\right\rbrace$\\
$\argmin, \argmax$ & argument resp. minimum et maximum\\
$\log$ & logarithme népérien\\
$\lfloor\cdot\rfloor, \lceil\cdot\rceil$ & partie entière resp. inférieure et supérieure\\
$\Vert\cdot\Vert$ & Norme, supposée euclidienne sauf\\
& mention du contraire.\\
$\pi_E$ & projection orthogonale sur le sous-espace vectoriel $E$\\
$A^T$ & transposée de la matrice $A$\\
$\lim$ & limite\\
$\underline{\lim}$ & limite inférieure\\
$u_n = O(v_n), u_n = o(v_n)\; (n\rightarrow\infty)$ & $(u_n)$ est resp. dominée par $(v_n)$\\
& et négligeable devant $(v_n)$ en $+\infty$.\\
$\mathbb{E}$ & espérance\\
$\mathrm{Var}$ & variance\\
$\mathrm{Cov}$ & covariance\\
$\mathcal{N}\left(m,\sigma^2\right)$ & loi normale d'espérance $m$ et de variance $\sigma^2$\\
$\mathcal{N}\left(\boldsymbol{m},\Sigma\right)$ & loi normale multivariée d'espérance $\boldsymbol{m}$\\
& et de matrice de variance/covariance $\Sigma$\\
$\chi^2(d)$ & loi du chi-deux à $d$ degrés de liberté\\
$\overset{p.s.}{=}$ & égalité presque-sûre\\
$\overset{d}{=}$ & égalité en loi\\
$\overset{d}{\underset{n\rightarrow\infty}{\longrightarrow}}$ & convergence en loi\\
$\overset{P}{\underset{n\rightarrow\infty}{\longrightarrow}}$ & convergence en probabilité\\
$X_n = O_P\left(Y_n\right), o_P\left(Y_n\right)\; (n\rightarrow\infty)$ & $(X_n/Y_n)$ est resp. bornée en probabilité\\
 & et convergente en probabilité vers 0 en $+\infty$.
\end{tabular}

==> chapitres/outils.tex <==
\section{Séries temporelles}
\input{./chapitres/outils/series}

\section{Processus empirique et Delta-méthode fonctionnelle}
\input{./chapitres/outils/processus_delta}

\section{Estimation robuste}
\input{./chapitres/outils/robuste}

\section{Inégalités maximales}
\input{./chapitres/outils/inegalites}

\section{Sélection de modèle}\label{ch:outils:sec:selection}
\input{./chapitres/outils/selection}

\section{Problèmes algorithmiques en segmentation}\label{ch:outils:sec:algo}
\input{./chapitres/outils/algo}


==> chapitres/outils/algo.tex <==
Les questions algorithmiques occupent une place importante en segmentation. La recherche de la segmentation optimale (en un sens à préciser) mène à un problème d'optimisation discrète sur un ensemble fini pouvant être de grande taille, qui ne peut être résolu en un temps raisonnable par l'exploration totale de cet ensemble.

Il s'agit de trouver la segmentation optimale (en un sens à préciser) à $m$ ruptures d'une série temporelle $\boldsymbol{y}= \left(y_1,\dots ,y_N\right)$, où $m+1\leq N$. On ne fixe pas à priori de restriction sur l'ensemble auquel appartiennent ces observations.

Définissons, pour $1\leq k+1 \leq  \min (m+1 , n) \leq \max (m+1 , n) \leq N$,

\begin{equation}\label{eq:minProblemAL}
C_{k,n} = \underset{\boldsymbol{t}=(t_0,\dots,t_{k+1})\in\mathcal{A}_{n,k}}{\min} \; \underset{\boldsymbol{\theta}=\left(\theta_1,\dots,\theta_{k+1}\right)\in \Theta^{k+1}}{\min} \sum_{l=1}^{k+1} f_{t_{l-1}+1,t_l}(\boldsymbol{y} ,\theta_l) \; ,
\end{equation}
où:
\begin{itemize}
\item $\mathcal{A}_{n,k} = \left\lbrace (t_0,\dots,t_{k+1})\in \mathbb{N}^{k+2} ; \; 0=t_0<t_1<\dots <t_k <t_{k+1}=n\right\rbrace.$ C'est l'ensemble des segmentations à $k$ ruptures d'une série à $n$ observations.
\item On ne fixe pas de restriction à priori à l'ensemble $\Theta$. À ce niveau, la seule contrainte sur l'ensemble sur lequel se fait la minimisation en $\boldsymbol{\theta}$ est d'être un produit cartésien $\Theta^{k+1}$.
\item Les fonctions $f_{i,j} \; (1\leq i\leq j\leq N)$ dépendent des observations et d'un paramètre ($\theta_l$ pour le $l^e$ terme de la somme). Ces fonctions sont inférieurement bornées. On souhaite que la minimisation de ces fonctions en le paramètre $\theta_l$ ne soit pas trop coûteuse (en un sens à préciser).
\end{itemize}

$C_{k,n}$ est le \emph{coût} de la segmentation optimale à $k$ ruptures de $y_1,\dots ,y_n$. Le but est de calculer $C_{m,N}$, ainsi que la segmentation $\boldsymbol{t}$ et le paramètre $\boldsymbol{\theta}$ qui réalisent ce minimum. Une fois calculée la segmentation optimale $\boldsymbol{\widehat{t}}$, il est facile de retrouver le paramètre optimal $\boldsymbol{\widehat{\theta}}$  par
$$\widehat{\theta}_l =\underset{\theta_l\in\Theta}{\argmin} f_{\widehat{t}_{l-1}+1,\widehat{t}_l}(\boldsymbol{y} ,\theta_l) \; .$$
Le problème est donc essentiellement de retrouver la segmentation optimale. Or, l'ensemble $\mathcal{A}_{N,m}$ est de cardinal $C_{N-1}^m$. Tester chaque segmentation possible peut être très coûteux en temps de calcul. C'est notamment le cas dans certaines applications en génomique où $N$ est d'ordre $10^5$ ou $10^6$. L'algorithme de programmation dynamique d'\textcite{AugerLawrence}, décrit dans la section~\ref{subs:DPA}, permet de résoudre ce problème.
Pour $1\leq i \leq j \leq N$, on définit:
$$C(i,j) = \min_{\theta\in \Theta} f_{i,j}(\boldsymbol{y},\theta) \; .$$
Ainsi
\begin{equation}\label{eq:minHalfProblemAL}
C_{k,n} = \underset{\boldsymbol{t}=(t_0,\dots,t_{k+1})\in\mathcal{A}_{n,k}}{\min} \sum_{l=1}^{k+1} C(t_{l-1}+1,t_l) \; .
\end{equation}
Si la \emph{matrice de coût} $\left(C(i,j)\right)_{1\leq i \leq j \leq N}$ est connue, le problème d'optimisation est simplifié.

\subsection{Programmation dynamique}\label{subs:DPA}
\input{./chapitres/outils/algo/DPA}
\subsection{Programmation dynamique élaguée}\label{subs:PDPA}
\input{./chapitres/outils/algo/PDPA}

==> chapitres/outils/algo/DPA.tex <==
La programmation dynamique a été introduite par \textcite{bellman1954theory}. Sa philosophie est résumée par le Principe d'optimalité de Bellman:

\enquote{Une politique optimale a la propriété que, quels que soient l'état initial et les décisions initiales, les décisions restantes doivent constituer une politique optimale vis-à-vis du résultat des décisions précédentes.} \textcite{bellman1954theory}.

L'utilisation de la programmation dynamique en segmentation a été introduite par \textcite{AugerLawrence}. %%% Réponse à EL et CLL: Bellman cité.

Pour calculer $C_{m,N}$, on calcule $C_{k,n}$ pour tous $k,n$ tels que $1\leq k+1\leq \min(m+1,n) \leq \max(m+1,n)\leq N$. \eqref{eq:minHalfProblemAL} donne une relation de récurrence:
\begin{eqnarray}
C_{k,n} & = & \underset{s=k,\dots ,n-1}{\min} \underset{(t_0,\dots,t_{k+1})\in\mathcal{A}_{n,k}, t_k = s}{\min}  \sum_{l=1}^{k+1} C\left(t_{l-1}+1,t_l\right) \nonumber \\
 & = & \underset{s=k,\dots ,n-1}{\min} \left\lbrace C(s+1,n)+\underset{(t_0,\dots,t_{k+1})\in\mathcal{A}_{n,k}, t_k = s}{\min}  \sum_{l=1}^{k} C\left(t_{l-1}+1,t_l\right)\right\rbrace \nonumber \\
 & = & \underset{s=k,\dots ,n-1}{\min} \left\lbrace C(s+1,n)+\underset{(t_0,\dots,t_{k})\in\mathcal{A}_{s,k-1}}{\min}  \sum_{l=1}^{k} C\left(t_{l-1}+1,t_l\right)\right\rbrace \nonumber \\
  & = & \underset{s=k,\dots ,n-1}{\min} \left\lbrace C(s+1,n)+C_{k-1,s}\right\rbrace \; . \label{eq:recDPA}
\end{eqnarray}
Cette relation permet d'écrire l'algorithme de programmation dynamique pour le calul de $C_{m,N}$ (cf. algorithme~\ref{alg:DPA}).

\begin{algorithm}%[H]
\Begin{\tcp{Calcul de la matrice de coût:}
 \For{$ i = 1, \dots , N$}{
\For{$ j = i, \dots , N$}{ Calculer $C(i,j)$
} }
\tcp{Initialisation:}%%%EDIT: rép à SR: je ne comprends pas ce qui t'interpelle dans l'initialisation.
\For{$ i = 1, \dots , N$}{$C_{0,n}:=C(1,n)$}
\tcp{Récurrence:}
\For{$ k = 1, \dots , m$}{\For{$ n = k+1, \dots , N$}{$C_{k,n}:=\underset{s=k,\dots ,n-1}{\min} \left\lbrace C(s+1,n)+C_{k-1,s}\right\rbrace$}}
}
\caption{Segmentation par programmation dynamique.} \label{alg:DPA} 
\end{algorithm} 
 
\subsubsection{Complexité en temps et en espace}

La complexité en temps des phases d'initialisation et de récurrence de l'algorithme \ref{alg:DPA} est en $O(mN^2)$. Si le calcul de la matrice de coût est en $O(N^2)$, la complexité en temps de l'ensemble de l'algorithme est en $O(mN^2)$. Il n'est pas possible d'obtenir une telle borne si le problème est posé en toute généralité comme dans l'équation \eqref{eq:minProblemAL}. Cette borne est vraie dans un certain nombre de cas comme celui des moindres carrés (cf. exemple \ref{ex:LS}). Pour obtenir une borne de ce type, il suffit que, pour tous $1\leq i\leq j < N$, $C(i,j+1)$ se calcule en temps borné (avec une complexité en $O(1)$) à partir de $C(i,j)$ et éventuellement d'un nombre borné d'autres variables calculées en même temps que $C(i,j)$ en temps borné; et que les $C(i,i)$ se calculent aussi en temps borné.

La complexité en espace, à priori en $O(N^2)$ à cause de la matrice de coût, peut être réduite à $O(mN)$ \citep{guedon2013exploring} en calculant les termes de cette matrice au fur et à mesure, le long de l'algorithme, en utilisant une relation de récurrence.

\subsubsection{Retour sur trace}

Sous cette forme, l'algorithme \ref{alg:DPA} permet de calculer le coût de la segmentation optimale, mais n'a pas comme sortie la segmentation optimale elle-même. Cet algorithme est complété par une procédure de retour sur trace (\emph{backtracking} en anglais, le retour sur les décisions prises dans l'exécution de l'algorithme) qui permet de reconstruire cette dernière. Par exemple, \textcite{guedon2013exploring} en donne le pseudo-code, cf. l'algorithme~\ref{alg:backtracking}.

On calcule $T(k,n)$ pour tous $1\leq k\leq m, k+1\leq n\leq N$, défini par
$$T(k,n) = \underset{s=k,\dots ,n-1}{\argmin} \left\lbrace C(s+1,n)+C_{k-1,s}\right\rbrace \; .$$

$T(k,n)$ est calculé en même temps que $C_{k,n}$ dans l'algorithme \ref{alg:DPA}. Cette matrice $T$ permet de reconstruire la segmentation optimale à la fin de l'exécution de l'algorithme \ref{alg:DPA}.

\begin{algorithm}%[H]
\Begin{
\begin{eqnarray*}
Seg & := & N\\
s & := & N\\
k & := & m
\end{eqnarray*}
\While{$k>0$}{
\begin{eqnarray*}
s & := & T(k,s)\\
Seg & := & s\parallel Seg \\
k & := & k-1
\end{eqnarray*}} \tcp{$\parallel$ est l'opérateur de concaténation.}
\Return{$Seg$} \tcp{Sortie: Segmentation optimale.}
}
\caption{Retour sur trace.} \label{alg:backtracking} 
 \end{algorithm} 


\subsubsection{Exemples}
\begin{exemple}[Moindres carrés]\label{ex:LS}
Dans cet exemple:
\begin{itemize}
\item $y_1,\dots ,y_N\in\mathbb{R}$,
\item $\Theta = \mathbb{R}$,
\item Les fonctions $f_{i,j}$ sont définies par $\forall \mu\in\mathbb{R},f_{i,j}(\boldsymbol{y},\mu)=\sum_{s=i}^j (y_i - \mu)^2$.
\end{itemize}
Ainsi il s'agit de calculer
$$C_{m,N}=\underset{\boldsymbol{t}=(t_0,\dots,t_{m+1})\in\mathcal{A}_{N,m}}{\min} \underset{\boldsymbol{\mu}=\left(\mu_1,\dots,\mu_{m+1}\right)\in\mathbb{R}^{m+1}}{\min} \sum_{k=1}^{m+1}\sum_{i=t_{k-1}+1}^{t_k} \left(y_i - \mu_k\right)^2 \; .$$

Pour tous $1\leq i\leq j\leq N$,
$$C(i,j) = \sum_{s=i}^j (y_s - \overline{y}_{i:j})^2 \; ,$$
où $\overline{y}_{i:j}=(j-i+1)^{-1}\sum_{s=i}^j y_s$.

En particulier, $\forall i=1,\dots ,N, C(i,i)=0$ et pour tous $1\leq i\leq j < N$,

\begin{eqnarray}
\sum_{s=i}^{j+1}y_s & = & \left(\sum_{s=i}^j y_s\right) + y_{j+1} \; , \label{eq:LaMiseaJourlaPlusSimpleduMonde}\\
C(i,j+1) & = & \frac{j-i+1}{j-i+2}\left\lbrace C(i,j) + y_{j+1}^2 \right\rbrace - \frac{2}{j-i+2}y_{j+1}\sum_{s=i}^j y_s \; . \label{eq:MaJCij}
\end{eqnarray}

Si, en même temps que $C(i,j)$, on calcule $\sum_{s=i}^j y_s$, qui se met à jour très simplement en temps borné (cf. équation \eqref{eq:LaMiseaJourlaPlusSimpleduMonde}), la formule de récurrence \eqref{eq:MaJCij} permet le calcul en temps borné de $C(i,j+1)$ en fonction de $C(i,j)$ et de $\sum_{s=i}^j y_s$. Cela garantit le calcul de la matrice de coût en un temps $O(N^2)$, ce qui garantit la complexité en temps de l'algorithme \ref{alg:DPA} en $O(mN^2)$ dans cet exemple.
\end{exemple}

\begin{exemple}[Vraisemblance conditionnelle gaussienne $AR(1)$ avec ruptures dans le paramètre d'autorégression]
Supposons que $Y_0,\dots ,Y_N$ vérifient
$$Y_i = \rho_l Y_{i-1} + \epsilon_i \textit{ si } t_{l-1}<i\leq t_l \; ,$$
où les $\rho_l\in\mathbb{R}$ sont inconnus,  les $\epsilon_i$ sont normales, centrées, de variance $\sigma^2$ inconnue, i.i.d. Soient $y_0,\dots ,y_N$ des réalisations de $Y_0,\dots ,Y_N$. Maximiser la vraisemblance conditionnellement à $Y_0=y_0$, si l'on considère que cette fonction est déjà maximisée en $\sigma^2$, se ramène au problème de minimisation:
\begin{equation}\label{eq:ar1breaksinrho}
\underset{\boldsymbol{t}=(t_0,\dots,t_{m+1})\in\mathcal{A}_{N,m}}{\min} \underset{\left(\rho_1,\dots,\rho_{m+1}\right)\in \mathbb{R}^{m+1}}{\min} \sum_{l=1}^{m+1} \sum_{i=t_{l-1}+1}^{t_l}\left(y_i-\rho_l y_{i-1}\right)^2 \; .
\end{equation}
On notera que dans cet exemple, contrairement aux moindres carrés, le $l^e$ terme de la somme de l'équation \eqref{eq:ar1breaksinrho} dépend d'une observation $y_i$ avec $i\not\in \left\lbrace t_{l-1}+1, \dots ,t_l\right\rbrace$.
\end{exemple}


Les conditions minimales sur les termes de la somme de l'équation \eqref{eq:minProblemAL} pour pouvoir utiliser l'algorithme \ref{alg:DPA} sont, pour tout $l$, que le $l^e$ terme ne dépende pas:
\begin{itemize}
\item des $t_r$ avec $r\not\in \left\lbrace l-1, l\right\rbrace$,
\item des $\theta_r$ avec $r\neq l$.
\end{itemize}

\begin{exemple}[Vraisemblance gaussienne $AR(1)$ avec ruptures dans l'espérance]
Supposons que $Y_0,\dots ,Y_N$ vérifient
\begin{eqnarray*}
Y_i - \mathbb{E}Y_i & = & \rho \left(Y_{i-1}-\mathbb{E}Y_{i-1}\right) + \epsilon_i\\
\mathbb{E}Y_i & = & \mu_l \textit{ si } t_{l-1}<i\leq t_l ,
\end{eqnarray*}
où $\rho\in\mathbb{R}$ est connu, les $\mu_l\in\mathbb{R}$ sont inconnus, les $\epsilon_i$ sont normales, centrées, de variance $\sigma^2$ inconnue, i.i.d. Soient $y_0,\dots ,y_N$ des réalisations de $Y_0,\dots ,Y_N$. Maximiser la vraisemblance conditionnellement à $y_0$, si l'on considère que cette fonction est déjà maximisée en $\sigma^2$, se ramène à minimiser en $\boldsymbol{t}=(t_0,\dots,t_{m+1})\in\mathcal{A}_{N,m}$ et en $\left(\mu_1,\dots,\mu_{m+1}\right)\in \mathbb{R}^{m+1}$ l'expression suivante:
$$\sum_{l=1}^{m+1} \left\lbrace \sum_{i=t_{l_1}+2}^{t_l}\left(y_i-\rho y_{i-1} - (1 - \rho)\mu_l\right)^2 + \left(y_{t_{l_1}+1} - \mu_l - \rho(y_{t_{l-1}} - \mu_{l-1} )\right)^2\right\rbrace \; .$$
La programmation dynamique ne permet pas de résoudre ce problème à cause du produit croisé $\mu_l\mu_{l-1}$ qui apparaît dans le développement de l'expression.
\end{exemple}

De même, cet algorithme ne peut pas être à priori adapté au cas où tous ces termes partagent un même paramètre global. Cette adaptation n'est possible que dans des conditions très particulières où le minimum en ce paramètre global a la propriété de pouvoir s'écrire comme une expression similaire à celle de l'équation \eqref{eq:minProblemAL}, comme dans l'exemple suivant.
\begin{exemple}[Vraisemblance gaussienne et moindres carrés]
Il s'agit de résoudre le problème d'optimisation suivant:
$$\underset{\boldsymbol{t}=(t_0,\dots,t_{m+1})\in\mathcal{A}_{N,m}}{\max}\underset{\sigma>0}{\max} \underset{\left(\mu_1,\dots,\mu_{m+1}\right)\in \mathbb{R}^{m+1}}{\max} \sum_{l=1}^{m+1} \sum_{i=t_{l-1}+1}^{t_l}\log\left\lbrace\frac{1}{\sigma\sqrt{2\pi}}\exp \left(-\frac{1}{2\sigma^2}\left(y_i-\mu_l\right)^2\right)\right\rbrace \; .$$
Le maximum en $\sigma$ est atteint en $\sigma=\left(\frac{1}{N}\sum_{l=1}^{m+1}\sum_{i=t_{l-1}+1}^{t_l} \left(y_i - \mu_l\right)^2\right)^{1/2}$. Maximisé en $\sigma$, le problème se ramène donc au problème d'optimisation suivant:
$$\underset{\boldsymbol{t}=(t_0,\dots,t_{m+1})\in\mathcal{A}_{N,m}}{\max} \underset{\left(\mu_1,\dots,\mu_{m+1}\right)\in \mathbb{R}^{m+1}}{\max} -\frac{N}{2}\left\lbrace \log\left(2\pi\right) + \log\left( \frac{1}{N} \sum_{l=1}^{m+1} \sum_{i=t_{l-1}+1}^{t_l}\left(y_i-\mu_l\right)^2\right)\right\rbrace \; .$$
Ce problème est équivalent aux moindres carrés.
\end{exemple}

\begin{exemple}[Vraisemblance binomiale négative]\label{outils:algo:exemple:negbin}
Ici, il s'agit de résoudre le problème d'optimisation suivant:
$$\underset{\boldsymbol{t}=(t_0,\dots,t_{m+1})\in\mathcal{A}_{N,m}}{\min}\underset{r>0}{\min} \underset{\boldsymbol{\mu}=\left(\mu_1,\dots,\mu_{m+1}\right)\in \left]0,+\infty\right[^{m+1}}{\min} \sum_{l=1}^{m+1} \sum_{i=t_{l-1}+1}^{t_l}\log\left\lbrace \frac{(r+\mu_l)^{r+y_i}y_i!\Gamma (r)}{r^r\mu_l^{y_i}\Gamma (r+y_i)}\right\rbrace \; , $$
où $\Gamma$ est la fonction Gamma d'Euler. La programmation dynamique ne permet pas de résoudre ce problème de minimisation. Mais si le paramètre $r$ est connu, la minimisation en $\boldsymbol{\mu}$ peut se faire à l'aide de l'algorithme \ref{alg:DPA}.
\end{exemple}

==> chapitres/outils/algo/PDPA.tex <==
L'élagage est une technique qui permet d'accélérer des algorithmes basés sur des disjonctions de cas (\enquote{Diviser pour régner}, programmation dynamique). L'idée est de se donner une variable, facile à mettre à jour durant l'exploration de l'ensemble des possibilités, qui, si elle remplit un certain critère, considère un des sous-cas envisagés comme ne contenant pas l'optimum recherché. Cette variable peut être un nombre, une fonction ou un ensemble.

\textcite{pruned} utilise l'élagage pour accélérer l'algorithme de programmation dynamique pour la segmentation. Cet algorithme a été implémenté pour plusieurs fonctions de coût dans un package R nommé \texttt{Segmentor3IsBack} \citep{cleynen2014segmentor3isback}.

Cet algorithme peut s'utiliser dans le cas particulier du problème de minimisation de l'équation \eqref{eq:minProblemAL}, où
\begin{equation}\label{eq:conditionC1_PDPA}
f_{i,j}(\boldsymbol{y},\theta) = \sum_{s=i}^{j} \gamma \left(y_s , \theta\right) \; .
\end{equation}

Au lieu de calculer directement les $C_{k,n}$, nous nous intéressons à un problème de minimisation fonctionnelle plus complexe:
$$R_{k,n}(\theta) = \underset{\nu=k,\dots ,n-1}{\min} R_{k,\nu,n}(\theta) \; ,$$

où

$$R_{k,\nu,n}(\theta) = C_{k-1,\nu} +  \sum_{i=\nu +1}^{n} \gamma \left(y_i , \theta\right) \; .$$

Les $C_{k,n}$ et les $R_{k,n}$ sont liés par la relation $C_{k,n} = \underset{\theta}{\min} R_{k,n} (\theta)$.

La relation de récurrence \eqref{eq:recDPA} permet de calculer $C_{k,n}$ avec une complexité en $O(n)$. La relation de récurrence suivante permettrait de calculer $R_{k,n}(\theta)$ en temps borné:
\begin{equation}\label{eq:recPDPA}
R_{k,n}(\theta) = \min\left\lbrace R_{k,n-1}(\theta), C_{k-1,n-1}+\gamma (y_n ,\theta ) \right\rbrace \; .
\end{equation}
Le problème est qu'il est impossible de faire ce calcul pour tous les $\theta$ envisagés (possiblement une infinité).

Il est en revanche possible de déterminer l'ensemble $\mathcal{S}_{n,n-1}^k$ des $\theta$ tels que $C_{k-1,n-1}+\gamma (y_n ,\theta )\leq R_{k,n}(\theta)$, c'est-à-dire l'ensemble des $\theta$ tel que c'est la deuxième partie du terme de droite de l'équation~\eqref{eq:recPDPA} qui réalise le minimum.

Plus généralement, on définit
$$\mathcal{S}_{n,\nu}^k = \left\lbrace \theta\in\Theta ; \; C_{k-1,\nu}+\sum_{i=\nu+1}^n \gamma (y_i,\theta)\leq R_{k,n}(\theta) \right\rbrace$$
pour tous $1\leq k \leq \nu < n \leq N$ et $k \leq m$. C'est l'ensemble des $\theta$, paramètre du dernier segment, tel que $\nu$ est la dernière rupture optimale dans la segmentation à $k$ ruptures de $y_1,\dots ,y_n$. Cela permet de définir l'ensemble des dernières ruptures optimales pour un certain $\theta$:
$$\mathcal{\tau}_n^k = \left\lbrace \nu\in\left\lbrace k,\dots , n-1\right\rbrace ; \; \mathcal{S}_{n,\nu}^k \neq \emptyset \right\rbrace \; . $$
pour tous $1\leq k \leq \min(m,n)\leq \max (m,n) \leq N$.

Les relations suivantes permettent le calcul par récurrence de ces ensembles.

\begin{prop}\label{prop:PDPArec}
Pour tous $1\leq k \leq m$ et $k\leq n < N$,
\begin{eqnarray}
\mathcal{S}_{n+1,n}^k & = & \left\lbrace \theta \in\Theta ; \; \forall \nu\in \mathcal{\tau}_n^k, C_{k-1,n}\leq R_{k,\nu,n}(\theta) \right\rbrace \; , \label{eq:S_nnuinit} \\
\forall \nu \in\left\lbrace k,\dots , n-1\right\rbrace , \mathcal{S}_{n+1,\nu}^k & = & \mathcal{S}_{n,\nu}^k \cap \left\lbrace \theta\in\Theta ; \; R_{k,\nu,n}(\theta) \leq C_{k-1,n}\right\rbrace \; , \label{eq:S_nnurec}\\
\forall \nu \in\left\lbrace k,\dots , n-1\right\rbrace , \mathcal{S}_{n,\nu}^k = \emptyset & \Rightarrow & \forall n' \in \left\lbrace n,\dots ,N\right\rbrace , \mathcal{S}_{n',\nu}^k = \emptyset \; , \label{eq:PDPAstop}\\
\mathcal{\tau}_{n+1}^k & = & \left\lbrace \nu \in \mathcal{\tau}_n^k\cup\left\lbrace n \right\rbrace ; \; \mathcal{S}_{n+1,\nu}^k \neq \emptyset \right\rbrace \; . \label{eq:taurec}
\end{eqnarray}
\end{prop}
La proposition \ref{prop:PDPArec} permet d'écrire l'algorithme de programmation dynamique élagué pour la segmentation. La relation \eqref{eq:PDPAstop} fournit un critère d'arrêt de l'exploration de l'ensemble des segmentations.

\begin{algorithm}%[H]
\Begin{
 \For{$ k = 1, \dots , m$}{
 \begin{eqnarray*}
 \mathcal{\tau}_{k+2}^k & := & \left\lbrace k \right\rbrace \\
R_{k,k+1,k+2}(\theta) & := & C_{k-1,k+1} + \gamma(y_{k+2},\theta) 
 \end{eqnarray*}
 \For{$n=k+2,\dots ,N-1$}{
 \For{$\nu\in\mathcal{\tau}_n^k $}{
 $\mathcal{S}_{n+1,\nu}^k:=\mathcal{S}_{n,\nu}^k \cap \left\lbrace \theta\in\Theta ; \; R_{k,\nu,n}(\theta) \leq C_{k-1,n} \right\rbrace$
 }\tcp{D'après \eqref{eq:S_nnurec}}
 $\mathcal{S}_{n+1,n}^k  =  \left\lbrace \theta \in\Theta ; \; \forall \nu\in \mathcal{\tau}_n^k, C_{k-1,n}\leq R_{k,\nu,n}(\theta) \right\rbrace $
 \tcp{D'après \eqref{eq:S_nnuinit}}
 $\mathcal{\tau}_{n+1}^k  =  \left\lbrace \nu \in \mathcal{\tau}_n^k\cup\left\lbrace n \right\rbrace ; \; \mathcal{S}_{n+1,\nu}^k \neq \emptyset \right\rbrace$
 \tcp{D'après \eqref{eq:taurec}}
 \For{$\nu \in \mathcal{\tau}_{n+1}^k$}{
$ R_{k,\nu,n+1}(\theta):=R_{k,\nu,n}(\theta)+\gamma(y_{n+1},\theta)$}
 \begin{eqnarray*}
 D_{k,n+1} & := & \underset{\nu\in\mathcal{\tau}_{n+1}^k}{\min}\underset{\theta\in\Theta}{R_{k,\nu,n+1}(\theta)}\\
 I_{k,n+1} & := & \underset{\nu\in\mathcal{\tau}_{n+1}^k}{\argmin}\underset{\theta\in\Theta}{R_{k,\nu,n+1}(\theta)}
 \end{eqnarray*}
 \tcp{$ D_{k,n+1}$ coût optimal de la segmentation à $k$ ruptures de $y_1,\dots ,y_{n+1}$.}
 \tcp{$ I_{k,n+1}$ dernière rupture optimale de la segmentation à $k$ ruptures de $y_1,\dots ,y_{n+1}$.}
	}
}
}
\caption{Segmentation par programmation dynamique élaguée.} \label{alg:PDPA} 
\end{algorithm}

\subsubsection{Complexité}
\begin{prop}\label{prop:ComplexitePDPA}
Si:
\begin{enumerate}
\item $\Theta$ est un intervalle de $\mathbb{R}$,
\item pour tous $1\leq i\leq j\leq N$, $\theta\mapsto\sum_{s=i}^j \gamma(y_s,\theta)$ a un unique extremum local (qui est le minimum global),
\item $\forall k\in \left\lbrace 1,\dots ,m\right\rbrace, \forall n \in \left\lbrace k+1 , \dots ,N\right\rbrace , \forall \nu \in \left\lbrace k, \dots , n-1\right\rbrace, R_{k,\nu,n}$ est minimisé en temps borné,
\item  $\forall k\in \left\lbrace 1,\dots ,m\right\rbrace, \forall n \in \left\lbrace k+1 , \dots ,N\right\rbrace , \forall \nu \in \left\lbrace k, \dots , n-1\right\rbrace$,  les racines de $R_{k,\nu,n}(\theta)=C_{k-1,t}$ sont calculées en temps borné,
\end{enumerate}
alors l'algorithme \ref{alg:PDPA} a:
\begin{enumerate}
\item une complexité en temps $O(mN^2)$,
\item une complexité en espace $O(mN)$.
\end{enumerate}
\end{prop}

La première hypothèse de la proposition \ref{prop:ComplexitePDPA} tient de propriétés des intervalles de $\mathbb{R}$ difficilement généralisables à d'autres espaces.

La proposition~\ref{prop:ComplexitePDPA} donne une borne supérieure à la complexité en temps de l'algorithme~\ref{alg:PDPA}. Toutefois, dans bien des cas, la complexité est inférieure, grâce à l'élagage qui donne des ensembles $\mathcal{\tau}_{n}^k$ de cardinal d'ordre inférieur à $n$, idéalement d'ordre $O(1)$ (qui, dans ce cas, entraîne une complexité en temps de l'algorithme~\ref{alg:PDPA} d'ordre $O(mN)$). Les simulations réalisées par \textcite{pruned} montrent que, avec la perte quadratique $\gamma(y_i,\mu) = (y_i - \mu)^2$, à $m$ fixé, l'algorithme~\ref{alg:PDPA} est plus rapide que l'algorithme~\ref{alg:DPA}. \textcite{pruned} annonce une complexité en temps \enquote{moyenne} en $O(mN\log(N))$.

Récemment, \textcite{maidstone2014optimal} ont proposé un algorithme de programmation dynamique différemment élagué, l'algorithme SNIP. Les conditions permettant de l'utiliser sont plus faibles que \eqref{eq:conditionC1_PDPA}, cela rend donc cet algorithme particulièrement intéressant quand cette dernière condition n'est pas vérifiée. Toutefois, si  \eqref{eq:conditionC1_PDPA} est vérifiée, l'algorithme SNIP élague toujours moins que l'algorithme de \textcite{pruned}. Dans les chapitres~\ref{ch:ar1} et~\ref{ch:arp}, nous avons pu nous ramener à un cas où \eqref{eq:conditionC1_PDPA} est vérifiée. Par conséquent, nous n'avons pas utilisé l'algorithme SNIP dans notre travail.

==> chapitres/outils/inegalites.tex <==
Dans cette section, on énonce l'inégalité de Kolmogorov, sa généralisation qu'est l'inégalité de H\'ajek-Rényi, une généralisation de cette dernière, ainsi que leur utilisation en segmentation. Dans toute cette section, $\left(\eta_i\right)_{i\geq 1}$ est une suite de variables aléatoires réelles, centrées, de carré intégrable. Pour tout $n\geq 1$, on définit $S_n = \sum_{i=1}^n \eta_i$.

\subsection{Inégalité de Kolmogorov}
\input{./chapitres/outils/inegalites/kolmogorov}

\subsection{Inégalité de H\'ajek-Rényi}
\input{./chapitres/outils/inegalites/hajek}

\subsection{Généralisation de l'inégalité de H\'ajek-Rényi}
\input{./chapitres/outils/inegalites/generalisations}

\subsection{Utilisation en segmentation}
\input{./chapitres/outils/inegalites/segmentation}



==> chapitres/outils/inegalites/generalisations.tex <==
Cette inégalité de H\'ajek-Rényi a fait l'objet de nombreuses généralisations, notamment au cas où les variables aléatoires $\eta_i$ sont dépendantes. Nous n'en énoncerons qu'une.

\begin{prop}[Inégalité de H\'ajek-Rényi pour les processus linéaires]\label{prop:HRBai}
Soit $\epsilon=\left(\epsilon_i\right)_{i\in\mathbb{Z}}$ une suite de v.a.r. i.i.d. centrées de variance $\sigma^2$.

Supposons qu'il existe une suite réelle $\left(a_j\right)_{j\geq 0}$ telle que:
\begin{itemize}
\item $\forall i\geq 1, \eta_i = \sum_{j=0}^\infty a_j \epsilon_{i-j}$ presque-sûrement,
\item $\sum_{j=0}^\infty j\left|a_j\right|<+\infty$.
\end{itemize}

Alors, pour toute suite décroissante de réels positifs $\left(c_n\right)_{n\geq 1}$,
$$\forall m>n\geq 1,\forall x>0, P\left(\underset{i=n,\dots ,m}{\max}\left(c_i \left|S_i\right|\right) \geq x\right)\leq \frac{A\sigma^2}{x^2}\left(n c_n^2 + \sum_{i=n+1}^m c_i^2\right) \; ,$$
où $A$ est une constante réelle qui ne dépend que de la suite $\left(a_j\right)_{j\geq 0}$.
\end{prop}
Résultat démontré par \textcite{Bai}. De plus, \textcite{LM} démontrent un théorème qui permet notamment la généralisation de l'inégalité de H\'ajek-Rényi aux processus à longue mémoire~\parencite[voir par exemple][pour une introduction à ces processus]{beran2013long}.


%La deuxième généralisation est énoncée car le résultat est repris tel quel dans la section \ref{App:Proof}. Non pas que la généralité de l'énoncé ait été nécessaire aux démonstrations du chapitre \ref{ch:ar1}, mais par souci de concision et de cohérence avec une des références principales de ce chapitre \cite{LM}.
%
%\begin{prop}[Inégalité de H\'ajek-Rényi pour les processus à longue mémoire]\label{prop:HRLM}
%
%Alors, pour toute suite décroissante de réels positifs $\left(c_n\right)_{n\geq 1}$,
%\begin{equation}\label{eq:HRBai}
%\forall m>n\geq 1,\forall x>0, P\left(\underset{i=n,\dots ,m}{\max}\left(c_i \left|S_i\right|\right) \geq x\right)\leq \frac{A\left(\Phi\right)\sigma^2}{x^2}\left(n c_n^2 + \sum_{i=n+1}^m c_i^2\right) \; .
%\end{equation}
%où $A\left(\Phi\right)$ est une constante réelle qui ne dépend que du paramètre de longue mémoire $\Phi$.
%\end{prop}

==> chapitres/outils/inegalites/hajek.tex <==
\textcite{HR} généralisent l'inégalité de Kolmogorov:
\begin{theo}[Inégalité de H\'ajek-Rényi]\label{th:HR}
Si les variables aléatoires $\eta_i$ sont mutuellement indépendantes, alors, pour toute suite décroissante de réels positifs $\left(c_n\right)_{n\geq 1}$,
$$\forall m>n\geq 1,\forall x>0, P\left(\underset{i=n,\dots ,m}{\max}\left(c_i \left|S_i\right|\right) \geq x\right)\leq \frac{1}{x^2}\left(c_n^2 \sum_{i=1}^n \Var \eta_i + \sum_{i=n+1}^m c_i^2\Var \eta_i\right) \; .$$
\end{theo}

Le théorème \ref{th:kolmogorov} est un cas particulier du théorème \ref{th:HR}, avec $n=1$ et $\forall n\geq 1, c_n = 1$. Si $\forall n\geq 1, c_n = \frac{1}{n}$, on obtient un contrôle sur les déviations maximales des moyennes:
$$\forall m>n\geq 1,\forall x>0, P\left(\underset{i=n,\dots ,m}{\max}\left(\frac{1}{i} \left|S_i\right|\right) \geq x\right)\leq \frac{1}{x^2}\left(\frac{1}{n^2} \sum_{i=1}^n \Var \eta_i + \sum_{i=n+1}^m \frac{1}{i^2}\Var \eta_i\right) \; .$$

\begin{corollaire}\label{cor:HR}
Sous les mêmes hypothèses que le théorème \ref{th:HR},
$$\forall n\geq 1,\forall x>0, P\left(\underset{i\geq n}{\max}\left(c_i \left|S_i\right|\right) \geq x\right)\leq \frac{1}{x^2}\left(c_n^2 \sum_{i=1}^n \Var \eta_i + \sum_{i=n+1}^\infty c_i^2 \Var \eta_i\right) \; .$$
\end{corollaire}

En particulier, si $\forall n\geq 1, c_n = \frac{1}{n}$, on obtient là aussi un contrôle sur les déviations maximales des moyennes:
$$\forall n\geq 1,\forall x>0, P\left(\underset{i\geq n}{\max}\left(\frac{1}{i} \left|S_i\right|\right) \geq x\right)\leq \frac{1}{x^2}\left(\frac{1}{n^2} \sum_{i=1}^n \Var \eta_i + \sum_{i=n+1}^\infty \frac{1}{i^2}\Var \eta_i\right) \; .$$


==> chapitres/outils/inegalites/kolmogorov.tex <==
\begin{theo}[Inégalité de Kolmogorov]\label{th:kolmogorov}
Si les variables aléatoires $\eta_i$ sont mutuellement indépendantes, alors
$$ \forall n\geq 1,\forall x>0, P\left(\underset{i=1,\dots ,n}{\max}\left|S_i\right| \geq x\right)\leq \frac{1}{x^2}\sum_{i=1}^n \Var \eta_i \; .$$
\end{theo}

La démonstration de cette inégalité figure dans bien des ouvrages de probabilités. L'article original \citep{kolmogoroff1928summen} étant en allemand, les non-germanophones peuvent consulter par exemple \textcite[Theorème 2.5.2.]{durrett2010probability}. L'inégalité de Bienaymé-Tchebychev nous aurait seulement assuré $P\left(\left|S_n\right| \geq x\right)\leq \frac{1}{x^2}\sum_{i=1}^n \Var \eta_i$. L'inégalité maximale du théorème~\ref{th:kolmogorov} est un résultat bien plus puissant. L'inégalité de Kolmogorov est un ingrédient essentiel de la démonstration de la loi forte des grands nombres.

==> chapitres/outils/inegalites/segmentation.tex <==
L'inégalité de Kolmogorov, et surtout les inégalités de H\'ajek-Rényi, interviennent régulièrement en segmentation; qu'il s'agisse d'une rupture simple \citep{Bai} ou de ruptures multiples~\parencites{lavielle1999}{LM}, de détection \emph{on-line}~\citep{BKmonitoring} ou \emph{off-line}~\citep{Bai}.

Ici, $y_1, \dots , y_n$ sont des observations telles que $y_i = \mu(i) + \eta_i$ pour tout $1\leq i\leq n$ où $\mu:\left\lbrace 1,\dots ,n\right\rbrace \rightarrow \mathbb{R}$ a une ou des ruptures $\lfloor n\tau \rfloor$, et $\eta$ est une suite de v.a.r. centrées (avec éventuellement des hypothèses supplémentaires).

Dans ce contexte, l'inégalité sert principalement à démontrer le taux de convergence de l'estimateur des moindres carrés $\widehat{\tau}_n$ de la rupture $\tau\in (0,1)$, à savoir $\widehat{\tau}_n - \tau = O_P(n^{-1})$ sous certaines conditions sur $\eta$. Cette démarche peut se généraliser à d'autres estimateurs \citep{lavielle1999}.

Dans les chapitres~\ref{ch:ar1} et~\ref{ch:arp}, l'utilisation d'une inégalité de H\'ajek-Rényi généralisée est cachée derrière les références aux résultats de \textcite{LM}. Il est fait référence à ce résultat en particulier pour ne pas multiplier les références dans l'article. Toutefois, l'aspect longue-mémoire n'est pas utilisé et on aurait pu se contenter de faire référence à un résultat plus faible. L'inégalité de Kolmogorov est, elle, utilisée dans la preuve de la proposition~\ref{ar1:Prop:SelBeta}, qui concerne la sélection du nombre de ruptures par critère pénalisé.
%
%Nous allons reprendre la démonstration de \cite{Bai} pour illustrer l'utilisation d'une inégalité de H\'ajek-Rényi dans ce contexte.
%
%Plus précisément, supposons que $\eta$ vérifie les hypothèses de la proposition \ref{prop:HRBai}. Soient $\tau^*\in\left(0,1\right)$ et $t^* = \lfloor n\tau^*\rfloor$. Supposons qu'il existe $\mu_1^*, \mu_2^*\in\mathbb{R}$ tels que:
%\begin{eqnarray*}
%\forall i\in  1,\dots ,t^*, \mu(i) & = & \mu_1^* \; ,\\
%\forall i\in  t^*+1,\dots ,n, \mu(i) & = & \mu_2^* \; .
%\end{eqnarray*}
%
%On définit:
%\begin{eqnarray*}
%\widehat{t}_n & = & \underset{t=1,\dots ,n-1}{\argmin} \sum_{i=1}^t \left(Y_i - \overline{Y}_{1:t}\right)^2 + \sum_{i=t+1}^n \left(Y_i - \overline{Y}_{(t+1):n}\right)^2 \; , \\
%\widehat{\tau}_n & = & \frac{\widehat{t}_n}{n} \; .
%\end{eqnarray*}
%
%où $Y_{i:j} = \frac{1}{j-i+1}\sum_{k=i}^j Y_k$. Il s'agit de montrer que:
%
%\begin{equation}\label{eq:tauxBai}
%\widehat{\tau}_n - \tau^* = \mathcal{O}_P \left(n^{-1}\right) \; .
%\end{equation}



==> chapitres/outils/processus_delta.tex <==
On introduit ici des notions et énonce des résultats utilisés par la suite dans les preuves \ref{ar1:proof:corr_tcl} et \ref{arp:proof:corr_tcl} de la normalité asymptotique d'estimateurs. 
\subsection{Processus empirique}\label{subs:processus_empirique}
\input{./chapitres/outils/processus_delta/processus}
\subsection{Delta-méthode fonctionnelle}
\input{./chapitres/outils/processus_delta/delta}
\subsection{Fonctions d'un processus gaussien}
\input{./chapitres/outils/processus_delta/fonctions}


==> chapitres/outils/processus_delta/delta.tex <==
L'idée est de généraliser la Delta-méthode à des espaces de dimension infinie. La référence de cette section est \textcite[chapitres 3, 20, 21]{van}.

\subsubsection{Delta-méthode en dimension finie}
\begin{theo}\label{th:DeltaMethode}
Soit $\Theta\subset\mathbb{R}^k$, $\theta\in\Theta$ et une application $\phi:\Theta\rightarrow \mathbb{R}^m$ différentiable en $\theta$. Soit $T$ v.a. sur $\mathbb{R}^k$, $\left(T_n\right)$ une suite de v.a. sur $\Theta$ et $\left(r_n\right)$ une suite réelle de limite $+\infty$. Supposons que
$$ r_n\left(T_n - \theta\right) \underset{n\rightarrow\infty}{\overset{d}{\longrightarrow}} T \; .$$
Alors
$$ r_n\left(\phi(T_n)-\phi(\theta)\right)\underset{n\rightarrow\infty}{\overset{d}{\longrightarrow}} \phi'_\theta (T) \; , $$
où $\phi'_\theta$ est la différentielle de $\phi$ en $\theta$. De plus,
$$ r_n\left(\phi(T_n)-\phi(\theta)\right) = \phi'_\theta\left(r_n\left(T_n - \theta\right)\right) + o_P(1) \; . $$
\end{theo}

\subsubsection{Différentiabilité au sens de Hadamard}
La généralisation du théorème \ref{th:DeltaMethode} à des espaces de dimension infinie nécessite de se pencher plus avant sur la notion de différentiabilité et de différentielle dans un espace de dimension infinie. Il existe différentes notions de différentiabilité, qui sont équivalentes en dimension finie mais pas en dimension infinie. La notion dont nous avons besoin ici est la différentiabilité au sens de Hadamard.
\begin{definition}
Soit deux espaces vectoriels normés $(E,\Vert\cdot\Vert_E)$ et $(F,\Vert\cdot\Vert_F)$. Soit $\theta\in\Theta\subset E$ et $E_0$ un sous-espace vectoriel de $E$. Soit $\phi:E\rightarrow F$. $\phi$ est dit \emph{différentiable au sens de Hadamard} en $\theta$ \emph{tangentiellement} à $E_0$ s'il existe $\phi'_\theta:E_0\rightarrow F$ linéaire et continue telle que pour tout $h\in E_0$, pour tout $\varepsilon>0$, pour toute application $g:(0,\varepsilon)\rightarrow E_0$ de limite $h$ en $0$ et telle que $\forall t\in (0,\varepsilon), \theta + tg(t)\in \Theta$,
$$ \underset{t\rightarrow 0}{\lim}\left\Vert \frac{\phi(\theta+tg(t))-\phi(\theta)}{t} - \phi'_\theta (h) \right\Vert_E =0 \; . $$
$\phi'_\theta$ est appelée \emph{différentielle} de $\phi$ en $\theta$ tangentiellement à $E_0$.
\end{definition}
\subsubsection{Delta-méthode fonctionnelle}
\begin{theo}\label{th:delta_methode_fonctionnelle}
Soit deux espaces vectoriels normés $(E,\Vert\cdot\Vert_E)$ et $(F,\Vert\cdot\Vert_F)$. Soit $\theta\in\Theta\subset E$ et $E_0$ un sous-espace vectoriel de $E$. Soit $\phi:E\rightarrow F$ différentiable au sens de Hadamard en $\theta$ tangentiellement à $E_0$. Soient $T$ v.a. sur $E_0$, $\left(T_n\right)$ une suite de v.a. sur $\Theta$ et $\left(r_n\right)$ une suite réelle de limite $+\infty$. Supposons que
$$ r_n\left(T_n - \theta\right) \underset{n\rightarrow\infty}{\overset{d}{\longrightarrow}} T \; .$$
Alors
$$ r_n\left(\phi(T_n)-\phi(\theta)\right)\underset{n\rightarrow\infty}{\overset{d}{\longrightarrow}} \phi'_\theta (T) \; , $$
où $\phi'_\theta$ est la différentielle de $\phi$ en $\theta$. De plus, si $E=E_0$, alors
$$ r_n\left(\phi(T_n)-\phi(\theta)\right) = \phi'_\theta\left(r_n\left(T_n - \theta\right)\right) + o_P(1) \; . $$
\end{theo}

Typiquement, $E$ peut être l'espace $D\left[-\infty,+\infty\right]$~(cf. définition~\ref{def:Skorohod}) et $r_n\left(T_n - \theta\right)$ le processus empirique~(cf. définition~\ref{def:ecdf_ep}). D'un résultat de convergence du processus empirique~(comme les théorèmes~\ref{th:Donsker} et~\ref{th:CM}), on peut déduire la normalité asymptotique d'un estimateur \emph{plug-in}~($\phi(F_n)$ est l'estimateur de $\phi(F)$).
C'est notamment grâce à ce résultat qu'on obtient, sous certaines conditions, la normalité asymptotique des quantiles empiriques comme estimateurs des quantiles de la loi.

==> chapitres/outils/processus_delta/fonctions.tex <==
Le résultat suivant \parencite[théorème 4]{arcones1994limit} est utilisé en association avec les théorèmes~\ref{th:CM} et~\ref{th:delta_methode_fonctionnelle} pour démontrer la normalité asymptotique d'estimateurs.

\begin{definition}\label{def:rang_hermite}
Soit $f:\mathbb{R}^d\rightarrow \mathbb{R}$, de carré intégrable par rapport à une mesure gaussienne, et $X=\left(X^{(p)}\right)_{1\leq p \leq d}$ vecteur gaussien sur $\mathbb{R}^d$. Le \emph{rang d'Hermite} de $f$ par rapport à $X$ est
$$ \inf \left\lbrace m\geq 1 ; \exists Q \textit{ polynôme à } d \textit{ variables, de degré } m \textit{ tel que } \mathbb{E}\left[\left(f\left(X\right)-\mathbb{E}\left[X\right]\right) Q\left(X\right)\right]\neq 0 \right\rbrace \; . $$
\end{definition}

\begin{theo}\label{th:arcones}
Soit $\left(X_i\right)_{i\in\mathbb{Z}}=\left(\left(X_i^{(p)}\right)_{1\leq p \leq d}\right)_{i\in\mathbb{N}^\star}$ un processus gaussien centré stationnaire $d$-varié. Soit $f:\mathbb{R}^d\rightarrow \mathbb{R}$ de carré intégrable par rapport à une mesure gaussienne et de rang d'Hermite $m$ par rapport à $X_0$. Supposons que
$$ \forall (p,q)\in\left\lbrace 1,\dots ,d\right\rbrace^2, \sum_{k\in\mathbb{Z}} \left|\mathrm{Cov}\left(X_0^{(p)}, X_k^{(q)}\right)\right|^m < \infty \; . $$ 
Alors
$$ \frac{1}{\sqrt{n}}\sum_{i=1}^n \left(f\left(X_i\right) - \mathbb{E}\left[f\left(X_i\right)\right]\right) \overset{d}{\underset{n\rightarrow\infty}{\longrightarrow}} \mathcal{N}\left(0, \widetilde{\sigma}^2\right) \; , $$
où
$$ \widetilde{\sigma}^2 = \mathrm{Var}\left(f\left(X_0\right)\right) + 2\sum_{i=1}^{\infty} \mathrm{Cov}\left(f\left(X_0\right), f\left(X_i\right)\right) \; . $$
\end{theo}

==> chapitres/outils/processus_delta/processus.tex <==
La référence de cette section est en premier lieu \textcite[chapitre 19]{van}.

\begin{definition}\label{def:ecdf_ep}
Soient $X_1,\dots ,X_n$ des v.a.r. La \emph{fonction de répartition empirique} est la fonction aléatoire $F_n:\mathbb{R}\rightarrow \left[0,1\right]$ définie par
$$\forall t\in\mathbb{R}, F_n(t) = \frac{1}{n}\sum_{i=1}^n \mathbf{1}_{X_i\leq t} \; .$$
Si les $X_i$ ont la même loi, de fonction de répartition $F$, le \emph{processus empirique} est la fonction réelle aléatoire $\sqrt{n}\left(F_n - F\right)$.
\end{definition}

D'après le théorème de Glivenko-Cantelli, si $\left(X_n\right)_{n\geq 1}$ est une suite de v.a.r. i.i.d. de même loi de fonction de répartition $F$, la fonction de répartition empirique converge presque-sûrement vers $F$ pour la norme uniforme. C'est l'équivalent de la loi forte des grands nombres pour la fonction de répartition empirique. De même, le théorème \ref{th:Donsker} ci-dessous fournit un équivalent du théorème central-limite.

\begin{definition}\label{def:Skorohod}
On note $D\left[-\infty,+\infty\right]$ l'espace vectoriel des fonctions bornées de $\left[-\infty,+\infty\right]$ dans $\mathbb{R}$ et càdlàg (continues à droite et ayant une limite à gauche en tout point, ayant une limite en $-\infty$ et en $+\infty$), muni de la norme uniforme.
\end{definition}
En particulier, les fonctions de répartition sur $\mathbb{R}$ sont des éléments de $D\left[-\infty,+\infty\right]$.
\begin{definition}
Soit $F$ une fonction de répartition sur $\mathbb{R}$. Un $F$-\emph{pont brownien} est une variable aléatoire $G_F$ sur $D\left[-\infty,+\infty\right]$ telle que:
\begin{itemize}
\item $\forall k\geq 1, \forall \left(t_1,\dots ,t_k\right)\in\mathbb{R}^k, \left(G_F (t_1),\dots ,G_F(t_k)\right)$ est un vecteur gaussien centré,
\item $\forall (s,t)\in\mathbb{R}^2, s\leq t \Rightarrow Cov\left(G_F(s),G_F(t)\right) = F(s)(1-F(t))$.
\end{itemize}
\end{definition}
\begin{theo}[Donsker]\label{th:Donsker}
Soit $\left(X_n\right)_{n\geq 1}$ une suite de v.a.r. i.i.d. de fonction de répartition $F$. Alors $\left(\sqrt{n}\left(F_n - F\right)\right)$ converge en loi dans $D\left[-\infty,+\infty\right]$ vers un $F$-pont brownien.
\end{theo}

Toutefois, ce résultat est insuffisant dans le cas d'une suite de variables aléatoires dépendantes. Pour traiter ce cas, nous avons utilisé le théorème suivant prouvé par \textcite{CM}.
\begin{definition}\label{def:Hermite}
Pour un entier naturel $k$, le $k^e$ \emph{polynôme de Hermite} est défini par
$$ H_k (x) = (-1)^k e^{x^2/2} \frac{d^k}{dx^k}e^{-x^2/2} \; .  $$
\end{definition}
\begin{theo}\label{th:CM}
Soit $\left(Z_n\right)_{n\in \mathbb{Z}}$ une suite stationnaire de v.a.r. normales centrées réduites. Soit $G$ une fonction borélienne et $\left(X_n\right)_{n\geq 1} = \left(G\left(Z_n\right)\right)_{n\geq 1}$. Soit $F$ la fonction de répartition de $X_1$. Pour $x$ réel et $k$ entier naturel, on note $J_k (x) = \mathbb{E}\left(H_k (Z_1)\left(\mathbf{1}_{X_1 \leq x} - F(Z_1)\right)\right)$. On définit
\begin{eqnarray*}
\forall x\in\mathbb{R}, \; m_x & = & \min\left\lbrace k ; \; J_k (x) \neq 0\right\rbrace \; , \\
m & = & \min\left\lbrace m_x ; \; x\in\mathbb{R}, 0<F(x)<1\right\rbrace \; .
\end{eqnarray*}
Supposons que $F$ est continue et que
$$ \sum_{h=1}^\infty \left|\gamma_Z (h)\right|^m < +\infty \; . $$
Soit $W$ une v.a. sur $D\left[-\infty,+\infty\right]$, un processus gaussien centré --- c'est-à-dire tel que pour tout $k\geq 1, \forall \left(t_l\right)_{1\leq l\leq k}\in\mathbb{R}^k, \left(W (t_l)\right)_{1\leq l\leq k}$ est un vecteur gaussien centré --- de fonction d'autocovariance:
$$ (x,y)\mapsto \mathrm{Cov}(W(x),W(y)) = \sum_{q=m}^\infty \frac{J_q (x)J_q (y)}{q!}\left\lbrace 1 + 2\sum_{h=1}^\infty \gamma_Z (h)^q \right\rbrace \; . $$
Alors $\left(\sqrt{n}\left(F_n - F\right)\right)$ converge en loi dans $D\left[-\infty,+\infty\right]$ vers $W$.
\end{theo}

==> chapitres/outils/robuste.tex <==
Un estimateur robuste est un estimateur dont les propriétés ne sont pas altérées par la présence de valeurs aberrantes dans les observations (c'est-à-dire de loi différente de celle des autres observations) ou par une relaxation des hypothèses du modèle.

Les \emph{M-estimateurs} d'un paramètre $\theta$ du modèle, définis par
$$ \widehat{\theta} = \underset{\theta\in\Theta}{\argmin} \sum_{i=1}^n \rho (X_i , \theta) \; , $$
si $X_1,\dots ,X_n$ sont les observations et $\rho$ une certaine fonction, jouent un rôle important dans l'estimation robuste. Les différentes propriétés de robustesse de l'estimateur peuvent être obtenues par un choix adéquat de la fonction $\rho$. Par exemple, si $\Theta=\mathbb{R}$, $X_1,\dots ,X_n\in\mathbb{R}$ et $\rho \left(X_i,\theta\right) = \left|X_i - \theta\right|$, alors $\widehat{\theta}=\underset{i=1,\dots ,n}{\med} X_i$. La médiane est un exemple simple d'estimateur robuste. Cela étant dit, il ne sera pas détaillé ici l'étude générale des M-estimateurs qui ne nous est pas utile en tant que telle, même si ce n'est pas sans raison que les estimateurs que nous considérons utilisent les quantiles (dont la médiane).

\subsection{Point d'effondrement}
\input{./chapitres/outils/robuste/effondrement}
\subsection{Estimation robuste d'un paramètre d'échelle}\label{subs:CR}
\input{./chapitres/outils/robuste/echelle}
\subsection{Estimation robuste des fonctions d'autocovariance et d'autocorrélation d'un processus stationnaire du second ordre}\label{subs:REstScaleAutoco}
\input{./chapitres/outils/robuste/autocovariance}

==> chapitres/outils/robuste/autocovariance.tex <==
Dans cette section sont présentés les estimateurs de \textcite[un pour la fonction d'autocovariance, un pour la fonction d'autocorrélation]{MG}. On se donne $\boldsymbol{X}=\left(X_i\right)_{i\in\mathbb{Z}}$, un processus stationnaire du second ordre (non-nécessairement centré), et on cherche à estimer $\gamma_X (h)$ et $\rho_X (h)$ à partir de $n$ observations successives de $\boldsymbol{X}$.

\subsubsection{Estimation robuste de la fonction d'autocovariance}

Cet estimateur de la fonction d'autocovariance utilise l'identité suivante, valable pour deux v.a.r. de carré intégrable $A$ et $B$:
$$ \PCov (A,B) = \frac{1}{4}\left\lbrace\PVar(A+B)-\PVar(A-B)\right\rbrace \; .$$
Cette égalité est notamment vraie pour $A=X_i$ et $B=X_{i+h}$. Ainsi, pour tout $i\in\mathbb{Z}$,
$$ \gamma_X (h) = \frac{1}{4} \left\lbrace\PVar(X_i+X_{i+h})-\PVar(X_i-X_{i+h})\right\rbrace \; . $$

Cela conduit à estimer préalablement les variances $\PVar(X_i+X_{i+h})$ et $\PVar(X_i-X_{i+h})$. L'estimateur $Q_n$ (cf. équation \eqref{eq:CRQ}) permet de faire cela de façon robuste.

On se donne $\boldsymbol{u}^h=\left(X_1,\dots ,X_{n-h}\right)$ et $\boldsymbol{v}^h=\left(X_{h+1},\dots ,X_{n}\right)$. L'estimation robuste de $\PVar(X_i+X_{i+h})$ et de $\PVar(X_i-X_{i+h})$ se fait respectivement par $Q_{n-h}^2 (\boldsymbol{u}^h+\boldsymbol{v}^h)$ et $Q_{n-h}^2 (\boldsymbol{u}^h-\boldsymbol{v}^h)$. \textcite{MG} proposent donc comme estimateur robuste de $\gamma_X (h)$:
\begin{equation}\label{eq:MGcov}
\widehat{\gamma}_n (h,\boldsymbol{X}) = \frac{1}{4}\left\lbrace Q_{n-h}^2 (\boldsymbol{u}^h+\boldsymbol{v}^h) - Q_{n-h}^2 (\boldsymbol{u}^h-\boldsymbol{v}^h) \right\rbrace \; .
\end{equation}
\textcite{MG} annoncent un point d'effondrement de $1/4$ quand $\boldsymbol{X}$ est un processus ARMA, mais dans un sens différent que celui de la définition \ref{def:BP}. En effet, ils considèrent que les perturbations affectent le processus d'innovation intervenant dans l'équation ARMA vérifiée par $\boldsymbol{X}$ et non les observations de $\boldsymbol{X}$ directement.

\subsubsection{Estimation robuste de la fonction d'autocorrélation}
 Pour estimer $\rho_X(h)$, on pourrait utiliser
 $$ \frac{\widehat{\gamma}_n (h,\boldsymbol{X})}{Q_n (\boldsymbol{X})} \; . $$
 Toutefois, l'identité suivante est valable pour deux v.a.r. de carré intégrable $A$ et $B$:
$$ \frac{1}{2}\left\lbrace\PVar(A)+\PVar(B)\right\rbrace = \frac{1}{4}\left\lbrace\PVar(A+B)+\PVar(A-B)\right\rbrace \; ,$$
et donc 
$$ \PVar(A) = \frac{1}{4}\left\lbrace\PVar(A+B)+\PVar(A-B)\right\rbrace $$
si $A$ et $B$ ont la même variance. On peut donc utiliser
$$\frac{1}{4}\left\lbrace Q_{n-h}^2 (\boldsymbol{u}^h+\boldsymbol{v}^h) + Q_{n-h}^2 (\boldsymbol{u}^h-\boldsymbol{v}^h)\right\rbrace $$
pour estimer de façon robuste $\gamma_X(0)$. Ainsi,
\begin{equation}\label{eq:MGcorr}
\widehat{\rho}_n (h,\boldsymbol{X}) = \frac{Q_{n-h}^2 (\boldsymbol{u}^h+\boldsymbol{v}^h) - Q_{n-h}^2 (\boldsymbol{u}^h-\boldsymbol{v}^h)}{Q_{n-h}^2 (\boldsymbol{u}^h+\boldsymbol{v}^h) + Q_{n-h}^2 (\boldsymbol{u}^h-\boldsymbol{v}^h)}
\end{equation}
est un estimateur robuste de $\rho_X(h)$. Il a le même point d'effondrement que $\widehat{\gamma}_n (h)$ et présente l'avantage d'être compris entre $-1$ et $1$, tout comme $\rho_X(h)$. Notons aussi que, dans le cas gaussien, $\widehat{\rho}_n (h,\boldsymbol{X})$ ne dépend pas de la constante $c_{Q,\Phi}$.

\subsubsection{Propriétés asymptotiques}
\textcite{levy2011robust} établissent le résultat suivant.

\begin{theo}\label{ch:outils:sec:robuste:prop:asymptotiqueCLL}
Soit $\boldsymbol{X}=\left(X_i\right)_{i\in\mathbb{Z}}$ un processus gaussien univarié centré stationnaire. Soit $h\in\mathbb{N}$. Soient $Q_n(\boldsymbol{X})$ et $\widehat{\gamma}_n (h,\boldsymbol{X})$ définis resp. en \eqref{eq:CRQ} et \eqref{eq:MGcov}. Soit
\begin{equation*}%\label{IF:Q}
\IF(x,Q,\Phi)
=c_{Q,\Phi}\left(\frac{1/4-\Phi(x+1/c_{Q,\Phi})
+\Phi(x-1/c_{Q,\Phi})}{\int_{\rset} \phi(y)\phi(y+1/c_{Q,\Phi})\rmd y}\right)\;,
\end{equation*}
où $\Phi$ est la fonction de répartition de la loi normale centrée réduite, $\phi=\Phi^\prime$ et $c_{Q,\Phi}$ est définie en \eqref{eq:constante_cQPhi}. Soit
\begin{multline*}%\label{ch:outils:sec:robuste:def:psi}
\psi : (x,y)\mapsto \left\{(\gamma_X (0)+\gamma_X (h)) \; \IF\left(\frac{x+y}{\sqrt{2(\gamma_X (0)+\gamma_X (h))}},Q,\Phi\right) \right. \\
\left. - (\gamma_X (0)-\gamma_X (h)) \; \IF\left(\frac{x-y}{\sqrt{2(\gamma_X (0)-\gamma_X (h))}},Q,\Phi\right)\right\}\; .
\end{multline*}
Supposons que la fonction d'autocovariance de $\boldsymbol{X}$ vérifie
$$ \sum_{h=1}^\infty \left| \gamma_X (h) \right| < \infty \; . $$
Alors
\begin{eqnarray}
\sqrt{n}\left(Q_n(\boldsymbol{X})-\sqrt{\gamma_X (0)}\right) & \underset{n\rightarrow\infty}{\overset{d}{\longrightarrow}} & \mathcal{N}\left(0, \tilde{\sigma}_Q^2\right) \; , \label{ch:outils:sec:robuste:convergenceQn} \\
\sqrt{n}\left(\widehat{\gamma}_n(h,\boldsymbol{X})-\gamma (h)\right) & \underset{n\rightarrow\infty}{\overset{d}{\longrightarrow}} & \mathcal{N}\left(0, \tilde{\sigma}_{\widehat{\gamma}}^2 (h) \right) \; , \label{ch:outils:sec:robuste:convergenceGamma} 
\end{eqnarray}
où
\begin{multline}\label{ch:outils:sec:robuste:defSigmaQ} 
\tilde{\sigma}_Q^2 = \\ \gamma_X(0) \mathbb{E}\left[\IF^2\left(\frac{X_1}{\sqrt{\gamma_X (0)}},Q,\Phi\right)\right] + 2\gamma_X (0) \sum_{k=1}^\infty \mathbb{E}\left[\IF\left(\frac{X_1}{\sqrt{\gamma_X (0)}},Q,\Phi\right)\IF\left(\frac{X_{k+1}}{\sqrt{\gamma_X (0)}},Q,\Phi\right)\right] \; ,
\end{multline}
\begin{equation}\label{ch:outils:sec:robuste:defSigmaGamma} 
\tilde{\sigma}_{\widehat{\gamma}}^2 (h) = \mathbb{E}\left[\psi^2\left(X_1,X_{1+h}\right)\right] + 2 \sum_{k=1}^\infty \mathbb{E}\left[ \psi\left(X_1,X_{1+h}\right) \psi\left(X_{k+1},X_{k+1+h}\right) \right] \; .
\end{equation}

De plus,
\begin{eqnarray*}
\sqrt{n-h}\left(\widehat{\gamma}_n(h,\boldsymbol{X})-\gamma (h)\right) = \frac{1}{\sqrt{n-h}}\sum_{i=1}^{n-h} \psi\left(X_i,X_{i+h}\right) + o_P(1) \; .
\end{eqnarray*}
\end{theo}
On en déduit le corollaire suivant par le lemme de Slutsky:
\begin{corollaire}\label{ch:outils:sec:robuste:cor:asymptotiqueCLL}
Sous les mêmes hypothèses que le théorème~\ref{ch:outils:sec:robuste:prop:asymptotiqueCLL} et si $\widehat{\rho}_n (h,\boldsymbol{X})$ est l'estimateur défini en \eqref{eq:MGcorr}, alors
\begin{eqnarray}\label{ch:outils:sec:robuste:convergenceRho} 
\sqrt{n}\left(\widehat{\rho}_n(h,\boldsymbol{X})-\rho_X (h)\right) & \underset{n\rightarrow\infty}{\overset{d}{\longrightarrow}} & \mathcal{N}\left(0, \frac{\tilde{\sigma}_{\widehat{\gamma}}^2 (h)}{\gamma_X^2(0)} \right) \; ,
\end{eqnarray}
où $\tilde{\sigma}_{\widehat{\gamma}}^2 (h)$ est défini en \eqref{ch:outils:sec:robuste:defSigmaGamma}.
\end{corollaire}


==> chapitres/outils/robuste/echelle.tex <==
Soit $\boldsymbol{X}=\left(X_i\right)_{i\in\mathbb{N}}$ où les $X_i$ sont des v.a.r. i.i.d. telles que
$$ \forall i \geq 1, X_i = \mu + \sigma u_i \; ,$$
où $\mu\in\mathbb{R}$ et $\sigma>0$ sont inconnus et les v.a.r. $u_i$ sont i.i.d. de loi connue de fonction de répartition $F$. On appelle ce modèle le modèle de \emph{localisation-dispersion} \parencite[équation~(2.66)]{maronna}. Le but est d'estimer $\sigma$.

Plusieurs estimateurs de ce type ont été proposés:
\begin{itemize}
\item La \emph{distance interquartile} $IQR_n(\boldsymbol{X}) = c_{IQR, F} \left(X_{\left(\left\lceil \frac{3}{4}n\right\rceil\right)} - X_{\left(\left\lceil \frac{1}{4}n\right\rceil\right)}\right)$. La constante positive $c_{IQR, F}$ est choisie en fonction de $F$ pour obtenir la consistance de l'estimateur. Le point d'effondrement de l'estimateur $IQR$ est $1/4$.
\item La \emph{déviation absolue médiane à la médiane} $MAD_n (\boldsymbol{X}) = c_{MAD, F} \underset{i=1,\dots ,n}{\med}\left| X_i - \underset{j=1,\dots ,n}{\med} X_j \right|$. La constante $c_{MAD, F}>0$ est choisie en fonction de $F$ pour obtenir la consistance de l'estimateur. Le point d'effondrement de l'estimateur $MAD$ est $1/2$.
\end{itemize}

\textcite{CR} introduisent deux nouveaux estimateurs, 
\begin{eqnarray}
S_n (\boldsymbol{X}) & = & c_{S,F} \underset{i=1,\dots ,n}{\med} \; \underset{j=1,\dots ,n}{\med} \left| X_i - X_j \right| \; , \label{eq:CRS}\\
Q_n (\boldsymbol{y}) & = & c_{Q,F} \left\lbrace \left| X_i - X_j\right| ; \; 1\leq i < j\leq n \right\rbrace_{\left(\frac{1}{2}\left\lfloor\frac{n}{2}\right\rfloor\left(\left\lfloor\frac{n}{2}\right\rfloor+1\right)\right)} \; , \label{eq:CRQ2}
\end{eqnarray}
où $E_{(k)}$ est la $k^e$ statistique d'ordre de $x_1,\dots ,x_r$ et $E=\left\lbrace x_1,\dots ,x_r\right\rbrace$. Les constantes strictement positives $c_{S,F}$ et $c_{Q,F}$ sont choisies en fonction de $F$ pour obtenir la consistance de l'estimateur. À titre d'exemple, si $F=\Phi$ est la fonction de répartition de la loi normale centrée réduite,
\begin{eqnarray}
c_{S,\Phi} & = & \med \left| \sqrt{\Phi^{-1}\left(\frac{3}{4}\right)} + u_1\right|^{-1} \approx 1.1926 \; , \label{eq:constante_cSPhi}\\
c_{Q,\Phi} & = & \frac{1}{\sqrt{2}\Phi^{-1}\left(\frac{5}{8}\right)} \approx 2.2191 \; . \label{eq:constante_cQPhi}
\end{eqnarray}
$S_n$ et $Q_n$ ont le même point d'effondrement $\frac{1}{n}\left\lfloor \frac{n}{2}\right\rfloor$, soit asymptotiquement $1/2$. La complexité en temps du calcul de ces deux estimateurs est $O\left(n\log n\right)$ \citep{CRalgo}. Dans la section \ref{subs:REstScaleAutoco}, ces estimateurs servent de base pour construire des estimateurs des fonctions d'autocovariance et d'autocorrélation d'un processus stationnaire du second ordre. \textcite{CR} font remarquer que $\frac{1}{2}\left\lfloor\frac{n}{2}\right\rfloor\left(\left\lfloor\frac{n}{2}\right\rfloor+1\right)\approx \left\lceil \frac{1}{4} C_n^2 \right\rceil$. \mbox{\textcite{levy2011robust}} utilisent alors cette approximation pour définir $Q_n$:
\begin{equation}
Q_n (\boldsymbol{y})= c_{Q,F} \left\lbrace \left| X_i - X_j\right| ; \; 1\leq i < j\leq n \right\rbrace_{\left(\left\lceil \frac{1}{4} C_n^2 \right\rceil\right)} \; .\label{eq:CRQ}
\end{equation}
Nous reprenons cette définition.

==> chapitres/outils/robuste/effondrement.tex <==
La référence de cette partie est \textcite[paragraphe 3.2.5.]{maronna}.

%\subsubsection{Point d'effondrement}
On observe $\boldsymbol{v}=\left(v_1,\dots ,v_n\right)\in\mathbb{R}^n$, réalisation d'une variable aléatoire dont la loi dépend d'un paramètre $\theta\in\Theta$. On suppose que $\Theta\subset\mathbb{R^d}$. Soit $\widehat{\theta}_n $ un estimateur de $\theta$.
On souhaite mesurer la proportion d'observations $X_i$ que l'on peut modifier arbitrairement tout en conservant une borne sur les déviations induites sur l'estimation. La proportion maximale d'observations que l'on peut ainsi modifier est le \emph{point d'effondrement} (\emph{breakdown point} en anglais) de $\widehat{\theta}_n $.
Pour $\boldsymbol{v}=\left(v_1,\dots ,v_n\right), \boldsymbol{u}=\left(u_1,\dots ,u_n\right)\in\mathbb{R}^n$ et $I\subset \left\lbrace 1,\dots ,n\right\rbrace$, on notera 
\begin{equation}\label{eq:remplacement}
\boldsymbol{v}\setminus_I \boldsymbol{u} =\left(u_i \mathbf{1}_{i\in I} + v_i\mathbf{1}_{i\not\in I}\right)_{1\leq i\leq n}\; .
\end{equation}
\begin{definition}[Point d'effondrement]\label{def:BP}
Soient $\widehat{\theta}_n:\mathbb{R}^n\rightarrow\Theta$ et $\boldsymbol{v}\in\mathbb{R}^n$. Le \emph{point d'effondrement} de $\widehat{\theta}_n$ en $\boldsymbol{v}$ est
\begin{multline*}
\varepsilon_n^* \left(\widehat{\theta}_n,\boldsymbol{v}\right) = \\
\frac{1}{n}\max\left\lbrace m\geq 0 ; \; \exists K\subset \mathring{\Theta}, K \textit{ compact}, \forall \boldsymbol{u}\in\mathbb{R}^n, \forall I\subset\left\lbrace 1,\dots ,n\right\rbrace, |I|=m\Rightarrow \widehat{\theta}_n\left(\boldsymbol{v}\setminus_I \boldsymbol{u}\right)\in K\right\rbrace \; ,
\end{multline*}
où $\boldsymbol{v}\setminus_I \boldsymbol{u}$ est défini en \eqref{eq:remplacement} et $\mathring{\Theta}$ est l'intérieur de $\Theta$. Si $\varepsilon_n^* \left(\widehat{\theta}_n,\cdot \right)$ est constante sur $\mathbb{R}^n$, l'unique valeur prise par cette fonction est appelée \emph{point d'effondrement} de $\widehat{\theta}_n$ et est notée $\varepsilon_n^* \left(\widehat{\theta}_n\right)$. Dans ce cas, si la suite $\left(\varepsilon_n^* \left(\widehat{\theta}_n\right)\right)_n$ a une limite, la limite est appelée \emph{point d'effondrement} de $\widehat{\theta}$ et est notée  $\varepsilon^* \left(\widehat{\theta}\right)$.
\end{definition}
Le point d'effondrement d'un estimateur consistant est inférieur ou égal à $1/2$.
%\subsubsection{Fonction d'influence}

==> chapitres/outils/selection.tex <==
Un catalogue non-exhaustif de principes de sélection de modèle est établi dans les sections~\ref{ch:outils:sec:selection:subs:frequentiste} et~\ref{ch:outils:sec:selection:subs:bayesien}. Leur application à la segmentation est discutée dans la section~\ref{ch:outils:sec:selection:subs:segmentation}.

\subsection{Introduction}\label{ch:outils:sec:selection:subs:introduction}
\input{./chapitres/outils/selection/introduction}

\subsection{Sélection de modèle par critère pénalisé, cadre fréquentiste}\label{ch:outils:sec:selection:subs:frequentiste}
\input{./chapitres/outils/selection/frequentiste}


\subsection{Sélection de modèle bayésienne}\label{ch:outils:sec:selection:subs:bayesien}
\input{./chapitres/outils/selection/bayesien}


\subsection{Sélection du nombre de ruptures dans un modèle de segmentation}\label{ch:outils:sec:selection:subs:segmentation}
\input{./chapitres/outils/selection/segmentation}


==> chapitres/outils/selection/bayesien.tex <==
\subsubsection{Introduction}
\input{./chapitres/outils/selection/bayesien/introduction}

\subsubsection{Critère BIC}
\input{./chapitres/outils/selection/bayesien/BIC}

==> chapitres/outils/selection/bayesien/BIC.tex <==
Est présenté ici le critère de \textcite{schwarz}, équivalent au critère appelé BIC pour \emph{Bayesian information criterion}. Ce critère permet d'approcher $P(m=\cdot | \boldsymbol{y})$ par une log-vraisemblance maximisée pénalisée et, par conséquent, de remplacer le problème de maximisation de $P(m=\cdot | \boldsymbol{y})$ par le problème approché:
\begin{equation}\label{eq:BIC_vraisemblance_penalisee}
\widehat{m} = \underset{0\leq m^\prime\leq M}{\argmin} \left( -2\widehat{\mathcal{L}}_{m^\prime} + \mathrm{pen}_n (m^\prime) \right) \; ,
\end{equation}
où $\widehat{\mathcal{L}}_{m^\prime}$ est le maximum de la log-vraisemblance du modèle $\mathcal{M}_{m^\prime}$.

Nous présentons le critère BIC dans le contexte où variables aléatoires $y_i$ sont i.i.d., suivant la présentation de \textcite{kass1995bayes} et de \textcite{BIC}. $\mathcal{M}_m$ est ici le modèle auquel appartient la loi de chacune de ces observations. Ici, $m$ est une variable aléatoire sur $\left\lbrace 0,\dots ,M\right\rbrace$, que l'on va supposer de loi uniforme pour simplifier (c'est la loi à priori sur les modèles). D'après \eqref{eq:max_Pym}, comme $m$ suit la loi uniforme, il est équivalent de maximiser la loi à posteriori $P\left(m=\cdot|\boldsymbol{y}\right)$ ou la vraisemblance intégrée. On peut écrire la vraisemblance intégrée \eqref{eq:vraisemblance_integree} sous la forme

\begin{equation}\label{eq:VraisemblanceIntegree}
P(\boldsymbol{y} | m ) = \int_{\Theta_m} e^{nL_n (\vartheta)}\mathrm{d}\vartheta \; ,
\end{equation}
où
\begin{equation}\label{eq:Ln}
L_n(\vartheta) = \frac{1}{n} \sum_{i=1}^n \log \left(P\left(y_i|m,\theta_m=\vartheta\right) \right) + \frac{\log P\left(\theta_m = \vartheta | m\right)}{n} \; .
\end{equation}

\begin{prop}[Approximation de Laplace]\label{prop:Laplace}
Soient $d\geq 1$ entier et $L:\mathbb{R}^d\rightarrow \mathbb{R}$ une fonction trois fois différentiable sur $\mathbb{R}^d$. Supposons que $L$ atteint son unique maximum sur $\mathbb{R}^d$ en $\overline{x}$. Alors,
\begin{equation*}
\int_{\mathbb{R}^d} e^{nL(x)}\mathrm{d}x = e^{nL(\overline{x})} \left(\frac{2\pi}{n}\right)^{d/2} \left| - L^{\prime\prime}(\overline{x})\right| + O\left(n^{-1}\right) \; .
\end{equation*}
\end{prop}
Nous ne discuterons pas ici des conditions qui permettent d'appliquer ce résultat à la suite de fonctions $L_n$ \parencite[voir][]{BIC}. Ici, l'approximation de Laplace reste valable,  à une modification du terme d'erreur près:
\begin{equation*}
P(\boldsymbol{y} | m ) = e^{n L_n\left(\overline{\theta}_m\right)} \left(\frac{2\pi}{n}\right)^{d_m/2} \left| - L_n^{\prime\prime} \left(\overline{\theta}_m\right)\right| + O_P\left(n^{-1}\right) \; ,
\end{equation*}
où $\overline{\theta}_m$ est l'argument maximum de $L_n$ sur $\Theta_m$. D'après \eqref{eq:Ln}, le maximum de vraisemblance $\widehat{\theta}_m$ maximise $L_n(\vartheta) - \frac{P\left(\theta = \vartheta | m\right)}{n}$. Or, $\frac{\log P\left(\theta = \vartheta | m\right)}{n}$ est d'ordre $O(n^{-1})$ donc, asymptotiquement, $\overline{\theta}_m$ peut être remplacé par $\widehat{\theta}_m$. Finalement, on obtient
\begin{equation}\label{eq:approx_BIC}
\log \left(P\left(\boldsymbol{y} | m \right)\right) = \widehat{\mathcal{L}}_m -\frac{1}{2} d_m \log(n) + O_P (1) \; , (n\rightarrow \infty ) \; .
\end{equation}
%De cette équation et du problème d'approximation \eqref{eq:BIC_probleme_approximation} posé on déduit que $\mathrm{pen}_n :m^\prime\mapsto d_{m^\prime} \log n$ et 
Par conséquent, on propose de sélectionner le modèle suivant:
\begin{eqnarray}
\widehat{m} & = & \underset{0\leq m^\prime \leq M}{\argmin} BIC(m^\prime) \; , \\
\textit{où } BIC(m^\prime) & = & = -2\widehat{\mathcal{L}}_{m^\prime} + d_{m^\prime} \log(n) \; . \label{eq:BIC_definition}
\end{eqnarray}
\textcite{kass1995bayes} font une distinction entre le \emph{critère de Schwarz} et le critère BIC. Le critère de Schwarz est égal, par définition, à $-1/2\times$ le critère BIC. C'est ce dernier critère qui approche la probabilité à posteriori du modèle \eqref{eq:approx_BIC}. Toutefois, la confusion est grande entre ces deux critères qui sélectionnent le même modèle et il n'est pas rare de trouver l'expression \enquote{le critère BIC de Schwarz} dans la littérature.
\begin{remarque}
\begin{itemize}
\item On retrouve un critère pénalisé, ce qui fait le lien avec le cadre fréquentiste défini dans la section~\ref{ch:outils:sec:selection:subs:frequentiste}.
%\item $\log \left(P\left(\boldsymbol{y} | m \right)\right)$ croît linéairement en $n$, l'approximation faite grâce à l'équation \eqref{eq:approx_BIC} est donc satisfaisante.
\item BIC pénalise plus la log-vraisemblance maximisée qu'AIC. Les modèles sélectionnés sont donc plus parcimonieux.
\item Comme le fait remarquer \textcite[section 3.5]{choi1992arma}, le critère BIC a été introduit à quelques années d'intervalle par des auteurs différents, les familles de modèles considérés et les arguments employés variant avec eux. \textcites{akaike1977entropy}{akaike1978bayesian}{akaike1978} propose le critère BIC pour différents problèmes de sélection de modèle, dont la sélection des ordres $p$ et $q$ d'une série temporelle $ARMA(p,q)$ gaussienne centrée. Toutefois, l'approximation de Laplace n'est pas encore la justification de ces critères, des lois à priori spécifiques sont définies pour obtenir une identité entre le modèle qui maximise la probabilité à posteriori du modèle et celui qui minimise le critère BIC.  \textcite{hannan1980estimation} démontre que les ordres $\widehat{p}_n$ et $\widehat{q}_n$ ainsi sélectionnés sont consistants.
\item La construction du critère BIC est donnée dans le cas d'un échantillon i.i.d., mais ce critère peut s'utiliser dans bien d'autres cas, tant que les lois à priori et la log-vraisemblance sont suffisamment régulières et que la notion de dimension du modèle est bien définie.
\item Les hypothèses de la proposition~\ref{prop:Laplace} imposent des conditions de régularité à la fonction de log-vraisemblance pour que l'approximation \eqref{eq:approx_BIC} reste valable. Comme le font remarquer \textcite{berger2001objective}, l'irrégularité de la vraisemblance pour certains modèles fait que l'approximation \eqref{eq:approx_BIC} n'est plus valable. Dans le cas qui nous intéresse, la segmentation, nous verrons dans la section \ref{ch:outils:sec:selection:subs:segmentation} qu'une autre pénalité nous permettra d'approcher la probabilité à posteriori du modèle.
\end{itemize}
\end{remarque}

==> chapitres/outils/selection/bayesien/introduction.tex <==
On pourra se référer à \textcite[chapitre 7]{robert2006choix}, pour une présentation générale. On reprendra ici des notations usuelles, quoique abusives, de la statistique bayésienne. Si $X$ est une variable aléatoire:
\begin{itemize}
\item $P\left(X=x\right)$ est la densité de $X$ en $x$ par rapport à une certaine mesure de référence. La fonction de densité pourra être désignée par $P\left(X=\cdot\right)$.
\item Si la densité de $X$ dépend d'un paramètre $\theta\in\Theta$ et si on considère que ce paramètre est lui-même une variable aléatoire, la densité de $X$ conditionnellement à $\theta$ est $P\left(X=\cdot|\theta\right)$.
\item Toujours dans cette situation, $P\left(X|\theta\right)$ est la vraisemblance de $X$. La fonction de vraisemblance de $X$ en $\vartheta\in\Theta$ est alors $P\left(X|\theta=\vartheta\right)$.
\end{itemize}

Dans cette approche bayésienne:
\begin{itemize}
\item Les modèles sont paramétrés, de sorte que dans le modèle $\mathcal{M}_m$, la loi des observations $\boldsymbol{y}$ dépende d'un paramètre $\theta_m\in\Theta_m$. On note alors $P\left(\boldsymbol{y}|m,\theta_m\right)$ la vraisemblance de~$\boldsymbol{y}$.
\item $m$ est une variable aléatoire sur $\left\lbrace 0,\dots ,M\right\rbrace$.
\item Le paramètre $\theta_m$ est une variable aléatoire, elle suit une loi à priori $P\left(\theta_m|m\right)$ conditionnellement à $m$.
\end{itemize}

On s'intéresse à la loi à posteriori de $m$: $P\left(m=\cdot |\boldsymbol{y}\right)$. Cette loi est déterminée par la formule de Bayes:
\begin{equation*}%\label{eq:formule_Bayes}
P\left(m=\cdot |\boldsymbol{y}\right) = \frac{P\left(\boldsymbol{y}|m=\cdot \right)P\left(m=\cdot \right)}{P\left(\boldsymbol{y}\right)} \; .
\end{equation*}
Le principe de la sélection de modèle bayésienne est de sélectionner le modèle qui maximise la probabilité à posteriori du modèle sachant les observations. Cela revient à estimer $m$ par \emph{Maximum à posteriori}:
\begin{equation}\label{eq:max_proba_a_posteriori}
\widehat{m} = \underset{0\leq m^\prime \leq M}{\argmax} P\left(m= m^\prime | \boldsymbol{y} \right) \; .
\end{equation}
Il est équivalent de maximiser le \emph{facteur de Bayes} des modèles $\mathcal{M}_{m^\prime}$ et $\mathcal{M}_0$:
\begin{equation}\label{eq:max_Pym}
\widehat{m} = \underset{0\leq m^\prime \leq M}{\argmax} \frac{P\left(m=m^\prime | \boldsymbol{y} \right)}{P\left(m = 0 | \boldsymbol{y} \right)} = \frac{P\left(\boldsymbol{y}|m=m^\prime\right)P\left(m=m^\prime\right)}{P\left(\boldsymbol{y}|m= 0\right)P\left(m=0\right)} = \underset{0\leq m^\prime \leq M}{\argmax} P\left(\boldsymbol{y}|m=m^\prime \right)P\left(m=m^\prime\right) \; .
\end{equation}

$P\left(\boldsymbol{y}|m\right)$ est la \emph{vraisemblance intégrée} du modèle $\mathcal{M}_m$:
\begin{equation}\label{eq:vraisemblance_integree}
P\left(\boldsymbol{y}|m\right) = \int_{\theta_m\in\Theta_m} P\left(\boldsymbol{y}|m,\theta_m\right)P\left(\theta_m|m\right)\mathrm{d}\theta_m \; .
\end{equation}

Le facteur de Bayes des modèles $\mathcal{M}_{m^\prime}$ et $\mathcal{M}_0$ est le rapport des vraisemblances intégrées de ces modèles, corrigées du facteur $\frac{P\left(m=m^\prime\right)}{P(m=0)}$ représentant l'apriori sur les modèles.

Pour résoudre ce problème de maximisation \eqref{eq:max_Pym}, il faut être capable de calculer la vraisemblance intégrée \eqref{eq:vraisemblance_integree}. Trois cas se présentent:
\begin{itemize}
\item Cette intégrale est aisément calculable. On se trouve dans cette situation quand la vraisemblance $P\left(\boldsymbol{y}|m,\theta_m\right)$ et la loi à priori $P\left(\theta_m=\cdot|m\right)$ ont de bonnes propriétés réciproques. On peut par exemple se trouver dans cette situation si la loi à priori $P\left(\theta_m=\cdot|m\right)$ du paramètre $\theta_m$ appartient à une \emph{famille de lois de probabilités conjuguées} par $P\left(\boldsymbol{y}|m,\theta_m\right)$. $P\left(\theta_m=\cdot |\boldsymbol{y},m\right)$ appartient alors à la même famille de lois de probabilité sur $\Theta_m$. Le lecteur pourra se référer à \textcite[section 3.3]{robert2006choix} pour une présentation générale des lois à priori conjuguées.
\item L'intégrale \eqref{eq:vraisemblance_integree} est approchée par intégration numérique, faisant éventuellement appel à des méthodes d'échantillonnage.  Voir \textcite[section 7.3]{robert2006choix}.
\item On fournit une approximation de l'intégrale \eqref{eq:vraisemblance_integree} valable quand le nombre d'observations $n$ tend vers l'infini. Cette méthode est présentée dans la section suivante.
\end{itemize}

==> chapitres/outils/selection/frequentiste.tex <==
On reprend ici les notations définies dans la section~\ref{ch:outils:sec:selection:subs:introduction}. $\gamma_n : S \rightarrow \mathbb{R} $ est une fonction de contraste empirique, par exemple $-2/n \times$ la log-vraisemblance. Dans chacun des modèles $\mathcal{M}_m$, le paramètre $s^\star$ est estimé par minimisation de $\gamma_n$ sur $S_m$. Un tel estimateur est noté $\widehat{s}_m$.

\subsubsection{Critère pénalisé}

\input{./chapitres/outils/selection/frequentiste/critere}


\subsubsection{Sélection de modèle consistante}

\input{./chapitres/outils/selection/frequentiste/consistante}


\subsubsection{Sélection de modèle et oracle}
\input{./chapitres/outils/selection/frequentiste/oracle}


==> chapitres/outils/selection/frequentiste/consistante.tex <==
Il faut déterminer quelles conditions asymptotiques sur la suite réelle $\left(\mathrm{pen}_n (m)\right)_n$ dans~\eqref{eq:ch:outils:sec:selection:subs:frequentiste} garantissent la consistance de $\widehat{m}_n$.

Par exemple, on considère une famille finie de modèles $ARMA(p,q),\; (0\leq p\leq p_{\max}, 0\leq q\leq q_{\max})$ gaussiens et centrés contenant le vrai modèle $ARMA\left(p^\star,q^\star\right)$. D'après \textcite[chapitre 14, théorème 4.3]{azencott}, si la fonction de contraste $\gamma_n$ est l'opposé de la log-vraisemblance et si la pénalité est de la forme $\mathrm{pen}_n (p,q) = \frac{1}{2} (p+q)(1+p+q)\beta_n$, où $\left(\beta_n\right)_n$ est une suite réelle positive, alors
\begin{eqnarray*}
\lim_{n\rightarrow\infty} \frac{\beta_n}{n} = 0  & et & \underset{n\rightarrow\infty}{\underline{\lim}} \frac{\beta_n}{\log \log n} > 1
\end{eqnarray*}
est une condition suffisante pour que $\left(\widehat{p}_n,\widehat{q}_n\right)$ défini par~\eqref{eq:ch:outils:sec:selection:subs:frequentiste} converge presque-sûrement vers $\left(p^\star,q^\star\right)$.

==> chapitres/outils/selection/frequentiste/critere.tex <==
La sélection de modèle par critère pénalisé se fait en sélectionnant le modèle $\mathcal{M}_{\widehat{m}_n}$ tel que
\begin{equation}\label{eq:ch:outils:sec:selection:subs:frequentiste}
\widehat{m}_n = \underset{0\leq m\leq M}{\argmin} \left\lbrace \gamma_n\left(\widehat{s}_m\right) + \mathrm{pen}_n (m) \right\rbrace \; ,
\end{equation}
où $\mathrm{pen}_n : \left\lbrace 0 ,\dots ,M\right\rbrace \rightarrow \mathbb{R}$. $\mathrm{pen}_n$ est appelée la \emph{pénalité}. Cette pénalité doit être choisie de façon à répondre à certaines exigences. Au choix:
\begin{enumerate}
\item Rendre la sélection de modèle consistante, c'est-à-dire $\widehat{m}_n$ converge en probabilité vers le vrai $m$.
\item Imiter le comportement de \emph{l'oracle}.
\end{enumerate}


==> chapitres/outils/selection/frequentiste/oracle.tex <==
Pour simplifier l'exposé, prenons l'exemple de la sélection d'un modèle de régression. On dispose d'un vecteur aléatoire $\boldsymbol{y} = \left(y_i\right)_{1\leq i\leq n}$ tel que $\boldsymbol{y} = s^\star + \boldsymbol{\epsilon}$, où les composantes $\epsilon_i$ de $\boldsymbol{\epsilon}$ sont de loi normale, indépendantes, centrées, de même variance $1$ (sans perdre de généralité). $S$ est un sous-espace vectoriel de $\mathbb{R}^n$ et $\|\cdot \|$ est la norme euclidienne sur $\mathbb{R}^n$. Ici,
\begin{equation}\label{eq:fonction_contraste}
\forall s\in S, \gamma_n (s)  = \frac{1}{n} \left\| \boldsymbol{y} - s\right\|^2  \; . 
\end{equation}

Idéalement, on aimerait sélectionner le modèle
\begin{equation}
m\left(s^\star\right)  =  \argmin_{0\leq m \leq M} \mathbb{E}\left[\left\| s^\star - \widehat{ s}_m\right\|^2\right] \; . \label{eq:modele_oracle}
\end{equation}

$\widehat{s}_{m\left(s^\star\right)}$ est appelé \emph{l'oracle}. Ce n'est pas un estimateur de $s^\star$, car il dépend du vrai paramètre $s^\star$. Il faut donc sélectionner le modèle $\mathcal{M}_{\widehat{m}_n}$ de sorte que les propriétés de $\widehat{s}_{\widehat{m}_n}$ s'approchent de celles de l'oracle en un certain sens. L'idée de la sélection de modèle par minimisation du critère $C_p$ de \textcite{mallows1973some} est de remplacer l'expression à minimiser dans l'équation \eqref{eq:modele_oracle} par une expression approchée ne dépendant pas de $s^\star$. La différence entre les deux critères tend vers $0$ quand $n$ tend vers l'infini et l'approximation provient de $\mathbb{E}\left[\left\| \widehat{ s}_m\right\|^2\right]\approx \left\| \widehat{ s}_m\right\|^2$. Cela revient à prendre une pénalité $\mathrm{pen}_n (m) = \frac{2 d_m}{n}$. Dans le cas où la fonction de contraste $\gamma_n$ est $-2/n\times $ la log-vraisemblance, un raisonnement de même type conduit au critère AIC \parencites(\emph{Akaike information criterion}, voir)(){akaike1998information}{akaike1974new}, défini par la même pénalité. Toutefois, la construction du critère AIC implique un développement de Taylor à l'ordre deux de la log-vraisemblance. Par conséquent, cette dernière doit être au moins deux fois différentiable.

Dans ce raisonnement, l'approximation $\mathbb{E}\left[\left\| \widehat{ s}_m\right\|^2\right]\approx \left\| \widehat{ s}_m\right\|^2$ repose sur deux choses. D'une part, il faut que $n$ soit suffisamment grand. Néanmoins, en ce qui concerne le critère AIC, une version adaptée AICc, proposée par \textcite{hurvich1989regression}, existe pour les cas où cette condition n'est pas vérifiée. D'autre part, il faut que le nombre de modèles ne dépende pas de $n$. Ces conditions ne sont pas toujours remplies, ce qui a motivé l'approche non-asymptotique en sélection de modèle \parencites{birge2001gaussian}[voir][pour une présentation générale]{massart2007concentration}. Ici, plutôt que de compter sur la convergence de $\left\| \widehat{ s}_m\right\|^2$ vers son espérance, on va contrôler ses variations autour de son espérance à l'aide d'une inégalité de concentration de la mesure, dans le but d'obtenir une inégalité oracle:
\begin{equation}\label{eq:inegalite_oracle}
\exists C_n\geq 1, \; \mathbb{E}\left[\left\| s - \widehat{s}_{\widehat{m}_n}\right\|^2\right] \leq  C_n \inf_{0\leq m\leq M}\mathbb{E}\left[\left\| s - \widehat{s}_{m}\right\|^2\right] \; .
\end{equation}

==> chapitres/outils/selection/introduction.tex <==
La question générale de la sélection de modèle est: parmi un ensemble donné de modèles, lequel choisir au vu des observations? Notamment, on s'attache à estimer la dimension du modèle.

%La présentation suivante de la problématique générique de la sélection de modèle provient de \cite[chapitre 1]{massart2007concentration}. 
On dispose d'observations $\boldsymbol{y}=(y_1,\dots ,y_n)$, un $n$-uplet de variables aléatoires sur un ensemble $E$, et de $M+1$ modèles $\mathcal{M}_0,\dots ,\mathcal{M}_M$, sous-modèles de $\mathcal{M}$. La loi de $\boldsymbol{y}$ dépend d'un paramètre $s^\star\in S$. La loi de $\boldsymbol{y}$ appartient au modèle $\mathcal{M}_m$ si et seulement si $s^\star\in S_m$, où $ S_0,\dots, S_M$ sont des sous-ensembles de $S$. On note $d_m$ la dimension de $S_m$ ($0\leq m\leq M$).

Par exemple, on peut considérer une famille de modèles $ARMA(p,q)$ pour $\boldsymbol{y}$ sans connaître les ordres $p$ et $q$. Il faut alors construire un critère de sélection de modèle pour choisir ces ordres qui définissent un modèle dans lequel on va travailler. De même, dans un modèle de segmentation, on sélectionne le nombre de ruptures du modèle.

La sélection de modèle peut se faire à l'aide de tests d'hypothèses sur l'appartenance de la loi des observations à un modèle \citep{rao2001model}. Le problème est que, au-delà de deux modèles considérés, cela implique de réaliser plusieurs tests successifs, le résultat dépendant de l'ordre dans lequel est réalisée cette succession. Alternativement, on cherche le meilleur modèle parmi une collection, selon un critère à définir. Nous allons aborder cette dernière approche dans deux cadres, fréquentiste et bayésien.

==> chapitres/outils/selection/segmentation.tex <==
Nous allons reprendre chacun des principes de sélection de modèle exposés dans les sections~\ref{ch:outils:sec:selection:subs:frequentiste} et~\ref{ch:outils:sec:selection:subs:bayesien} et s'intéresser à leur application éventuelle en segmentation. La difficulté principale dans ce cadre spécifique tient de la nature discrète des instants de rupture. $m$ est ici le nombre de ruptures. C'est pour estimer ce nombre de ruptures que la sélection de modèle est nécessaire.

\subsubsection{Sélection consistante du nombre de ruptures}
\input{./chapitres/outils/selection/segmentation/consistante}


\subsubsection{Sélection du nombre de ruptures par imitation d'un oracle}
\input{./chapitres/outils/selection/segmentation/oracle}

\subsubsection{Critères BIC et BIC modifié}\label{ch:outils:sec:selection:subs:seg:subsubs:bic}
\input{./chapitres/outils/selection/segmentation/BIC}

\subsubsection{Autres méthodes bayésiennes de sélection du nombre de ruptures}
\input{./chapitres/outils/selection/segmentation/autres}

\subsubsection{Calibration des constantes et hyperparamètres}
\input{./chapitres/outils/selection/segmentation/constantes}

==> chapitres/outils/selection/segmentation/BIC.tex <==
\textcite{yao} propose l'utilisation du critère BIC défini en~\eqref{eq:BIC_definition} pour la segmentation de l'espérance d'un processus gaussien à variance inconnue et démontre la consistance du nombre de ruptures ainsi sélectionné. Toutefois, une étude de simulations \parencite[section 2.4.]{Zha05} comparant cette méthode à quatre autres met en lumière ses faibles performances.

Contrairement au raisonnement de \textcite{schwarz}, le critère BIC, dans le cadre de la segmentation, ne correspond pas à une approximation de la probabilité à posteriori du nombre de ruptures sachant les observations. La difficulté d'approcher cette probabilité dans le problème de la segmentation provient de la discontinuité de la fonction de vraisemblance en les paramètres de localisation des ruptures. Or, l'approximation de Laplace (cf. proposition \ref{prop:Laplace}), permettant de lier le critère BIC à cette probabilité, nécessite des conditions de régularité qui ne sont pas remplies dans le cas présent.

Il est possible de contourner cet obstacle \citep{ZS} et d'obtenir une approximation du facteur de Bayes par le résultat qui suit.
\begin{theo}\label{th:mBIC_ZS}
Soit $m$ une v.a. sur $\mathbb{N}$, $\boldsymbol{\mu}=\left(\mu_0,\dots,\mu_m\right)$ un vecteur aléatoire réel et $\sigma$ v.a.r. positive. Conditionnellement à $m$, $\boldsymbol{t}=\left(t_0,\dots ,t_{m+1}\right)$ est une v.a. sur 
$$\mathcal{C}_{m,n}=\left\lbrace \left(t_0^\prime,\dots ,t_{m+1}^\prime\right)\in\mathbb{R}^{m+2} ; 0=t_0^\prime < t_1^\prime < \dots < t_m^\prime < t_{m+1}^\prime = 1\right\rbrace \; .$$
Les lois à priori sont spécifiées par \textcite[Théorème 2]{ZS}.
Soit $\boldsymbol{y}=\left(y_1,\dots ,y_n\right)$ un vecteur aléatoire réel tel que, conditionnellement à $m$, $\boldsymbol{\mu}$, $\boldsymbol{t}$ et $\sigma$, les $y_i$ sont indépendants et de loi $\mathcal{N}\left(\mu_k ,\sigma^2\right)$ si $t_k < i \leq t_{k+1}$. Alors,
\begin{multline}\label{eq:mBIC_ZS}
\log \frac{P(m | \boldsymbol{y})}{P(m=0 | \boldsymbol{y})} = \frac{n+1}{2}\log\left(SS_{all}\right) - \frac{n-m+1}{2} \log\left(SS_{wg}\right) + \log\left(\frac{\Gamma\left(\frac{n-m+1}{2}\right)}{\Gamma\left(\frac{n+1}{2}\right)}\right)\\
 - \frac{1}{2}\sum_{k=0}^m \log \widehat{n}_k + \left(\frac{1}{2}-m\right)\log (n) + O_P (1) \; (n\rightarrow +\infty ) \; , 
\end{multline}
où
\begin{eqnarray*}
SS_{all} & = & \min_{\mu\in\mathbb{R}} \sum_{i=1}^n \left(y_i - \mu\right)^2 \; ,\\
SS_{wg} & = & \min_{\boldsymbol{t}\in\mathcal{C}_m} \min_{\boldsymbol{\mu}\in\mathbb{R}^{m+1}} \sum_{k=0}^m \sum_{i=t_k +1}^{t_{k+1}} \left(y_i - \mu_k \right)^2 \; , \\
\widehat{n}_k & = & \widehat{t}_{k+1} - \widehat{t}_k \; , \textit{où}\\
\left(\widehat{t}_0,\dots ,\widehat{t}_{m+1}\right) & = & \underset{\boldsymbol{t}\in\mathcal{C}_m}{\argmin} \min_{\boldsymbol{\mu}\in\mathbb{R}^{m+1}} \sum_{k=0}^m \sum_{i=t_k +1}^{t_{k+1}} \left(y_i - \mu_k \right)^2 \; ,
\end{eqnarray*}
et où $\Gamma$ est la fonction Gamma d'Euler.
\end{theo}
L'approximation du facteur de Bayes \eqref{eq:mBIC_ZS} permet de définir un critère pénalisé de sélection de modèle, qu'on appelle \emph{BIC modifié} (mBIC) de \textcite{ZS}.


==> chapitres/outils/selection/segmentation/autres.tex <==
\textcite{rigaill2012exact} proposent l'utilisation de lois à priori conjuguées des paramètres propres à chaque segment dans plusieurs modèles de segmentation où les observations sont indépendantes (conditionnellement aux paramètres) ainsi que certaines lois à priori spécifiques pour les paramètres de localisation des ruptures. Ce choix permet l'obtention d'une forme analytique de la vraisemblance intégrée~\eqref{eq:vraisemblance_integree} et son calcul. Toutefois, les lois à priori des paramètres dépendent d'hyperparamètres, que l'on retrouve dans la loi à posteriori du nombre de ruptures.

==> chapitres/outils/selection/segmentation/consistante.tex <==
On peut imposer que les variables $n$ et $m$ soient séparées dans la pénalité:

$$ \mathrm{pen}_n (m) = \beta_n m \; .$$

On étudie la convergence du nombre de ruptures estimé $\widehat{m}_n$ vers $m$ en fonction des propriétés asymptotiques de la suite $\left(\beta_n\right)$. Ce type de résultat est fréquent dans la littérature~\parencites{lee1995}[théorème 3.1]{lavielle1999}[théorème 9]{LM}[théorème 4]{braun2000multiple}[théorème 3.1]{BKW10}. Les propositions~\ref{ar1:Prop:SelBeta} et~\ref{ar1:Prop:SelBeta2} sont des résultats de ce type.

Reste le problème de la spécification de $\left(\beta_n\right)$. En effet, les résultats cités ci-dessus ne donnent que des conditions de convergence de $\widehat{m}_n$ et absolument pas de formule pour $\left(\beta_n\right)$.
On peut fixer une forme de $\beta_n$ à priori, dépendante de constantes non spécifiées (voir par exemple la remarque~\ref{ar1:remark:forme_beta}). Les conditions sur $\left(\beta_n\right)$ sont alors traduites en conditions sur ces constantes.

==> chapitres/outils/selection/segmentation/constantes.tex <==
Parmi les critères de sélection de modèle pour la segmentation présentés, on trouve des constantes non spécifiées. \textcites{lavielle2005using}{arlot2009data} proposent des heuristiques de calibration de ces constantes. Dans le cadre bayésien, la présence d'hyperparamètres pose un problème similaire \citep{rigaill2012exact}. L'avantage du critère BIC modifié est l'absence de telles constantes.

==> chapitres/outils/selection/segmentation/oracle.tex <==
L'approximation à la source du critère du $C_p$ de Mallows n'est plus valable dans le cadre des modèles de segmentation \parencite[chapitre 4]{massart2007concentration}. Cela motive l'utilisation d'un critère non-asymptotique.

On considère $\boldsymbol{y}=\left(y_1,\dots,y_n\right)$, un vecteur gaussien de composantes indépendantes et de même variance $1$ (sans perdre de généralité). On cherche à sélectionner le nombre de ruptures $m$ dans l'espérance de $\boldsymbol{y}$. La fonction de contraste est définie par \eqref{eq:fonction_contraste}.

Pour établir une inégalité oracle, \textcite{lebarbier2005detecting} utilise les résultats de \textcite{birge2001gaussian} et propose la pénalité suivante:
\begin{equation}\label{eq:penalite_emilie}
\mathrm{pen}_n (m) = \frac{m+1}{n} \left(c_1 \log\left(\frac{n}{m+1}\right) +c_2\right) \; ,
\end{equation}
$c_1>0$ et $c_2>0$ étant deux constantes.

==> chapitres/outils/series.tex <==
Dans toute cette section, on s'intéressera à un processus aléatoire réel $X=\left(X_i\right)_{i\in\mathbb{Z}}$. On présente ici les propriétés des séries temporelles utilisées dans le reste du manuscrit. Notre référence principale à ce sujet est \textcite{brockwell}.

\input{./chapitres/outils/series/stationnarite}

\input{./chapitres/outils/series/arma}

\input{./chapitres/outils/series/estimation_stationnaire}

==> chapitres/outils/series/arma.tex <==
\subsection{Processus ARMA}\label{subs:ARMA}
%%%EDIT: mis en Subsection.
Les processus ARMA sont une classe importante de processus stationnaires. En effet, pour tout $\gamma:\mathbb{Z}\rightarrow\mathbb{R}$ fonction d'autocovariance associée à un processus stationnaire du second ordre et, pour tout $H\in\mathbb{N}$, il existe un processus ARMA $X$ tel que $\forall h \in\mathbb{Z},|h|\leq H\Rightarrow \gamma_X (h) = \gamma (h)$.%%%EDIT: Reformulé plus précisément. Réf demandée par CLL: Intro au chapitre 3 du Brockwell-Davis.

\begin{definition}
$B$ est l'automorphisme de \emph{décalage} sur l'espace vectoriel des processus aléatoires (réels) du second ordre indicés par $\mathbb{Z}$, défini par $\forall i \in\mathbb{Z}, \left(BX\right)_i = X_{i-1}$.

On note $B^j = B\circ \dots \circ B$ ($j$ fois) pour $j\geq 1$, $B^j = B^{-1}\circ \dots \circ B^{-1}$ ($-j$ fois) pour $j\leq -1$ et $B^0$ l'identité.
 
Pour tout polynôme (réel ou complexe) $P(z) = \sum_{j=0}^d a_j z^j$, on définit $P\left(B\right) = \sum_{j=0}^d a_j B^j$. 
\end{definition}

\begin{prop}\label{prop:CvLaurent}
Soit $\left(\psi_j\right)_{j\in\mathbb{Z}}$. Si $\sum_{j=-\infty}^{+\infty} \left|\psi_j\right|<+\infty$ et $X$ stationnaire, alors pour tout $i\in \mathbb{Z}$, $\sum_{j=-\infty}^{+\infty} \psi_j X_{i-j}$ converge absolument, dans l'espace $L^2$ et presque-sûrement. Le processus $\left(\sum_{j=-\infty}^{+\infty} \psi_j X_{i-j}\right)_{i\in\mathbb{Z}}$ est lui-même stationnaire.
\end{prop}
La proposition \ref{prop:CvLaurent} permet la définition suivante.
\begin{definition}
Soit $\left(\psi_j\right)_{j\in\mathbb{Z}}$. Si $\sum_{j=-\infty}^{+\infty} \left|\psi_j\right|<+\infty$,
on peut définir $\Psi\left(B\right) = \sum_{j=-\infty}^{+\infty} \psi_j B^j$, endomorphisme de l'espace vectoriel des processus aléatoires stationnaires du second ordre indicés par $\mathbb{Z}$.
\end{definition}

\begin{definition}\label{def:arma}
On dit que $X$ est un processus $ARMA(p,q)$ si c'est un processus stationnaire à l'ordre deux et s'il existe $\Phi (z) = 1 - \sum_{j=1}^p \phi_j z^j$ et $\Theta (z) = 1 + \sum_{j=1}^q \theta_j z^j$ des polynômes et $\epsilon=\left(\epsilon_i\right)_{i\in\mathbb{Z}}$ bruit blanc tel que
\begin{equation}\label{eq:arma}
\Phi\left(B\right)X = \Theta\left(B\right) \epsilon \; ,
\end{equation}
ou, de façon équivalente,
\begin{equation}\label{eq:arma_expanded}
\forall i\in\mathbb{Z}, X_i - \sum_{j=1}^p \phi_j X_{i-j} = \epsilon_i + \sum_{j=1}^q \theta_j \epsilon_{i-j} \; .
\end{equation}
\end{definition}
\begin{remarque}
Un tel processus n'existe pas nécessairement pour tout couple de polynômes $\left(\Phi,\Theta\right)$ (cf. exemple \ref{ex:ar1}, cas $\left|\rho\right|=1$).
\end{remarque}
\begin{exemple}
Un processus $ARMA(0,0)$ est un bruit blanc.
\end{exemple}
\begin{exemple}
Si $p=0$, on parle de processus de \emph{moyenne mobile} et on note $MA(q)$ au lieu de $ARMA(0,q)$. Un tel processus existe pour tout polynôme $\Theta$ et pour tout bruit blanc $\epsilon$.
\end{exemple}
\begin{exemple}
Si $q=0$, on parle de processus \emph{autorégressif} et on note $AR(p)$ au lieu de $ARMA(p,0)$. L'étymologie est parlante: il s'agit d'une régression linéaire du processus sur lui-même, en l'occurrence sur son passé. Le présent s'explique linéairement par le passé et le bruit blanc $\epsilon$ joue le rôle de la perturbation.
\end{exemple}
\begin{exemple}[Processus $AR(1)$]\label{ex:ar1}
Ici, \eqref{eq:arma_expanded} devient 
\begin{equation}\label{eq:arOne}
\forall i\in\mathbb{Z}, X_i - \rho X_{i-1} = \epsilon_i \; ,
\end{equation}
 où $\rho$ est un nombre réel.
\begin{itemize}
\item Si $\left|\rho\right|<1$, l'unique solution stationnaire (à égalité presque-sûre près) de \eqref{eq:arOne} est $X=\left(X_i\right)_{i\in\mathbb{Z}}$ défini par, pour tout $i\in\mathbb{Z}$, $X_i \overset{p.s.}{=} \sum_{j=0}^{\infty} \rho^j \epsilon_{i-j}$. Dans ce cas, $\forall h\in\mathbb{Z}, \rho_X (h) = \rho^{|h|}$.
\item Si $\left|\rho\right|>1$, l'égalité devient  $X_i \overset{p.s.}{=} -\sum_{j=1}^{\infty} \rho^{-j} \epsilon_{i+j}$.
\item Si $\left|\rho\right|=1$, \eqref{eq:arOne} n'a pas de solution stationnaire.
\end{itemize}
Une différence importante apparaît entre les cas $\left|\rho\right|<1$ et $\left|\rho\right|>1$. Dans le premier cas, $X_i$ n'est pas corrélé avec $\left(\epsilon_j\right)_{j>i}$ (le \enquote{futur} du bruit blanc), alors que dans le second cas, $X_i$ s'écrit linéairement à  partir de $\left(\epsilon_j\right)_{j>i}$. Ce fait illustre la notion de causalité.
\end{exemple}

\begin{definition}
Soit $X$ un processus $ARMA(p,q)$ défini par \eqref{eq:arma}. $X$ est dit \emph{causal} s'il existe une suite $\left(\psi_j\right)_{j\geq 0}$ telle que $\sum_{j=0}^{\infty}\left|\psi_j\right|<\infty$ et
\begin{equation}\label{eq:causal}
\forall i\in\mathbb{Z}, X_i = \sum_{j=0}^{\infty} \psi_j \epsilon_{i-j} \; .
\end{equation}
D'après la proposition \ref{prop:CvLaurent}, cette série converge absolument, dans l'espace $L^2$ et presque-sûrement.
\end{definition}

\begin{theo}[Caractérisation de la causalité]\label{th:caracterisation_causalite}
Soit $X$ un processus $ARMA(p,q)$ défini par \eqref{eq:arma} et tel que les polynômes $\Phi$ et $\Theta$ n'ont pas de racine commune. Alors $X$ est causal si et seulement si $\forall z\in\mathbb{C}, \left|z\right|\leq 1 \Rightarrow \Phi (z) \neq 0$. Les coefficients $\psi_j$ de \eqref{eq:causal} s'obtiennent par le développement en série entière de $\frac{\Theta}{\Phi}$:
$$\forall z\in\mathbb{C}, \left|z\right|\leq 1 \Rightarrow \Psi (z) = \sum_{j=0}^\infty \psi_j z^j = \frac{\Theta (z)}{\Phi (z)} \; .$$
\end{theo}
%
%\begin{definition}\label{def:ARMAinversible}
%$X$ processus $ARMA(p,q)$ défini par \eqref{eq:arma} est dit \emph{inversible} s'il existe une suite $\left(\pi_j\right)_{j\geq 0}$ telle que $\sum_{j=0}^{\infty}\left|\pi_j\right|<\infty$ et
%\begin{equation}\label{eq:invertible}
%\forall i\in\mathbb{Z}, \epsilon_i = \sum_{j=0}^{\infty} \pi_j X_{i-j} \; .
%\end{equation}
%D'après la proposition \ref{prop:CvLaurent}, cette série converge absolument, dans l'espace $L^2$ et de façon presque sûre.
%\end{definition}
%
%\begin{theo}[Caractérisation de l'inversibilité]
%Soit $X$ processus $ARMA(p,q)$ défini par~\eqref{eq:arma}, tel que les polynômes $\Phi$ et $\Theta$ n'ont pas de racine commune. Alors $X$ est inversible si et seulement si $\forall z\in\mathbb{C}, \left|z\right|\leq 1 \Rightarrow \Theta (z) \neq 0$. Les coefficients $\pi_j$ de \eqref{eq:invertible} s'obtiennent par le développement en série entière de $\frac{\Phi}{\Theta}$:
%$$ \forall z\in\mathbb{C}, \left|z\right|\leq 1 \Rightarrow \Pi (z) = \sum_{j=0}^\infty \pi_j z^j = \frac{\Phi (z)}{\Theta (z)} \; .$$
%\end{theo}

\begin{theo}[Unicité de la solution de l'équation ARMA]
Soient $\epsilon$, $\Phi$ et $\Theta$ définis comme dans la définition \ref{def:arma}. Si $\forall z\in\mathbb{C}, \left|z\right|= 1 \Rightarrow \Phi (z) \neq 0$, alors \eqref{eq:arma} a une unique solution stationnaire $X$, définie par
$$ X=\Psi (B)\epsilon \; , $$
où $\Psi$ est le développement en série de Laurent de  $\frac{\Theta}{\Phi}$ au voisinage du cercle complexe unité.
\end{theo}

==> chapitres/outils/series/estimation_stationnaire.tex <==
\subsection{Estimation dans les processus stationnaires d'ordre deux}

\input{./chapitres/outils/series/estimation_stationnaire/estimation_autocorrelation}

\input{./chapitres/outils/series/estimation_stationnaire/estimation_arma}

==> chapitres/outils/series/estimation_stationnaire/estimation_arma.tex <==
\subsubsection{Estimation dans les processus ARMA}

\paragraph{Notations}

on notera ici, pour $X$ un processus faiblement stationnaire et $k\geq 0, p\geq 1, q\geq 0$ entiers,

\begin{eqnarray}
\Gamma_{q,p} & = & \left(\gamma_X (i-j-q)\right)_{1\leq i,j\leq p} \; , \label{eq:def_Gamma_qp}\\
R_{q,p} & = & \left(\rho_X (i-j-q)\right)_{1\leq i,j\leq p} \; , \label{eq:def_R_qp}\\
\boldsymbol{\gamma}_{k,p} & = & \left(\gamma_X(k),\dots ,\gamma_X(p)\right)^T  \textit{ si } p\geq k\; , \label{eq:def_gamma_kp} \\
\boldsymbol{\rho}_{k,p} & = & \left(\rho_X(k),\dots ,\rho_X(p)\right)^T \textit{ si } p\geq k \; . \label{eq:def_rho_kp}
\end{eqnarray}

Si $X$ est un processus $ARMA(p,q)$ vérifiant l'équation \eqref{eq:arma_expanded}, on notera $\Phi = \left(\phi_1,\dots ,\phi_p\right)^T$.

\paragraph{\'Equations de Yule-Walker et généralisation}

\begin{prop}\label{prop:Yule_Walker_ARMA}
Si $X$ est un processus $ARMA(p,q)$, avec $p\geq 1$ et $q\geq 0$, alors
\begin{eqnarray}
\Gamma_{q,p} \Phi & = & \boldsymbol{\gamma}_{1+q,p+q} \; , \label{eq:Yule_Walker_gamma_ARMA} \\
R_{q,p} \Phi & = & \boldsymbol{\rho}_{1+q,p+q} \; , \label{eq:Yule_Walker_rho_ARMA}
\end{eqnarray}
où $\Gamma_{q,p}$, $R_{q,p}$, $\boldsymbol{\gamma}_{1+q,p+q}$ et $\boldsymbol{\rho}_{1+q,p+q}$ sont définis en~\eqref{eq:def_Gamma_qp}--\eqref{eq:def_rho_kp}.
\end{prop}

\begin{remarque}
Si on fixe $q=0$, les équations \eqref{eq:Yule_Walker_gamma_ARMA} et \eqref{eq:Yule_Walker_rho_ARMA} sont les équations de Yule-Walker. $\Gamma_{0,p}$ et $R_{0,p}$ sont des matrices symétriques définies positives. En particulier, elles sont inversibles. Si $q\geq 1$, $\Gamma_{q,p}$ et $R_{q,p}$ ne sont pas symétriques. Le résultat suivant est tiré d'\textcite[chapitre 11, paragraphe 2]{azencott}.
\end{remarque}

\begin{prop}\label{prop:Inversibilite_Yule_Walker_ARMA}
Si $X$ un processus $ARMA(p,q)$ avec $p\geq 1$ et $q\geq 0$ et $\Gamma_{q,p}$, $R_{q,p}$, $\boldsymbol{\gamma}_{1+q,p+q}$ et $\boldsymbol{\rho}_{1+q,p+q}$ sont définis en \eqref{eq:def_Gamma_qp}--\eqref{eq:def_rho_kp}, alors $\Gamma_{q,p}$ et $R_{q,p}$ sont des matrices inversibles. En particulier,
\begin{equation}\label{eq:Yule_Walker_inverse}
\Phi = \Gamma_{q,p}^{-1} \boldsymbol{\gamma}_{1+q,p+q} = R_{q,p}^{-1} \boldsymbol{\rho}_{1+q,p+q} \; .
\end{equation}
\end{prop}

\paragraph{Utilisation des équations de Yule-Walker pour l'estimation}

On notera, pour $X$ un processus faiblement stationnaire, $p\geq 1, q\geq 0$ entiers et pour $\overline{\gamma}_X(h)$ (resp. $\overline{\rho}_X (h)$) estimateur de $\gamma_X(h)$ (resp. $\rho_X (h)$) si $h\in\mathbb{Z}$,

\begin{eqnarray*}
\overline{\Gamma}_{q,p} & = & \left(\overline{\gamma}_X (i-j-q)\right)_{1\leq i,j\leq p} \; , \\
\overline{R}_{q,p} & = & \left(\overline{\rho}_X (i-j-q)\right)_{1\leq i,j\leq p} \; , \\
\overline{\boldsymbol{\gamma}}_{q,p} & = & \left(\overline{\gamma}_X(q),\dots ,\overline{\gamma}_X(p)\right)^T  \textit{ si } p\geq q\; , \\
\overline{\boldsymbol{\rho}}_{q,p} & = & \left(\overline{\rho}_X(q),\dots ,\overline{\rho}_X(p)\right)^T \textit{ si } p\geq q \; .
\end{eqnarray*}

Si $X$ est un processus $ARMA(p,q)$, on peut alors estimer $\Phi$ à l'aide de l'équation \eqref{eq:Yule_Walker_inverse}, en remplaçant les $\gamma_X (h)$ par leurs estimateurs. On considère alors un des estimateurs suivants de $\Phi$:
\begin{eqnarray}
\overline{\Phi} & = & \overline{\Gamma}_{q,p}^{-1} \overline{\boldsymbol{\gamma}}_{1+q,p+q} \textit{ ou bien} \label{eq:general_Yule_Walker_gamma} \\
\overline{\Phi} & = & \overline{R}_{q,p}^{-1} \overline{\boldsymbol{\rho}}_{1+q,p+q} \; . \label{eq:general_Yule_Walker_rho}
\end{eqnarray}

Si les estimateurs des $\gamma_X(h)$ (resp. $\rho_X (h)$) sont les estimateurs de la méthode des moments~(voir définition~\ref{def:EMM_autocovariance_autocorrelation}) et si $q=0$, alors $\overline{\Gamma}_{q,p}$ et $\overline{R}_{q,p}$ sont des matrices symétriques définies positives. Le calcul de $\overline{\Phi}$ se fait alors à l'aide de l'algorithme de Durbin-Levinson \parencite[section 8.2]{brockwell}. En dehors de ces conditions, on n'a pas de garantie sur l'inversibilité de $\overline{\Gamma}_{q,p}$ ou $\overline{R}_{q,p}$. On peut tenter de démontrer qu'asymptotiquement ces matrices sont presque-sûrement inversibles.

\textcite{shevlyakov2014few} proposent d'estimer la fonction d'autocovariance ou d'autocorrélation de façon robuste puis d'utiliser~\eqref{eq:general_Yule_Walker_gamma} ou~\eqref{eq:general_Yule_Walker_rho} pour estimer $\Phi$ dans le cas $q=0$. Dans le chapitre~\ref{ch:arp}, nous proposons la même démarche avec $q=1$.

==> chapitres/outils/series/estimation_stationnaire/estimation_autocorrelation.tex <==
\subsubsection{Estimation de la fonction d'autocovariance et de la fonction d'autocorrélation}
On dispose de $n$ observations consécutives $X_1,\dots ,X_n,$ d'un processus faiblement stationnaire.

\begin{definition}\label{def:EMM_autocovariance_autocorrelation}
Soient $X_1,\dots ,X_n,$ $n$ observations consécutives d'un processus faiblement stationnaire $X$. Soit un entier $0\leq h< n$. \emph{L'estimateur de la méthode des moments} de $\gamma_X(h)$ est
\begin{equation*}%\label{eq:EMM_autocovariance}
\widehat{\gamma}_X (h) = \frac{1}{n} \sum_{i=1}^{n-h} \left(X_i - \overline{X}_n\right)\left(X_{i+h} - \overline{X}_n\right) \; ,
\end{equation*}
où $\overline{X}_n = \frac{1}{n}\sum_{i=1}^n X_i$. \emph{L'estimateur de la méthode des moments} de $\rho_X(h)$ est
\begin{equation*}%\label{eq:EMM_autocorrelation}
\widehat{\rho}_X (h) = \frac{\widehat{\gamma}_X (h)}{\widehat{\gamma}_X(0)} \; .
\end{equation*}
\end{definition}

\begin{remarque}
Il existe d'autres estimateurs de la fonction d'autocovariance et de la fonction d'autocorrélation. Voir, par exemple, la section \ref{subs:REstScaleAutoco}.
\end{remarque}

==> chapitres/outils/series/stationnarite.tex <==
\subsection{Stationnarité, fonctions d'autocovariance et d'autocorrélation}

La loi de $X$ est caractérisée par la famille des fonctions de répartition $\left(F_{\boldsymbol{i}}\right)_{\boldsymbol{i}\in\mathcal{I}}$, où $\mathcal{I} = \left\lbrace \boldsymbol{i} = \left(i_1, \dots , i_k \right)\in\mathbb{Z} ; i_1 < \dots < i_k , k\in\mathbb{N}^* \right\rbrace $ et $F_{\boldsymbol{i}} (\boldsymbol{z}) = P\left(X_{i_1} \leq z_1 , \dots , X_{i_k} \leq z_k\right)$, pour tout $\boldsymbol{z} = \left(z_1 , \dots , z_k\right)$.
Parmi ces lois, on souhaite caractériser celles qui sont invariantes par décalage d'indices.

\begin{definition}
$X$ est dit \emph{strictement stationnaire} si $\forall h \in \mathbb{Z}, \forall \boldsymbol{i}\in\mathcal{I}, F_{\boldsymbol{i}} = F_{\boldsymbol{i}+h}$, où  $\boldsymbol{i}+h = \left(i_1 +h,\dots ,i_k +h\right)$ si $\boldsymbol{i}=\left(i_1,\dots ,i_k\right)$.
\end{definition}

Il s'agit d'une propriété forte. Dans bien des cas, une notion plus faible de stationnarité suffit. Cette dernière étant liée aux moments d'ordre deux, il faut introduire la notion de processus du second ordre.

\begin{definition}
$X$ est dit \emph{du second ordre} si, pour tout $i\in\mathbb{Z}$, $X_i$ est de carré intégrable.
\end{definition}

\begin{definition}\label{def:stationnarite_faible}
Un processus du second ordre $X$ est dit \emph{faiblement stationnaire}, ou \emph{stationnaire à  l'ordre deux}, si:
\begin{enumerate}
\item $\forall i \in \mathbb{Z}, \mathbb{E}X_i = \mathbb{E} X_0 \; , $
\item $\forall i\in\mathbb{Z}, \forall h \in \mathbb{Z}, \cov \left(X_i, X_{i+h}\right) = \cov \left(X_0 , X_h\right) \; .$
\end{enumerate}
On définit alors la \emph{fonction d'autocovariance} $\gamma_X : \mathbb{Z}\rightarrow\mathbb{R}$ associée à   $X$ par
$$\forall h\in\mathbb{Z}, \gamma_X \left(h\right) = \cov \left(X_0 , X_h\right) \; , $$
 ainsi que la \emph{fonction d'autocorrélation} $\rho_X : \mathbb{Z}\rightarrow\mathbb{R}$ associée à   $X$ par 
 $$\rho_X = \frac{\gamma_X}{\gamma_X\left(0\right)}\; . $$
 $\rho_X$ n'est bien définie que si $\gamma_X\left(0\right)>0$.
\end{definition}
En l'absence de spécification, un processus dit \emph{stationnaire} n'est que faiblement stationnaire. L'exemple le plus simple d'un tel processus est le bruit blanc.

\begin{definition}
On dit que $X$ est un \emph{bruit blanc} de variance $\sigma^2>0$ si $X$ est un processus du second ordre faiblement stationnaire tel que $\mathbb{E}X_0 = 0$ et $\forall h\in\mathbb{Z},\gamma_X\left(h\right) = \sigma^2 \delta_{0,h}$.
\end{definition}

La stationnarité forte d'un processus du second ordre implique la stationnarité faible. La réciproque est fausse en général.

==> chapitres/perspectives.tex <==
\section{Limites de l'approche adoptée}

\input{./chapitres/perspectives/critiques}

\section{Perspectives}

\input{./chapitres/perspectives/estimation}


==> chapitres/perspectives/critiques.tex <==
L'approche proposée n'est pas exempte de certaines limites. Nous les formulerons concernant deux aspects: les limitations algorithmiques et la nature des résultats proposés.

\subsection{Programmation dynamique et dépendance}

\input{./chapitres/perspectives/critiques/PDA}


\subsection{Cadre asymptotique}

\input{./chapitres/perspectives/critiques/asymptotique}

==> chapitres/perspectives/critiques/PDA.tex <==
Dans cette section, nous discutons la spécificité de la méthode employée au cas d'un bruit autorégressif.

Nous avons proposé une méthode pour la segmentation de l'espérance d'un processus autorégressif. La justification de l'approche adoptée repose en grande partie sur la volonté de conserver l'utilisation de l'algorithme de programmation dynamique pour obtenir la segmentation optimale. Cet algorithme permet de minimiser un critère additif sur les segments~(voir section~\ref{ch:outils:sec:algo}). Toutefois, cette démarche semble difficilement généralisable. Plaçons-nous dans le modèle général suivant:
\begin{equation*}%\label{perspectives:eq:modele_matriciel}
\boldsymbol{y} = T\left(\boldsymbol{t}_n^{\star}\right) \boldsymbol{\mu}^{\star} + \sigma\boldsymbol{\eta}\;,
\end{equation*}
où $\sigma>0$ inconnu, $\boldsymbol{y}$ et $\boldsymbol{\eta}$ sont des matrices $n\times 1$ aléatoires; $\boldsymbol{\eta}^T$ est centrée, de carré intégrable et de matrice de variance/covariance $\Sigma$; $\boldsymbol{\mu}^{\star}$ est une matrice $(m+1)\times 1$; $\boldsymbol{t}_n^{\star} \in \mathcal{A}_{n,m} = \left\{\boldsymbol{t}=(t_0,\dots ,t_{m+1}) \in \rset^{m+2} ; 0=t_0 < t_1 <\dots t_m < t_{m+1}=n \right\}$ et pour $\boldsymbol{t}\in \mathcal{A}_{n,m}$,  $T\left(\boldsymbol{t}\right)$ est une matrice $n \times (m+1)$ dont la $k^e$ colonne est $( \underset{t_{k-1}}{\underbrace{0,\dots , 0}} \; \underset{t_k-t_{k-1}}{\underbrace{1,\dots ,1}} \; \underset{n - t_k}{\underbrace{0,\dots ,0}} )^T$.

On cherche à estimer $\boldsymbol{t}_n^{\star}$ à $m$ et $\Sigma$ connus. On a:
\begin{equation*}%\label{perspectives:eq:modele_matriciel_decor}
\Sigma^{-1/2}\boldsymbol{y} = \Sigma^{-1/2}T\left(\boldsymbol{t}_n^{\star}\right) \boldsymbol{\mu}^{\star} + \sigma\boldsymbol{\epsilon}\;,
\end{equation*}
où $\boldsymbol{\epsilon}^T$ est une v.a. sur $\rset^n$ centrée, de carré intégrable, dont la matrice de variance/covariance est l'identité. On souhaite estimer $\boldsymbol{t}_n^{\star}$ et $ \boldsymbol{\mu}^{\star}$ en minimisant sur $\mathcal{A}_{n,m}$ et l'ensemble des matrices réelles $n\times 1$ le critère des moindres carrés:
$$C\left(\boldsymbol{t},\boldsymbol{\mu}\right) = \left\|\Sigma^{-1/2}\boldsymbol{y} - \Sigma^{-1/2}T\left(\boldsymbol{t}\right)\boldsymbol{\mu}\right\|^2 \; . $$
À $\boldsymbol{t}$ fixé, on a:
$$ \underset{\boldsymbol{\mu}}{\min} \; C\left(\boldsymbol{t},\boldsymbol{\mu} \right) = \left\|\Sigma^{-1/2}\boldsymbol{y} - \pi_{\Sigma^{-1/2}T\left(\boldsymbol{t}\right)} \Sigma^{-1/2}\boldsymbol{y}\right\|^2 \; , $$
où $\pi_{\Sigma^{-1/2}T\left(\boldsymbol{t}\right)}$ est la matrice dans la base canonique de la projection orthogonale sur le sous-espace vectoriel de $\rset^n$ engendré par les colonnes de $\Sigma^{-1/2}T\left(\boldsymbol{t}\right)$. Pour que ce critère soit additif sur les segments, nous devons disposer d'une famille de vecteurs $\left(f(i,j)\right)_{1\leq i<j \leq n}$ de $\rset^n$ telle que pour tout $\boldsymbol{t}$, $\left(f(t_{k-1}+1,t_k)\right)_{1\leq k \leq m+1}$ est une base orthonormée du sous-espace vectoriel engendré par les colonnes de $\Sigma^{-1/2}T\left(\boldsymbol{t}\right)$. Dans ce cas, on a:
$$ \underset{\boldsymbol{\mu}}{\min} \; C\left(\boldsymbol{t},\boldsymbol{\mu} \right) = \left\|\Sigma^{-1/2}\boldsymbol{y}\right\|^2 - \sum_{k=1}^{m+1} \left\|\pi_{f(t_{k-1}+1,t_k)} \Sigma^{-1/2}\boldsymbol{y}\right\|^2 \; , $$
où $\pi_{f(t_{k-1}+1,t_k)}$ est la matrice dans la base canonique de la projection orthogonale sur la droite engendrée par $f(t_{k-1}+1,t_k)$, et le critère est bien additif sur les segments. Si $\Sigma$ est l'identité, l'existence d'une telle famille de vecteurs est triviale. Mais en toute généralité, on ne peut pas obtenir une telle famille de vecteurs pour un $\Sigma$ symétrique défini positif, éventuellement de Toeplitz, donné. Dans le cas des processus autorégressifs d'ordre fini, la solution proposée à ce problème de dépendance inter-segments fut, \textit{modulo} le conditionnement aux premières observations, d'approcher le sous-espace vectoriel engendré par $\Sigma^{-1/2}T\left(\boldsymbol{t}\right)$ par le sous espace-vectoriel engendré par $T\left(\boldsymbol{t}^\prime\right)$, où $\boldsymbol{t}^\prime$ contient des ruptures artéfactuelles, puis de post-traiter la segmentation obtenue. Cette démarche est impossible à généraliser à des processus stationnaires autres que l'AR($p$), car c'est seulement dans ce cas-là que les coefficients $(i,j)$ de $\Sigma^{-1/2}$ sont nuls si $|i-j|>p$.

Un autre choix pourrait être d'approcher $\Sigma$ par $\Sigma(\boldsymbol{t})$ dépendant de la segmentation $\boldsymbol{t}$, composée de blocs diagonaux de la taille des segments. Cela revient à ne pas prendre en compte la dépendance inter-segments dans l'inférence. Dans ce cas, les colonnes de $\Sigma^{-1/2}\left(\boldsymbol{t}\right)T\left(\boldsymbol{t}\right)$ sont bien orthogonales et le critère est additif sur les segments. Cette additivité est suffisante pour minimiser le critère par l'algorithme de programmation dynamique, mais insuffisante pour permettre l'utilisation de l'algorithme de programmation dynamique élaguée qui requiert des conditions supplémentaires~(voir section~\ref{subs:PDPA}). Notre approche de segmentation après décorrélation nous a permis de préserver la possibilité d'utiliser la programmation dynamique élaguée. Elle ne peut cependant pas être généralisée à des structures de dépendance plus complexes.

==> chapitres/perspectives/critiques/asymptotique.tex <==
Le cadre asymptotique permettant d'énoncer les résultats de notre travail peut être critiqué à plusieurs niveaux. Nous nous sommes placés dans le cadre asymptotique désormais classique où la localisation des ruptures dépend linéairement de la longueur des séries:
\begin{equation}\label{perspectives:eq:cadre_asymptotique}
t_{k,n}^\star = \left\lfloor n\tau_k^\star \right\rfloor \; (1\leq k \leq m) \; ,
\end{equation}
où $t_{1,n}^\star,\dots ,t_{m,n}^\star$ sont les instants des rupture de la série $y_1,\dots ,y_n$. Dans le cas où les observations sont indépendantes, ce cadre est naturel et indolore, nous l'avions déjà évoqué dans la section~\ref{ch:intro:sec:indep:subs:frequentiste}. Plusieurs résultats~\parencites{BP}{lavielle1999}{LM} sont venus étendre les propriétés des estimateurs de la localisation des ruptures dans le cas où une dépendance sérielle est présente. Si l'on excepte \textcite{BP}, qui se placent dans le cadre plus général des modèles linéaires à changements structurels où certaines formes de dépendance sérielle peuvent être prises en compte dans l'inférence~(sans que cela ne soit une obligation), ces résultats impliquent qu'asymptotiquement, des conditions relativement permissives sur cette dépendance sérielle font que cette dernière n'affecte ni la consistance ni la vitesse de convergence des estimateurs des instants de rupture. Si l'on se limite aux processus stationnaires du second ordre, on suppose qu'il existe un tel processus $\left(\eta_i\right)_{i\in\zset}$ centré tel que:
\begin{equation}\label{perspectives:eq:modeleLM}
\forall k\in\left\{1,\dots ,m^\star+1\right\}, \forall i\in\left\{t_{k-1,n}^\star+1,\dots ,t_{k,n}^\star\right\}, y_i = \mu_k^\star + \eta_i \; ,
\end{equation}
où $\mu_1^\star,\dots ,\mu_{m^\star+1}\in\rset$. Des conditions sont alors imposées à la fonction d'autocovariance $\gamma_\eta$ du processus $\left(\eta_i\right)_{i\in\zset}$ pour permettre l'établissement des résultats asymptotiques; on a en particulier $\gamma_\eta (h)\underset{h\rightarrow\infty}{\longrightarrow} 0$.  Par exemple, pour tout $k\in\left\{1,\dots ,m^\star+1\right\}$,
$$\mathrm{Cov}\left(y_{t_{k-1,n}^\star+1},y_{t_{k,n}^\star}\right) = \gamma_\eta\left(t_{k,n}^\star-t_{k-1,n}^\star-1\right) = \gamma_\eta\left(\left\lfloor n\tau_k^\star \right\rfloor-\left\lfloor n\tau_{k-1}^\star \right\rfloor-1\right) \underset{n\rightarrow\infty}{\longrightarrow} 0 \; . $$ 
On remarque que $\gamma_\eta$ ne dépend pas de $n$, contrairement aux instants de rupture. Bien qu'il ait permis d'établir des résultats importants, deux critiques peuvent être formulées à ce modèle:
\begin{itemize}
\item la première concerne son réalisme pour certains problèmes. En effet, si $n$ représente le nombre de mesures réalisées sur un intervalle de temps fixe, il n'y a aucune raison pour que prendre de nouvelles mesures entre deux précédentes réduise la dépendance entre ces dernières. Par exemple, dans le cas de la météorologie, cela revient à supposer qu'en prenant de nombreuses mesures (de température, etc.) on réduit la portée temporelle de la dépendance météorologique.
\item la seconde concerne ce qu'on pourrait appeler un déséquilibre dans les rôles respectifs des ruptures et de la dépendance sérielle. Supposons par exemple que \eqref{perspectives:eq:cadre_asymptotique} ne soit plus vraie et qu'il n'y a qu'une rupture à l'instant $t$. L'estimateur des moments de l'autocovariance à l'ordre $h$ fixé ne sera pas affecté asymptotiquement par la présence de cette rupture; cela revient de ce point de vue à considérer $t$ valeurs aberrantes parmi $n$ observations. Dans le modèle \eqref{perspectives:eq:modeleLM}, on fait le contraire; on efface partiellement l'effet asymptotique de la dépendance sérielle sur les estimateurs des instants de rupture.
\end{itemize}

Un choix alternatif consisterait en le modèle où \eqref{perspectives:eq:cadre_asymptotique} reste vrai et on observe $y_1,\dots ,y_n,$ tels que:
\begin{equation}\label{perspectives:eq:modeleOU}
\forall k\in\left\{1,\dots ,m^\star+1\right\}, \forall i\in\left\{t_{k-1,n}^\star+1,\dots ,t_{k,n}^\star\right\}, y_i \overset{d}{=} \mu_k^\star + X_{i/n} \; ,
\end{equation}
où $\left(X_t\right)_{0<t\leq 1}$ est un processus stochastique centré. Par exemple, on pourrait considérer que $\left(X_t\right)_{t\geq 0}$ est un processus d'Ornstein-Uhlenbeck centré et stationnaire, c'est-à-dire un processus gaussien centré de fonction de covariance $\Gamma$ définie par:
\begin{equation}\label{perspectives:eq:covarianceOU}
 \forall (s,t) \in \left(0,1\right], \Gamma(s,t) = ve^{-\alpha \left| s-t \right|} \; , 
\end{equation}
où $v,\alpha>0$, voir par exemple \textcite{breiman1968probability}. C'est l'analogue en temps continu de l'AR(1), dont les discrétisations régulières $\left(X_{i/n}\right)_{i\in\mathbb{N}}$ sont des projections sur $\mathbb{R}^\mathbb{N}$ de processus AR(1) de paramètre d'autorégression $ve^{-\alpha/n}$. À ma connaissance, rien ne permet d'affirmer que l'estimateur des moindres carrés des ruptures converge dans ce cas, et encore moins à la vitesse $1/n$. La figure~\ref{perspectives:fig:bbarou} illustre le fait que, contrairement au modèle~\eqref{perspectives:eq:modeleLM} avec $\gamma_\eta (h) \underset{h\rightarrow\infty}{\longrightarrow} 0$, dans le modèle défini par~\eqref{perspectives:eq:modeleOU}, la dépendance sérielle reste visible quand $n$ devient grand, ce qui affecte la visiblité à l'\oe{}il nu de la rupture.

Pour qui voudrait montrer la nécessité de prendre en compte la dépendance sérielle dans l'estimation des instants de rupture, il faudrait plutôt se placer dans le modèle~\eqref{perspectives:eq:modeleOU} que dans le modèle~\eqref{perspectives:eq:modeleLM}, d'éventuelles conditions permettant la convergence des estimateurs pourraient être plus discriminantes. Nous n'avons pas fait cela. Nous avons proposé une solution pratique et réaliste d'un point de vue calculatoire à la prise en compte de la dépendance sérielle dans l'estimation des instants de ruptures avec un bruit autorégressif, et avons exhibé une classe d'estimateurs des paramètres de l'autorégression dont les propriétés asymptotiques pour des modèles de type \eqref{perspectives:eq:modeleLM} justifient notre approche.

\begin{figure}[!h]
\centering
\includegraphics[width=0.9\textwidth]{vanishou2.pdf}
\caption[Comparaison des cas où le bruit est un bruit blanc, est AR(1) et est la discrétisation d'un processus d'Ornstein-Uhlenbeck pour des séries avec rupture.]{On observe $\left(y_i\right)_{1\leq i\leq n}=\left(\mu_i+\eta_i\right)_{1\leq i\leq n}$ où, d'une part, $\mu_i = 0$ si $i\leq n/2$ et $\mu_i=1$ sinon et, d'autre part, $\left(\eta_i\right)_{1\leq i\leq n}$ est centré, gaussien et de variances marginales 1. Gauche: les $\eta_i$ sont indépendants. Centre: $\eta_1,\dots ,\eta_n$, sont $n$ observations successives d'un processus AR(1) d'autocorrélation 0.7 à l'ordre 1. Droite: $\left(\eta_i\right)_{1\leq i\leq n}=\left(X_{i/n}\right)_{1\leq i\leq n}$, où $\left(X_t\right)_{t\geq 0}$ est un processus d'Ornstein-Uhlenbeck stationnaire de fonction d'autocovariance donnée par \eqref{perspectives:eq:covarianceOU}, avec $v=1$ et $\alpha=-250 \log(0.7)$. $n=250$ (haut), $n=2500$ (milieu) ou $n=25000$ (bas).}\label{perspectives:fig:bbarou}
\end{figure}
%\begin{itemize}
%\item Je fais comme tout le monde depuis Bai.
%\item Ce cadre a permis de produire de nombreux résultats asymptotiques.
%\item Ce cadre là est naturel et indolore dans le cas indépendant.
%\item Appliqué à des données dépendantes, ce cadre modifie le statut de la dépendance: la portée de la dépendance varie avec $n$.
%\item Ornstein-Ühlenbeck discrétisé.
%\end{itemize}

==> chapitres/perspectives/estimation.tex <==
Dans cette section sont tracées quelques perspectives possibles à ce travail. En premier lieu, dans la section~\ref{persp:subs:autocov}, on propose l'exploration d'une voie permettant peut-être de lever certaines hypothèses de normalité des observations présentes dans les chapitres~\ref{ch:ar1} et~\ref{ch:arp}. Ensuite, dans la section~\ref{persp:subs:nonparam}, est discutée la possibilité de se servir de notre méthode à priori spécifique à la segmentation dans l'espérance de processus avec un bruit autorégressif dans le cas où la structure de dépendance est plus générale et non-paramétrique. Enfin, dans la section~\ref{persp:subs:negbin}, un parallèle est établi avec des problèmes connexes au notre qui pourtant n'impliquent pas de dépendance entre observations.

\subsection{Estimation de la fonction d'autocovariance et d'autocorrélation}\label{persp:subs:autocov}

\input{./chapitres/perspectives/estimation/rho}

\subsection{Structure de dépendance non-paramétrique}\label{persp:subs:nonparam}

\input{./chapitres/perspectives/estimation/non_parametrique}

\subsection{Méthodologie basée sur l'estimation robuste préliminaire d'un paramètre global dans un modèle de segmentation}\label{persp:subs:negbin}

\input{./chapitres/perspectives/estimation/extension}

==> chapitres/perspectives/estimation/extension.tex <==
Le travail proposé est fondé sur une stratégie en deux temps qui a montré son efficacité et peut sans aucun doute être généralisée à d'autres cas. Un exemple est le cas d'observations indépendantes où les observations suivent une loi dépendant de deux paramètres: l'un local, dépendant de chaque segment; l'autre global, commun aux observations de toute la série. Nous avions évoqué dans la section~\ref{ch:outils:sec:algo} l'impossibilité en général d'utiliser la programmation dynamique pour optimiser un critère de segmentation dans le cas où un paramètre global est présent. L'exemple~\ref{outils:algo:exemple:negbin} sur la loi binomiale négative permettant d'illustrer ce fait avec des ruptures dans le paramètre d'espérance et un paramètre de surdispersion constant. Il s'agit ici du problème de minimisation suivant:

$$\underset{t_0<t_1<\dots<t_{m+1}<t_{m+1}=n}{\min}\underset{r>0}{\min} \underset{\boldsymbol{\mu}=\left(\mu_1,\dots,\mu_{m+1}\right)\in \left]0,+\infty\right[^{m+1}}{\min} \sum_{l=1}^{m+1} \sum_{i=t_{l-1}+1}^{t_l}\log\left\lbrace \frac{(r+\mu_l)^{r+y_i}y_i!\Gamma (r)}{r^r\mu_l^{y_i}\Gamma (r+y_i)}\right\rbrace \; , $$
où $\Gamma$ est la fonction Gamma d'Euler. Pour de plus amples développements sur la loi binomiale négative en elle-même, voir \textcite{johnson2005univariate}. Ce problème est lié à la segmentation de données génomiques de comptage issues du séquençage à haut-débit (\emph{Next-generation sequencing}, NGS). \textcite{cleynen2013approches} adopte une approche en deux temps: estimation préalable du paramètre de surdispersion $r$, puis segmentation à $r$ fixé. Ci-dessous, certaines de ses considérations.

Même en l'absence de ruptures, il n'y a pas d'expression explicite de l'estimateur du maximum de vraisemblance du paramètre de surdispersion. L'estimateur de la méthode des moments s'obtient dans ce cas par:
\begin{equation}\label{eq:EMMnegBin}
\widehat{r} = \frac{\overline{y}^2}{S^2-\overline{y}} \; , 
\end{equation}
avec les notations usuelles de la moyenne et de la variance empiriques. Si on dispose de plusieurs échantillons indépendants de la loi binomiale négative, avec un paramètre de surdispersion $r$ commun, \textcite{bliss1958negative} proposent:
\begin{itemize}
\item pour chaque échantillon, estimer $r$ par la méthode des moments \eqref{eq:EMMnegBin},
\item estimer $r$ par une moyenne pondérée de ces estimateurs propres à chaque échantillon, les poids privilégiant les estimateurs de petite variance,
\item recalculer les poids en fonction de cette estimation de $r$ et recommencer.
\end{itemize}

Dans un modèle de segmentation, le problème est qu'on ne sait pas où termine l'échantillon d'une loi et débute l'échantillon d'une autre loi. \textcite{cleynen2013approches} s'inspire de l'approche de \textcite{bliss1958negative} en considérant des fenêtres glissantes sur les données segmentées au lieu des échantillons différents. Au lieu d'une moyenne pondérée, une médiane est utilisée pour rendre robuste l'estimateur à l'effet des fenêtres contenant les instants de rupture. Toutefois, pour le moment, les propriétés d'un estimateur de ce type n'ont pas été établies.

==> chapitres/perspectives/estimation/non_parametrique.tex <==
Dans les chapitres~\ref{ch:ar1} et~\ref{ch:arp}, nous avons supposé que le modèle autorégressif considéré était le vrai modèle. Dans la section~\ref{subs:heuristic}, en sélectionnant l'ordre de l'autorégression $p$ en même temps que le nombre de ruptures $m$, nous n'avons supposé vrai qu'un des modèles autorégressifs. De façon plus générale, nous ne sommes pas contraints de supposer qu'un des modèles autorégressifs est le vrai. On peut voir l'estimation dans un modèle autorégressif comme une façon commode d'estimer des coefficients permettant de décorréler la série.

En particulier, il faudrait refaire les démonstrations des propositions de la section~\ref{sec:change-points} avec des hypothèses plus faibles sur le processus d'innovation $\left(\epsilon_i\right)_{i\in\zset}$. C'est possible et cela repose sur les résultats de \textcite{LM} appliqués à la série décorrélée, qui n'exigent pas tout ce que nous avons exigé de $\left(\epsilon_i\right)_{i\in\zset}$.

De plus, l'ordre $p$ de l'autorégression à sélectionner ne doit pas nécessairement être le \enquote{bon} ordre, qui d'ailleurs dans ce cas n'existe pas, mais celui qui fournit la meilleure décorrélation. Cette idée est en contradiction avec la philosophie générale du critère BIC, qui cherche à identifier le modèle le plus proche du vrai modèle.

==> chapitres/perspectives/estimation/rho.tex <==
Les propriétés asymptotiques des estimateurs des paramètres de l'autorégression proposés n'ont été étudiées que dans le cas gaussien. Dans le chapitre~\ref{ch:arp} et la section~\ref{ch:commentaires}, les propriétés asymptotiques des estimateurs proposés $\widehat{\Phi}_n^{(p)}$ (cas AR($p$)) et $\widetilde{\rho}_n^\prime$ (estimateur alternatif dans le cas AR(1)) reposent sur les propriétés asymptotiques des estimateurs de \textcite{MG} de l'autocovariance. Ces propriétés ont été établies dans le cas gaussien par \textcite{levy2011robust}. Ainsi, pour étendre les propriétés des estimateurs proposés au cas non-gaussien, il faudrait étendre les propriétés asymptotiques des estimateurs de \textcite{MG}. \textcite{levy2011robust} utilisent des résultats de convergence du processus empirique~(cf. section~\ref{subs:processus_empirique}) pour déterminer les propriétés asymptotiques des quantiles intervenant dans les estimateurs de \textcite{MG}. Un autre type de résultats avec des implications concernant les propriétés asymptotiques des quantiles est les représentations de Bahadur. La spécificité du cas qui nous intéresse est que les quantiles intervenant dans l'estimateur de \textcite{MG} sont des \emph{U-quantiles}.

\subsubsection{Représentation de Bahadur pour les U-quantiles}

\input{./chapitres/perspectives/estimation/rho/bahadur}

\subsubsection{Le problème des constantes}

\input{./chapitres/perspectives/estimation/rho/constantes}


==> chapitres/perspectives/estimation/rho/bahadur.tex <==
\textcite{wendler2011bahadur} établit une représentation de Bahadur pour les U-quantiles de processus strictement stationnaires dépendants réels $\boldsymbol{X}=\left(X_i\right)_{i\in\zset}$, sous certaines conditions de régularité sur la dépendance entre observations. Une représentation de Bahadur est un développement asymptotique des quantiles empiriques sur la fonction de répartition empirique \parencite{kiefer1967}. On notera $F$ la fonction de répartition de la loi des $X_i$. Pour $h\in\zset$, on considèrera aussi les deux processus $\boldsymbol{X}^{ h\pm}=\left(X_i\pm X_{i+h}\right)_{i\in\zset}$, de loi marginale de fonction de répartition $F^{h \pm}$.

Ces résultats portent sur les U-quantiles, que l'on définit à partir des U-fonctions de répartition empirique. On considèrera des U-fonctions de répartition empirique qui sont des fonctions aléatoires réelles de variable réelle $U_n$, définies par:
\begin{equation}\label{perspectives:eq:uecdf}
\forall t\in\rset, U_n (t) = \frac{2}{n(n-1)} \sum_{1\leq i<j\leq n} g(X_i,X_j,t) \; ,
\end{equation}
où $g:\rset^3\rightarrow \left[0,1\right]$ est une fonction symétrique en les deux premières variables et croissante en la dernière. La U-fonction de répartition est alors $U:\rset\rightarrow \left[0,1\right]$ où, pour tout $t\in\rset$, $U(t)=\PE\left[g(A,B,t)\right]$ avec $A$ et $B$ des v.a.r. indépendantes de même loi que les $X_i$. Pour $p\in\left(0,1\right)$, le $p$-U-quantile et le $p$-U-quantile empirique sont alors respectivement $U^{-1}(p)$ et $U_n^{-1}(p)$. Par exemple, l'estimateur $Q_n$ de \textcite{CR} est:
\begin{equation}\label{perspectives:eq:defQn}
Q_n = c_{Q,F}U_n^{-1}(1/4) \; , 
\end{equation}
où $U_n$ est défini en \eqref{perspectives:eq:uecdf} avec
\begin{equation}\label{perspectives:eq:gQn}
\forall (x,y,t)\in\rset^3, g(x,y,t)=\1_{|x-y|\leq t} \; ,
\end{equation}
et $c_{Q,F}>0$ est une constante, dépendante de F. On considèrera aussi l'estimateur $Q_n$ des processus $\boldsymbol{X}^{ h\pm}$ qu'on notera $Q_n^{(h\pm)}$.  Les notations $U^{(h\pm)}$, $U_n^{(h\pm)}$ s'en déduisent.

Soit $p\in (0,1)$. Sous certaines conditions de régularité sur $g$---remplies si \eqref{perspectives:eq:gQn} est vérifiée---sur $U$ et sur la dépendance sérielle, \textcite{wendler2011bahadur} établit une représentation de Bahadur:
\begin{equation}\label{perspectives:eq:bahadur}
U_n^{-1}(p) - U^{-1}(p) = \frac{U_n\left(U^{-1}(p)\right)-p}{U^\prime\left(U^{-1}(p)\right)} + R_n \; .
\end{equation}
Nous ne détaillerons pas ici en quel sens le reste $R_n$ est \enquote{petit}. \textcite{wendler2011bahadur} en déduit ensuite la convergence en loi vers une loi normale de $\sqrt{n}\left(U_n^{-1}(p) - U^{-1}(p)\right)$ sous les mêmes hypothèses.

On obtient la convergence et la normalité asymptotique de $Q_n$. Si $X_1$ est de carré intégrable, pour que la limite de $Q_n$ soit bien $\sqrt{\Var(X_1)}$, il faut avoir:
\begin{equation}\label{perspectives:eq:cQF_Uquantile}
c_{Q,F} = \frac{\sqrt{\Var(X_1)}}{U^{-1}(1/4)} \; .
\end{equation}
Il n'est pas nécessaire de connaître $F$ pour déterminer une telle constante, il suffit de connaître un modèle de localisation-dispersion auquel il appartient:
$$ F \in \left\{ t\mapsto G\left(\frac{t-\mu}{\sigma}\right) ; \; \mu\in\rset, \sigma>0\right\} \; , $$
où $G$ est une fonction de répartition.

Les estimateurs de \textcite{MG} de l'autocovariance et de l'autocorrélation à l'ordre $h\in\zset$ de $\boldsymbol{X}$, sont notés respectivement $\widehat{\gamma}_n(h)$ et $\widehat{\rho}_n(h)$ (cf. équations \eqref{eq:MGcov} et \eqref{eq:MGcorr}).
%\begin{eqnarray}
%\widehat{\gamma}_n(h) & = & \frac{Q_{n-h}^{(h+)2} - Q_{n-h}^{(h-)2}}{4} \; , \label{perspectives:eq:gammaMG} \\
%\widehat{\rho}_n(h) & = & \frac{Q_{n-h}^{(h+)2} - Q_{n-h}^{(h-)2}}{Q_{n-h}^{(h+)2} + Q_{n-h}^{(h-)2}} \; . \label{perspectives:eq:rhoMG}
%\end{eqnarray}
Comme conséquence de la consistance et de la normalité asymptotique de $Q_{n}^{h\pm}$, sous les hypothèses du théorème 2 de \textcite{wendler2011bahadur} sur les processus $\boldsymbol{X}^{ h\pm}$, on a la consistance et la convergence en $O_P\left(n^{-1/2}\right)$ de $\widehat{\gamma}_n(h)$ et de $\widehat{\rho}_n(h)$. On remarquera que, dans le cas AR(1), cette propriété suffit à faire converger l'estimateur $\widetilde{\rho}_n^\prime$ du paramètre d'autorégression $\rho^\star$, défini en \eqref{ch:commentaires:sec:ar1:subs:autre:eq:def}, en $O_P\left(n^{-1/2}\right)$. Or, il s'agit de la condition énoncée dans la proposition~\ref{ar1:Prop:Segment2} pour décorréler les séries à segmenter à l'aide de cet estimateur.

Pour établir la normalité asymptotique de $\widehat{\gamma}_n(h)$ et de $\widehat{\rho}_n(h)$, il faudrait établir la normalité asymptotique conjointe des estimateurs $Q_{n-h}^{(h\pm)}$. On peut montrer que cette question se réduit à celle de la normalité asymptotique de U-statistiques sur le processus $\left(X_i,X_{i+h}\right)_{i\in\zset}$ par l'intermédiaire de l'équation~\eqref{perspectives:eq:bahadur} et du théorème de Cramér-Wold~\parencite[théorème 29.4]{billingsley1995probability}.

==> chapitres/perspectives/estimation/rho/constantes.tex <==
La convergence de $Q_n^2$ vers la variance du processus dépend du choix de la constante $c_{Q,F}$, qu'il faut fixer comme dans l'équation~\eqref{perspectives:eq:cQF_Uquantile}. Pour fixer ainsi une telle constante, il faut connaître un modèle de localisation-dispersion auquel appartient $F$. Par conséquent, la consistance de $\widehat{\gamma}_n(h)$ dépend des constantes $c_{Q,F^{(h\pm)}}$ des estimateurs $Q_{n-h}^{(h\pm)}$, où $F^{(h\pm)}$ est la loi marginale de $\boldsymbol{X}^{(h\pm)}$. Pour pouvoir les choisir de façon adéquate, il faut donc connaître les modèles de localisation-dispersion auxquels appartiennent respectivement $F^{(h +)}$ et $F^{(h -)}$. Il ne suffit pas de connaître $F$, il faut avoir un minimum d'information sur la loi des couples $\left(X_i,X_{i+h}\right)$, ce qui n'est pas toujours le cas quand l'on souhaite précisément estimer la covariance de ce couple. Si $\boldsymbol{X}$ est un processus gaussien, on sait que $F^{(h +)}$ et $F^{(h -)}$ appartiennent au même modèle de localisation-dispersion, celui des lois normales. En dehors de ce cas, cela reste un problème. La consistance de $\widehat{\rho}_n(h)$ ne dépend, pour sa part, que de $c_{Q,F^{(h+)}}/c_{Q,F^{(h-)}}$.  Si $\boldsymbol{X}$ est un processus gaussien, ce rapport vaut 1. Il serait précieux d'être capable d'établir des conditions sous lesquelles ce rapport vaut 1.

==> chapitres/perspectives/estimation/rho/stables.tex <==
%Plaçons nous dans le cadre des processus linéaires définis en \eqref{perspectives:eq:causaux}, où les $\epsilon_i$ suivent une loi stable symétrique intégrable, i.e. leur fonction caractéristique est $\phi:t\mapsto \exp\left(-d |t|^\alpha\right)$ avec les paramètres $\alpha\in\left(1,2\right]$ et $d>0$. Les lois normales centrées correspondent au cas $\alpha=2$. En dehors du cas de la loi normale, la variance associée à ces lois est infinie. Pour une présentation générale des lois stables, voir \cite{zolotarev1986one}. En travaillant sur la fonction caractéristique, on obtient aisément qu'un tel processus $\boldsymbol{X}$ (resp. $\boldsymbol{X}^{(h\pm)}$) a pour loi marginale une loi stable symétrique de paramètres $\alpha$ et $d_{\boldsymbol{X}}=d\sum_{j=-\infty}^\infty \left|\psi_j\right|^\alpha$ (resp. $d_{\boldsymbol{X}^{(h\pm)}}=d\sum_{j=-\infty}^\infty \left|\psi_j\pm \psi_{j+h}\right|^\alpha$).
%
%Comme dans le cas $\alpha<2$ ces lois ne sont pas de carré intégrable, on peut fixer arbitrairement la constante dans $Q_n$:
%$$ c_{Q,F} = c_{Q,F^{(h\pm)}} = c_{Q,\Phi} \; , $$
%où $c_{Q,\Phi}$ est ladite constante dans le cas de la loi normale. $Q_n$ (resp. $Q_{n-h}^{(h\pm)}$) converge donc vers
%$$ c_{Q,\Phi}U^{-1}(1/4) \left( \textit{ resp. } c_{Q,\Phi}U^{(h\pm)-1}(1/4) \; .$$
%Les propriétés des lois stables font que $\int \1_{\left|x-y\right\|\leq 1/4} \mathrm{d}F(x) \mathrm{d}F(y)$ dépend de $\alpha$ et linéairement de $d^{1/\alpha}$. Par conséquent, $U^{(h\pm)-1}(1/4)$ dépend linéairement de $d_{\boldsymbol{X}^{(h\pm)}}^{1/\alpha}
%Par conséquent, l'estimateur $\widehat{\rho}_n\left(h)$ de l'autocorrélation à l'ordre $h\in\zset$ converge vers
%$$ \frac{c_{Q,\Phi}U^{(h\pm)-1}(1/4)}{•} $$
